Optimizing Layout of Recursive Datatypes with Marmoset

While programmers know that the low-level memory representation of data structures can have significant effects on performance, compiler support to optimize the layout of those structures is an under-explored field. Prior work has optimized the layout of individual, non-recursive structures without considering how collections of those objects in linked or recursive data structures are laid out. This work introduces Marmoset, a compiler that optimizes the layouts of algebraic datatypes, with a special focus on producing highly optimized, packed data layouts where recursive structures can be traversed with minimal pointer chasing. Marmoset performs an analysis of how a recursive ADT is used across functions to choose a global layout that promotes simple, strided access for that ADT in memory. It does so by building and solving a constraint system to minimize an abstract cost model, yielding a predicted efficient layout for the ADT. Marmoset then builds on top of Gibbon, a prior compiler for packed, mostly-serial representations, to synthesize optimized ADTs. We show experimentally that Marmoset is able to choose optimal layouts across a series of microbenchmarks and case studies, outperforming both Gibbons baseline approach, as well as MLton, a Standard ML compiler that uses traditional pointer-heavy representations.

==> abstract.tex <==
% \section{Abstract}

\begin{abstract}


While programmers know that memory representation of data structures can have significant effects
on performance, compiler support to {\em optimize} the layout of those structures is an under-explored field.
Prior work has optimized the layout of individual, \textit{non-recursive} structures without considering how
collections of those objects in linked or \textit{recursive} data structures are laid out.
%The internal layout of constituent objects in linked data structures is an under-explored field.

%or focused on arranging the 
%placement of linked data structures without considering the internal layout of the constituent objects.

This work introduces \system, a compiler that optimizes the layouts of algebraic datatypes, with a special focus
on producing highly optimized, {\em packed} data layouts where recursive structures can be traversed with minimal
pointer chasing. \system performs an analysis of how a recursive ADT is used across functions to choose a \textit{global} layout
that promotes simple, strided access for that ADT in memory. It does so by building and solving a constraint system
to minimize an abstract cost model, yielding a predicted efficient layout for the ADT. \system then builds on top
of \gibbon, a prior compiler for packed, mostly-serial representations, to synthesize optimized ADTs. We show experimentally 
that \system is able to choose optimal layouts across a series of microbenchmarks and case studies, outperforming both 
\gibbon's baseline approach, as well as \mlton, a Standard ML compiler that uses traditional
pointer-heavy representations.


%\bf{ABSTRACT 2}
%
%Compilers treat the layout of fields in memory as a matter of
%preestablished convention, not as a free variable to optimize for a
%particular input program.
%%
%This rigidity incurs an opportunity cost, especially as we move to
%consider more compact in-memory representations for data; for example,
%as found in the \gibbon compiler which uses compact, mostly-serialized
%heap formats.
%
%This paper introduces \system, a compilation approach for functional
%programs which uses a solver to determine the optimal-cost ordering of
%data fields, optimizing for a particular traversal function over that
%data.
%%
%An experimental evaluation and case study shows that this approach
%yields an \auditme{XYZ} speedup over the compact-data approach alone,
%and an \auditme{XYZ} speedup over the mature GHC compiler with its
%traditional, pointer-heavy, non-compact data representations.
  
\end{abstract}


==> background.tex <==
%% \section{Background}
%% \label{sec:background}
%% \vs{background should be here. Needs background on Local and Gibbon.}
%% \mr{I introduced an Overview section that appears just before this one. Some of the material in the background section is now in Overview. Mostly the material is the high-level discussion. Now, the Background section will mainly be here to present the formalism, and anything not already introduced in the Overview.}

%% \note{new plan from Slack messages (VS): so really background could be why serializing helps (spatial locality == fast traversals)  + there is a compiler to automatically do this called gibbon + some local details?}
%% \mv{If this is just going to be an overview of the benefits of serialized heaps, is there a reason we can't just merge it into the previous section?}

%% In this section we present the Gibbon compiler in more detail, focusing in particular on its intermediate language and type system.
%% %
%% The Gibbon compiler uses LoCal~\cite{Local,gibbon-par} (\textbf{Lo}cation
%% \textbf{Cal}culus), a first-order intermediate representation (IR) where
%% programs are represented with an explicit byte-addressed, mostly-serialized data
%% layout. Gibbon translates programs into LoCal using \emph{location inference}, a
%% procedure built on top of region inference~\cite{regioncalcs} which annotates
%% programs with explicit location and region bindings and annotations. All values
%% reside within a region, which is (conceptually) an unbounded storage agea.
%% Locations are addresses within a region, and they are used for reading and
%% writing data. Locations roughly correspond to C's pointers but are less
%% flexible in that locations can only be written to once and arithmetic on
%% locations is highly restricted. A location is either: at the start of a region,
%% $N$ bytes past an existing location (to account for constant-sized data like integers), or \emph{after} the value at a particular
%% location (which may be constructed recursively). This serial ordering of locations is what ensures that the resulting
%% values are serialized in heap memory.
%% %
%% LoCal's type system tracks the data written to and read from
%% locations, ensuring that all data in all regions is well-typed.

%% \begin{figure}[]
%% \newcommand{\ctyatlocreg}[3]{\textcolor{emacsgreen}{#1}\textcolor{emacsbrown}{\bfseries\ensuremath{@}}\ensuremath{\locreg{#2}{#3}}}
%% \lstset{
%%     escapeinside={(@}{@)},          % if you want to add LaTeX within your code
%%     escapechar={\@},
%%     mathescape=true,
%% }
%% \begin{lstlisting}[ ]
%% 	data List = Cons Int List | Nil

%% 	@{\color{emacsblue}\text{mkList}}@ :: forall @\locreg{l}{r}@. Int -> @\ctyatlocreg{List}{l}{r}@
%% 	@{\color{emacsblue}\text{mkList}}@ [@\locreg{l}{r}@] n =
%% 	  if n == 0 then Nil @\locreg{l}{r}@ else
%% 	    @{\color{emacsblue}\texttt{letloc}}@ $\locreg{l_1}{r}$ = $\;\locreg{l}{r}$ + 9 in
%% 	    let tail: @\ctyatlocreg{List}{l_1}{r}@ = mkList [@\locreg{l_1}{r}@] (n-1) in
%% 	    Cons @\locreg{l}{r}@ n tail
%% \end{lstlisting}
%% \caption{\il{mkList} compiled into LoCal IR}\label{fig:mklist-LoCal}
%% \end{figure}

%% \begin{figure}[]
%% \includegraphics[scale=0.4]{figures/example1-list.pdf}
%% \caption{In-memory representation of list constructed by \il{mkList}}\label{fig:mklist-repr}
%% \end{figure}

%% An example LoCal program is shown in Figure~\ref{fig:mklist-LoCal}. The
%% \il{mkList} function takes a number \il{n} and a symbolic location \locreg{l}{r}
%% (read as: location \il{l} in region \il{r}), and returns a list of length \il{n}
%% at location \locreg{l}{r}. LoCal programs make use of a form of
%% \emph{destination-passing style}~\cite{destination-passing}, as the location
%% that the result will be written to is passed as an argument to the function.
%% %
%% If \il{n} is $0$, then \il{mkList} allocates \il{Nil} at location \locreg{l}{r}.
%% Otherwise, \il{mkList} must allocate a cons cell to \locreg{l}{r}. To do this, a
%% location $\locreg{l_1}{r}$ is introduced with a special \il{letloc} form, which
%% is 9 bytes past the location \locreg{l}{r} (one byte for the \il{Cons} tag and 8
%% bytes for the integer). Next, it recursively builds a list of length $(n-1)$ at
%% the newly bound location $\locreg{l_1}{r}$. Finally, it writes the \il{Cons} tag
%% and the integer \il{n}, completing the cons cell.
%% %
%% The resulting list is guaranteed by the types to be serialized in memory, within region \il{r}. Gibbon's location inference places all the cons cells in the same region because their allocations happen in order, ensuring the region will end up looking like the list in Figure~\ref{fig:mklist-repr}.

%% \mv{We can explain more about LoCal here if necessary. What do we need to establish about LoCal before moving on to section 4?}


==> conclusion.tex <==
\section{Conclusions}

%\ap{probably needs rewriting for ECOOP resubmission}
This paper introduces \system, which builds on \gibbon to generate efficient orders for algebraic datatypes. We show that a straightforward control-flow and data-flow analysis allows \system to identify opportunities to place fields of a data constructor near each other in memory to promote efficient consecutive access to those fields. Because a given function might use many fields in many different ways, \system adopts an approach of formulating the data layout problem as an ILP, with a cost model that assigns an abstract cost to a chosen layout. Armed with the ILP problem formulation, an off-the-shelf ILP solver allows \system to generate minimal-(abstract)-cost layout for algebraic datatypes. \system then uses the best layout to synthesize a new ADT and the \gibbon compiler toolchain to lower the code into an efficient program that operates over packed datatypes with minimal pointer chasing.

We show, across a number of benchmarks, that \system is able to effectively and consistently find the optimal data layout for a given combination of traversal function and ADT. In our experiments, \system-optimized layouts outperform not only \gibbon's default layouts but also the popular SML compiler \mlton.


==> defs.tex <==
% ================================================================================
% extra \newcommand's specific to this paper.
% ================================================================================

%% Oh no, we don't actually HAVE lambda!
%% Later we'll have to make this a higher-order calculus!
%% \newcommand{\ourcalc}[0]{\ensuremath{\lambda^{loc}}}
%% \newcommand{\lamadt}{\ensuremath{\lambda^{adt}}}
%% \newcommand{\lamcur}{\ensuremath{\lambda^{cur}}}

%% Proposal 1 - hey, we have capital lambda, and it's even the thing that binds
%% our lovely locations.
%% \newcommand{\ourcalc}[0]{\ensuremath{\Lambda^{loc}}}
%% \newcommand{\lamadt}{\ensuremath{\Lambda^{adt}}}
%% \newcommand{\lamcur}{\ensuremath{\Lambda^{cur}}}

% TODO: coming up with a new name.  RECONCILE usages with \ourcalc below.
% Ones using this macro have already been audited/reconciled.
\newcommand{\sysname}[0]{LoCal\xspace}

%% %% Proposal 2 - Core, like GHC Core.
% \newcommand{\ourcalc}[0]{\ensuremath{Core^{loc}}}

%% Helpers
\newcommand{\ourcalc}[0]{\sysname}
% \newcommand{\lamadt} [0]{\ensuremath{Core^{adt}}}
\newcommand{\lamadt} [0]{HiCal\xspace}
% \newcommand{\lamcur} [0]{\ensuremath{Core^{cur}}}
% \newcommand{\lamcur} [0]{\textsf{Cursored}}
% \newcommand{\lamcur} [0]{\textsf{CursedCal}}

\newcommand{\lamcur}[0]{NoCal\xspace}

\newcommand{\gramdef}{\; ::= \;}
\newcommand{\gramor}{\; | \;}
\newcommand{\keywd}[1]{\mathit{#1}}
\newcommand{\gramwd}[1]{\texttt{#1}}
\newcommand{\sgramwd}[1]{\texttt{#1}}
\newcommand{\skeywd}[1]{\mathit{#1}}

%% Grammar
\newcommand{\PROG}{\keywd{top}}
\newcommand{\DD}{\keywd{dd}}
\newcommand{\VD}{\keywd{vd}}
\newcommand{\FD}{\keywd{fd}}
\newcommand{\DC}{\keywd{K}}
\newcommand{\sDC}{\skeywd{K}}
\newcommand{\fields}{\skeywd{fe}}
\newcommand{\TC}{\keywd{T}}
\newcommand{\EXPR}{\keywd{e}}
\newcommand{\sEXPR}{\skeywd{e}}
\newcommand{\DATA}{\gramwd{data}}
\newcommand{\TYP}{\keywd{\tau}}
\newcommand{\hTYP}{\keywd{\hat{\tau}}}
\newcommand{\sTYP}{\skeywd{\tau}}
\newcommand{\var}{\svar}
\newcommand{\newVar}{y}
\newcommand{\svar}{x}
\newcommand{\fvar}{\sfvar}
\newcommand{\sfvar}{f}
\newcommand{\yvar}{y}
\newcommand{\fieldVar}{fl}
%\newcommand{\num}{n}
\newcommand{\ARROW}{\rightarrow}
\newcommand{\RP}{\keywd{dl}}
\newcommand{\sRP}{\skeywd{dl}}
\newcommand{\loc}{\skeywd{l}}
\newcommand{\sloc}{\skeywd{l}}
\newcommand{\concreteloc}[3]{\ensuremath{\langle #1, #2 \rangle ^{#3}}}
\newcommand{\reg}{\skeywd{r}}
\newcommand{\sreg}{\skeywd{r}}
\newcommand{\LS}{\keywd{ls}}
\newcommand{\LC}{\keywd{lc}}
\newcommand{\LE}{\keywd{le}}
\newcommand{\letpack}[3]{\gramwd{let}\;#1=#2\;\gramwd{in}\;#3}
\newcommand{\letloc}[3]{\gramwd{letloc}\;#1 = #2\;\gramwd{in}\;#3}
\newcommand{\letreg}[2]{\gramwd{letregion}\;#1\;\gramwd{in}\;#2}
\newcommand{\fapp}[2]{\fvar \;[#1]\; #2}
\newcommand{\fappnoloc}[1]{\fvar \; #1}
\newcommand{\TS}{\keywd{ts}}
\newcommand{\ssetbool}[4]{#4 = #3[#2\mapsto \keywd{#1}=\keywd{True}]}
\newcommand{\sinlinesetbool}[3]{#3[#2\mapsto \keywd{#1}=\keywd{True}]}
\newcommand{\CS}{\keywd{cs}}
\newcommand{\pat}{\keywd{pat}}

\newcommand{\copyPacked}[1]{(\gramwd{copyPacked}\; #1)}
\newcommand{\cpy}{\keywd{cpy}}
\newcommand{\copynoloc}[1]{\gramwd{copy} \; #1}

\newcommand{\ptr}[2]{(\gramwd{ptr}\;\keywd{#1}\;\keywd{#2})}
\newcommand{\sind}{i}
\newcommand{\ind}{\keywd{i}}
\newcommand{\indj}{\keywd{j}}
\newcommand{\VAL}{\keywd{v}}
\newcommand{\ec}{\keywd{\mathcal{E}}}
\newcommand{\evalc}[1]{\ec \llbracket #1 \rrbracket }
\newcommand{\STOR}{\keywd{S}}
\newcommand{\stepsto}{\Rightarrow}
\newcommand{\Name}{\Red{Name }}
\newcommand{\q}[1]{\texttt{#1}}
\newcommand{\frl}[1]{{\ensuremath \mathit{frl}(#1)}}
\newcommand{\caseclause}[2]{#1 \;\rightarrow \;#2}
\newcommand{\case}[2]{\gramwd{case}\; #1 \;\gramwd{of}\;#2}
\newcommand{\spat}{\keywd{spat}}
\newcommand{\switch}[2]{\gramwd{switch}\; #1 \;\gramwd{of}\;#2}
\newcommand{\readInt}[1]{\gramwd{\text{readInt}} \; #1}
\newcommand{\writeInt}[2]{\gramwd{\text{writeInt}} \; #1 \; #2}
\newcommand{\readTag}[1]{\gramwd{\text{readTag}} \; #1}
\newcommand{\writeTag}[2]{\gramwd{\text{writeTag}} \; #1 \; #2}
\newcommand{\readCursor}[1]{\gramwd{\text{readCursor}} \; #1}
\newcommand{\writeCursor}[2]{\gramwd{\text{writeCursor}} \; #1 \; #2}
\newcommand{\datacon}[3]{\ensuremath{#1 \;#2 \;#3}}
\newcommand{\dataconnoloc}[2]{\ensuremath{#1 \;#2}}
\newcommand{\litcon}[2]{\datacon{\keywd{L}}{#1}{#2}}
\newcommand{\litnum}{\keywd{n}}
\newcommand{\CP}{\keywd{cp}}
\newcommand{\tptr}[3]{\langle \mathit{ptr}\;#2\;#3 \rangle_{#1}}
\newcommand{\LM}{\keywd{M}}
\newcommand{\locis}[2]{\ensuremath{#1:#2}}
\newcommand{\lvar}{\keywd{lx}}
\newcommand{\has}[3]{\ensuremath{#1(#2) = #3}}
\newcommand{\startr}[1]{(\gramwd{start}\; #1)}
\newcommand{\afterl}[1]{(\gramwd{after}\; #1)}
\newcommand{\tightoverset}[2]{%
  \mathop{#2}\limits^{\vbox to -.5ex{\kern-0.75ex\hbox{$#1$}\vss}}}
\newcommand\set[1]{\{ \, \ensuremath{#1} \,\}}
\newcommand{\ecdot}{\bullet}
\newcommand{\heap}{\keywd{h}}
\newcommand{\alphaequiv}{=_{\alpha}}

%% Environments
\newcommand{\LENV}{\keywd{L}}
\newcommand{\RENV}{\keywd{R}}
\newcommand{\CENV}{\keywd{C}}
\newcommand{\TENV}{\keywd{\Gamma}}
\newcommand{\EENV}{\keywd{E}}
\newcommand{\SENV}{\keywd{\Sigma}}
\newcommand{\MENV}{\keywd{M}}
\newcommand{\FENV}{\keywd{F}}
\newcommand{\AENV}{\keywd{A}}
\newcommand{\NENV}{\keywd{N}}

%% Loc helpers
\newcommand{\inloc}[0]{\ensuremath{\downarrow\sloc}}
\newcommand{\outloc}[0]{\ensuremath{\uparrow\sloc}}
\newcommand{\locreg}[2]{\ensuremath{{#1}^{#2}}}
\newcommand{\tyatlocreg}[3]{#1 \ensuremath{@} \locreg{#2}{#3}}
\newcommand{\Cursorize}[0]{Cursorize}
\newcommand{\fresh}[0]{\keywd{fresh}}

%% Meta functions

% Takes FROM,TO, i.e. \subst{e}{x}{v}.
\newcommand{\subst}[3]{\ensuremath{#1[#3/#2]}}

\newcommand{\typeofcon}{\keywd{TypeOfCon}}
\newcommand{\typeoffield}{\keywd{TypeOfField}}
\newcommand{\kargtys}{\keywd{ArgTysOfConstructor}}
\newcommand{\allocptr}[2]{\keywd{MaxIdx}(#1,#2)}

% Update(M,key,val), e.g. M[key>val]
%\newcommand{\update}[3]{\ensuremath{((#2 \mapsto #3)\; #1)}}
\newcommand{\update}[3]{\ensuremath{#1+\{#2 \mapsto #3\}}}

\newcommand{\ewitness}[4]{\ensuremath{#1;#2;#3 \vdash_{ew} #4}}
\newcommand{\storewf}[6]{\ensuremath{#1;#2;#3;#4 \vdash_{wf} #5;#6}}
\newcommand{\storewfcfa}[3]{\ensuremath{#1 \vdash_{wf_{cfc}} #2;#3}}
\newcommand{\storewfca}[4]{\ensuremath{#1;#2 \vdash_{wf_{ca}} #3;#4}}

\newcommand{\tcfun}{\ensuremath{\vdash_{fun}}}
\newcommand{\tcpat}{\ensuremath{\vdash_{pat}}}
\newcommand{\tcts}{\ensuremath{\vdash_{ts}}}

%% Special references for proofs.
\newcommand{\refwellformed}[2]{WF~\ref{#1};\ref{#2}}
\newcommand{\refendwitness}[2]{EW~\ref{#1};\ref{#2}}
\newcommand{\refts}[1]{T-#1}
\newcommand{\refcase}[1]{Case-\ref{#1}}
\newcommand{\elimexists}[0]{$\exists$ elim}
\newcommand{\refinst}[0]{Inst.}

\newcommand{\tfunctiondef}{T-Function-Definition}
\newcommand{\tdatacon}{T-DataConstructor}
\newcommand{\ddatacon}{D-DataConstructor}
\newcommand{\dletloctag}{D-LetLoc-Tag}
\newcommand{\dletlocafter}{D-LetLoc-After}
\newcommand{\dletlocstart}{D-LetLoc-Start}
\newcommand{\dapp}{D-App}
\newcommand{\dletregion}{D-LetRegion}
\newcommand{\tcase}{T-Case}
\newcommand{\dcase}{D-Case}
\newcommand{\tpat}{T-Pattern}
\newcommand{\tprogram}{T-Program}
\newcommand{\tllafter}{T-LetLoc-After}
\newcommand{\tlltag}{T-LetLoc-Tag}
\newcommand{\tllstart}{T-LetLoc-Start}
\newcommand{\tlregion}{T-LetRegion}
\newcommand{\tvar}{T-Var}
\newcommand{\tlet}{T-Let}
\newcommand{\dletexp}{D-Let-Expr}
\newcommand{\dletval}{D-Let-Val}
\newcommand{\tapp}{T-App}
\newcommand{\tconcreteloc}{T-Concrete-Loc}

\newcommand{\emptytenv}{\emptyset}

%% Formatting

%% fdtools, harpoon are packages that provide this feature, but
%% have their own set of problems. We do this by hand instead:
%% https://tex.stackexchange.com/questions/304622
%% \makeatletter
%% \newcommand*\MY@rightharpoonupfill@{%
%%   \arrowfill@\relbar\relbar\rightharpoonup
%% }
%% \newcommand*\overrightharpoon{%
%%   \mathpalette{\overarrow@\MY@rightharpoonupfill@}%
%% }
%% \makeatother
\newcommand{\vectorize}[1]{\overline{#1}}
% \newcommand{\vectorize}[1]{\overrightharpoon{#1}}


\newcommand{\CFG}[0]{CFG\xspace}

\newcommand{\DFG}[0]{DFG\xspace}

\algnewcommand{\algorithmicswitch}{\textbf{switch}}
\algnewcommand{\algorithmiclet}[1]{\State \textbf{let} #1}
\algnewcommand{\algorithmicletmutable}[1]{\State \textbf{let mutable} #1}
\algnewcommand{\algorithmicmutate}[1]{\State \textbf{mutate} #1}
\algnewcommand{\algorithmicendlet}{\textbf{in}}
\algnewcommand{\algorithmiccase}{\textbf{case}}
\algnewcommand{\algorithmicendcase}{\State \textbf{end}}
\algnewcommand\algorithmicendswitch{\State \textbf{endswitch}}

% Define switch and case environments
\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{%
    \algorithmicswitch\ #1\ \algorithmicdo}{%
    \algorithmicend\ \algorithmicswitch%
}
\algdef{SE}[CASE]{Case}{EndCase}[1]{%
    \algorithmiccase\ #1}{%
    \algorithmicend\ \algorithmiccase%
}

\algnewcommand\Continue{\State \textbf{continue}}
\algblock{Input}{EndInput}
\algnotext{EndInput}
\algblock{Output}{EndOutput}
\algnotext{EndOutput}

\newcommand{\INDSTATE}[1][1]{\State\hspace{#1\algorithmicindent}}



==> design.tex <==
\section{Design}
\label{sec:design}

\system infers efficient layouts for dense representations of recursive
datatypes. \system's key idea is that the best data layout should match the way
a program accesses these data.
%
\secref{sec:overview} shows how this idea reduces to finding an
ordering of fields in data constructors. The ordering must align with the
order a function accesses those fields, in which case the optimization improves
performance of the function.

To find a better layout for a datatype in the single-function case, \system first analyzes possible executions of the function and their potential for field accesses. In particular, \system takes into account (a) the various paths through a function, each of which may access fields in a different order, and (b) dependencies between operations in the function, as in the absence of dependencies, the function can be rewritten to access fields in the original order, and that order will work best. \system thus constructs a control-flow graph (\secref{design:cfg}) and collects data-flow information (\secref{design:dfa}) to build a {\em field access graph}, a representation of the various possible orders in which a function might access fields (\secref{subsec:attributes} and \secref{design:fieldgraph}).

Once data accesses in a function are summarized in the field access graph, \system proceeds with synthesizing a data layout. \system incorporates knowledge about the benefits of sequential, strided access and the drawbacks of pointer chasing and backtracking to define an abstract cost model. The cost model allows to formulate an integer linear program whose optimal solution corresponds to a layout that minimizes the cost according to that model (\secref{design:genconstraints}).

The remainder of this section walks through this design in detail, and discusses how to extend the system to handle multiple functions that use a datatype (\secref{design:global}).

\subsection{\system's Language}
\system{} operates on the language \systemlang{} given in \figref{fig:grammar}.


\systemlang{} is a first-order, monomorphic, call-by-value functional language
with algebraic datatypes and pattern matching.
%
Programs consist of a series of datatype definitions, function definitions, and a main expression.
%
\systemlang{}'s expressions use A-normal form~\cite{ANF}.
%
The notation $\vectorize{x}$ denotes a vector $ [x_1, \ldots, x_n] $ and $\vectorize{x_{\ind}}$
the item at position $\ind$.
%
\systemlang{} is an intermediate representation (IR) used towards the front end in the Gibbon compiler.
The monomorphizer and specializer lower a program written in a polymorphic, higher-order subset of Haskell\footnote{With strict evaluation semantics using \il{-XStrict}.} to \systemlang{},
and then location inference is used to convert it to the {\em location calculus} (LoCal) code next~\cite{Local}.
%
It is easier to update the layout of types in \systemlang{} compared to LoCal,
as in \systemlang{} the layout is implicitly determined by the ordering of fields,
whereas the later LoCal IR makes the layout explicit using locations and regions (essentially, buffers and pointer arithmetic).

\begin{figure}[t]
	\small
	\input{formal_grammar2}
	\normalsize
        \caption{\new{Simplified grammar for a first-order, monomorphic functional language
            that \system operates on. \auditme{The full implementation includes more primitive datatypes, and built in primitives (such as a copy primitive).}}}
	%% \caption{Grammar definition of \system. This represents a
%%           point in compilation (1) with explicit locations, (2) after
%%           monomorphization. Functions are first order and the only
%%           remaining polymorphism is {\em location polymorphism}.}
	\label{fig:grammar}  
\end{figure}

%
% \csk{not sure if this phase ordering blurb is necessary...}
%
%In the remainder of this section, we describe the components of \system{}'s design in turn.

%
%% The remainder of this section is organized as follows, section~\ref{design:cfg} describes how we generate the control flow graph, section~\ref{design:fieldgraph} discusses how we generate the field access graph from the control flow graph,
%% {section~\ref{design:genconstraints} describes our cost model and how we obatain a minimum-cost ordering using
%% constraint solving.}
%% %% Section~\ref{design:genconstraints}, ~\ref{design:ilp} describe the constraint generation process and how we solve it using the ILP solver.
%% %% Finally, section~\ref{design:shufflefields} talks about the compiler pass that reorders the fields based on the locally optimal field ordering.

%% \note{RN: There's a lot of repetetion here. It might help to spell out the goal of each section in a small note at the top, and think through redundancy at that level.}

%% \subsection{Preliminaries}
%% \vs{Goal: Define all what a packed type is, what Algebraic data types are, fields, data constructors and grammar notation to make the user familiar with all the components of the analysis we are about to do. }
%% \begin{figure}[]
%% 	\begin{lstlisting}[ ]
	
%% 	data Tree a = Leaf a 
%% 	            | Node a (Tree a) (Tree a)
	
	

%% 	\end{lstlisting}
%% 	\caption{A packed data type in \system}
%% 	\label{lstlisting:packedtype}
%% \end{figure}

%% A \textit{packed type} (for example \textit{BlogList} in figure~\ref{fig:blog-traversal} and \textit{Tree} in figure~\ref{lstlisting:packedtype}) in \system is a data type whose values are serialized at contiguous addresses in memory.  As mentioned in the \secref{sec:overview}, the main motivation for such an in-memory serialization is to get the benefits of compactness, spatial locality and a predictable prefetch.
%% %
%% Still, where a traversal function doesn't touch all data, the compiler inserts necessary shortcut pointers (random access pointers) to different fields as required. This avoids generating dummy traversals.
%% \rn{Already covered...}

%% In the absence of such shortcut pointers, the traversal walks over unnecessary data by generating dummy traversals to reach the beginning of the desired location in the memory buffer. This doesn't preserve the asymptotic complexity of the program. Short cut pointers allow constant time access to data demanded by the function potentially ``out of the order'' it is serialized in memory. 

%% By matching the layout of the fields of a data type in memory to the traversal order of the function consuming it, 
%% we are optimizing the placement \textit{and} quantity of such shortcut pointers. At a high level, the layout of the data type should be such that it minimizes unnecessary {cursor} movement in the serialized buffer. This results in better locality and prefetching which enhances performance. Section~\ref{design:genconstraints} concretely defines such \textit{unnecessary movement} by encoding it in a cost model which is used to drive the layout optimization of the data type in memory. 

%% Defining a \textit{packed type} in \system can be done by using the keyword \textit{data} which allows the user to introduce data constructors to define the existence of different values that the packed type can take.
%% \rn{Definitely already covered!}
%% %
%% A packed type can have multiple such data constructors and each data constructor introduces different fields within itself which may be scalars or recursive fields.

%% Data constructors behave like function calls that take \textit{fields} of
%% some data {type variant as inputs and construct a value of that type}.
%% (Of course, any decent compiler open-codes the constructor primitives, not performing an actual runtime function call.)
%% %
%% We refer to scalar fields as primitive
%% types such as integers, floats and bools and non-scalar types are
%% \textit{packed} and potentially recursive fields.

%% \note{csk: specify that \system has 1-byte boolean values, but grammar doesn't include them for simplicity. can replicate booleans with case expressions of course.}
%% \note{csk: I've preserved the copy primitive in the grammar but it doesn't seem super relevant to marmoset.}

%% In our grammar, \figref{fig:grammar}, a data type of type $\tau$ is represented as $\DD$.  A data type can either be packed, unpacked, boxed or unboxed. However for our discussion, we assume its always \textit{packed and unboxed}. There can be multiple data constructors $\vectorize{\sDC}$ for a packed type $\DD$. Each data constructor $\sDC$ has some fields $\vectorize{\fields}$ of type $\vectorize{\sTYP}$ as shown in the grammar.

%% Given a program $\PROG$, it is constructed out of multiple data type declarations($\vectorize{\DD}$), functions($\vectorize{\FD}$) and expressions($\EXPR$). For a given program and function tuple $(\PROG, \FD)$ where the function $\FD$ consumes some data type $\DD$. We want to locally optimize the fields of the data constructors of $\DD$ for the function $\FD$. Hence for each data constructor $\sDC$ of the packed data type with fields $\vectorize{\fields}$ we want to find a total ordering on the fields of each data constructor such that it minimizes some costs and maximizes the performance of function $\FD$ that consumes the data type $\DD$.

%% \note{Need a discussion somewhere of how an entire program, with a control-flow graph of multiple functions, is handled.}

%% A programmer can write a program in \system using a subset of Haskell including polymorphic types. While compiling this language down to C, \system converts the higher-order, polymorphic language to a monomorphized intermediate representation with concrete types. There are a series of optimization passes including \lstinline{flatten} which flattens the intermediate representation and generated code in static single assignment, three address form. In order to find such an ordering, we analyze the function body of $\FD$ at the flattened level of the IR and gather the access patterns of the fields $\vectorize{\fields}$ for a data constructor $\sDC$ whose performance we are optimizing.

%% To orchestrate such an analysis, we construct a control flow graph for function $\FD$ after flattening the code in Gibbon's monomorphic IR\csk{edit due to grammar change.}\footnote{Called L1 in the implementation.}. We then use the control flow graph to construct a field access graph that captures the access patterns of the fields for a particular data constructor. Hence in our design, for a particular function, each data constructor $\sDC$ has an associated field access graph. This field access graph has the fields for that particular data constructor as vertices and directed edges between the vertices represent a temporal access between the two fields: {that is, both fields are accessed, and one is before the other.}

%% We use the field access graph to generate some constraints that we solve using an integer linear programming solver. The output of the solver is a mapping from the field to its locally optimal index in the data constructor that minimizes the costs when traversal $\FD$ traverses the data type.
  



% \begin{figure}[H]
% 		\begin{subfigure}[a]{\linewidth}
% 		\fontsize{10pt}{10pt}\selectfont
% 		\begin{flalign*}
% 	    	&\text{scalar types }  \ \  \epsilon  \ \  \text{\textbf{int} | \textbf{float} | \textbf{bool} | \textbf{char} }&\\
% 	    	&\text{non-scalar types } \ \  \epsilon  \ \  \text{\textbf{Vector (scalar types)} } &\\
% 	    	&\text{packed types} \ \  \epsilon \ \  
% 		\end{flalign*}
% 		\caption{Types in \system}
% 		\end{subfigure}
% \caption{Language definition of \system}
% \end{figure}

\subsection{Control-Flow Analysis}
\label{design:cfg}

%% \vs{Goal: Define how the control flow graph is build and its components / assumptions etc. }

\begin{algorithm}
    \caption{Control-Flow Graph Psuedocode}\label{alg:cfg}
    \begin{algorithmic}[1]
		\small
		\Input 
			\State exp: An expression in subset of \systemlang
			\State weight: The likelyhood of exp executing (\ie{} exp's inbound edge)
%			\State nodeId: A variable to track the id of cfg nodes
		\EndInput
		\Output
			\State A tuple of list of cfg nodes and the node id.
		\EndOutput
        \Function{ControlFlowGraph}{exp, weight}
            \algorithmiclet{nodeId = genFreshId()}
            \Switch{$exp$}
                \Case{LetE (v, ty, rhs) bod} \label{alg:cfg-let} 
					\algorithmiclet{(nodes, succId) = \Call{ControlFlowGraph}{bod, weight}}
					\algorithmiclet{newNode = (nodeId, (LetRHS (v, ty, rhs), weight), [succId])} \label{alg:cfg-likelihood}
					\State \Return (nodes ++ newNode, nodeId)
                \EndCase
%%                 \Case{IfE a b c} \label{alg:cfg-if}
%% 					\algorithmiclet{(n1, succB) = \Call{ControlFlowGraph}{b, weight/2}}
%% 					\algorithmiclet{(n2, succC) = \Call{ControlFlowGraph}{c, weight/2}}
%% 					\algorithmiclet{newNode = (nodeId, (a, weight), [succB, succC])}
%% 					\State \Return (n1 ++ n2 ++ [newNode], nodeId)
%%                \EndCase
				\Case{CaseE scrt cases} \label{alg:cfg-case}
					\algorithmiclet{(nodes, successors) = \Call{CfgCase}{weight/length(cases), cases}}
					\algorithmiclet{newNode = (nodeId, (scrt, weight), successors)}
					\State \Return (nodes ++ [newNode], nodeId)
				\EndCase
                \Case{VarE v}
                                        \algorithmiclet{newNode = (nodeId, (v, weight), [])}
					\State \Return ([newNode], nodeId)
                \EndCase
            \EndSwitch
        \EndFunction
    \end{algorithmic}
\end{algorithm}

%
We construct a control-flow graph with sub-expressions, and let-bound RHS's (right hand sides) of \systemlang{} as the nodes.
Algorithm~\ref{alg:cfg} shows the psuedocode for generating the control-flow graph.
%
\new{Because the syntax is flattened into A-normal form, there is no need to traverse within the RHS of a let expression.}
%
Edges between the nodes represent paths between expressions. The edges consist of {\em weights} (Line~\ref{alg:cfg-likelihood})
that represent the likelihood of a particular path being taken.
%%
%% csk: addressed
%% \rn{Not totally comfortable with calling this instruction
%%   level... since the ``instructions'' are arbitrary
%%   primitive-applications in the AST. It's not close to *machine*
%%   instruction level.}
%%   In this instruction-level control flow graph, each node is an instruction in three address form and edges exists between two nodes in the order of the execution of the program. The order of execution branches at \textit{if then else} instructions and \textit{case} instructions. For an \textit{if then else} condition, the order of execution branches in two different directions. For a case expression it branches $n$-ways, where $n$ is the number of different patterns that need to be matched for that particular case expression.
%
%% For this reason, we do not construct a traditional control-flow graph from the intermediate language but rather generate an instruction level control flow graph using the \textit{Data.Graph} library available with the \textit{containers} package in Haskell.
%Given a function definition, each sub-expression of the function body becomes a separate node in the \CFG.
An edge between two nodes indicates the order of the evaluation of the program.
%
% \footnote{The order of evaluation is straightforward to determine since \systemlang{} uses call-by-value semantics.}.
A node corresponding to a \il{let}-binding (Line~\ref{alg:cfg-let}) contains the bound expression
and has one outgoing edge to a node corresponding to the body expression.
%
A \il{case} expression (Line~\ref{alg:cfg-case}) splits the control flow $n$-ways,
where $n$ is the number of pattern matches.
{Outgoing edges of a node for a \il{case} expression have weights
  associated with them that correspond to the likelihood of taking a
  particular branch in the program.}
%% The likelihood parameter is threaded while generating the control flow graph, for the \textit{if then else} instruction since the control flow forks, the likelihood of each child edge becomes half, (\textit{likelihood of parent `div` 2} ). Similarly for a case instruction, each child's likelihood is assumed to be uniformly distributed for each of the possible match clauses.
%
%\mv{huh? why bring this up if we don't use the weights?}
%\ap{we now talk about it in the discussion, so let's skip it here}
% If available, dynamic profiling information can provide these weights.
% For the purposes of this paper, however, we find it is sufficient to use trivial placeholder weights: i.e. uniform weight over all branches.
% A node for a pattern match clause merely has an outgoing edge to its body expression.
%
Control flow terminates on a leaf \systemlang{} expression: a variable reference,
a data constructor or a function application.
% , for instance, either a data constructor, a function application, or a variable reference.

%% We plan to use dynamic techniques like profiling to calculate the actual frequency a particular path will be taken by the program at runtime. This depends on the input to the program.
%In the current implementation, a function call {\em does not} correspond to an edge to the callee's
%body in the \CFG, since \system{} only analyses one function at a time.
%
%In the future, we plan to extend our work to perform interprocedural analysis.
%
%\auditme{However, in the whole-program compilation setting (where types are already specialized and monomorphic), non-recursive functions can very often be inlined yielding a data traversal as a single recursive function.}

%
%\rn{This seems like a painful restriction to not extend the analysis across functions....}

\Figref{graph:running-cfg} shows the control-flow graph for the running example (\figref{fig:blog-traversal}).
%\new{(This example uses an \lstinline|if| expression, which is trivially desugared to \lstinline|case|.)}
%
{Each node corresponds to a sub-expression of the function \il{emphKeyword}.
%
The first \il{case} expression splits the control flow into two branches,
corresponding to whether the input list of blogs is empty or not.
%
The branch corresponding to the empty input list is assigned a probability $\alpha$, and
the other branch is assigned a probability $1 - \alpha$.
%
The next node corresponds to the pattern match \il{Blog content hashTags blogs'}.
%
Another two-way branch follows, corresponding to whether \il{keyword} occurs in
the \il{content} of this blog or not.
%
We assign the probabilities $\sigma$ and $1-\sigma$ to these branches respectively.
%
Note that as a result, the corresponding edges in the CFG have weights $(1 - \alpha)*\sigma$ and $(1 - \alpha)*(1 - \sigma)$, as the likelihood of {\em reaching} that condition is $(1 - \alpha)$.
%
Each of these branches terminate by creating a new blog entry with its content potentially updated.
%
In the current model, $\alpha$ and $\sigma$ are 0.5: they are uniformly distributed.
}
%

\auditme{One intuition for why realistic branch weights are not essential to \system's optimization is that accurate weights only matter if there is a trade off between control-flow paths that are best served by different layouts. The base cases (e.g. empty list) typically contribute {\em no} ordering constraints, and in our experience, traversals tend to have a preferred order per function, rather than tradeoffs intra-function, which would reward having accurate, profile-driven branch probabilities. Hence, for now, we use uniform weights even when looking at the intra-function optimization.}
%\mv{This is kinda confusing. I get the argument for why weights aren't that important to us right now, but the paper just spent some time setting up these weights just to argue that we don't need them. Could we move this discussion to future work?}
%\mk{I sort of agree, but I don't want to do too much restructuring of this portion of the paper this late in the game.}

%% Here each vertex corresponds to a top level instruction in the body of traversal~\ref{fig:blog-traversal}. Each path along the control flow graph has a corresponding probability of that path being taken as shown in figure~\ref{graph:running-cfg}. As mentioned, currently in our model the probabilities $\alpha$ and $\sigma$ are uniformly distributed. (In our example, $\alpha$ and $\sigma$ are 0.5)


%\vs{todo: add an example of a cfg here (use running example)}

\begin{figure}[t]
    \centering
    \captionsetup[subfigure]{justification=centering}
\begin{subfigure}[]{0.699\textwidth}
    \centering
  \includegraphics[scale=0.34]{figures/runningCFG}
  \caption{CFG with probability of executing along each path.}
  \label{graph:running-cfg}
\end{subfigure}
\begin{subfigure}[]{0.29\textwidth}
    \centering
  \includegraphics[scale=0.20]{figures/access-graph-running}
  \caption{Field-access graph $G$ generated from control-flow graph.
     Here we use field types to uniquely name them, since Haskell 
     record syntax was not used in this example to give each field a name.}
  \label{graph:running-access}
\end{subfigure}
\caption{Control-flow and corresponding field access graphs generated for the running example.}
\end{figure}
%\ap{TODO: the graphs go on the margins -- we should fix it. E.g. there is space now to put them back side by side}}


\subsection{Data Flow Analysis}
\label{design:dfa}

%\vs{Section Goal: Define why we need the data flow analysis and a quick summary of how we do it in the compiler.}

We implement a straightforward analysis (use-def chain, and def-use chain) for \lstinline|let| expressions to capture dependencies between 
\lstinline|let| expressions. We use this dependence information to form dataflow edges in the field access graph (\secref{design:fieldgraph})
and to subsequently optimize the layout and code of the traversal for performance. For \textit{independent} \lstinline|let| expressions in the function we are optimizing, we can transform the function body to have these let expressions in a different order. 
(Independent implies that there are no data dependencies between such \lstinline|let| expressions. Changing the order of independent \lstinline|let| expressions will
not affect the correctness of
% [non-crashing]
code, modulo exceptions.)
%\rn{Nontermination should be the same irrespective of let-binding order... we could swap nontermination and a panic as long as we have a partial language though... we reserve the right to do that?}
%
However, we do such a transformation only when we deem it to be more cost efficient. In order to determine 
when re-ordering \lstinline|let| expressions is more cost efficient, we classify fields based on specific attributes next.

\subsection{Field Attributes For Code Motion}
\label{subsec:attributes}

%% \vs{Section Goal: what are these attributes and how will they help getting a lost cost ordering. }

When trying to find the best layout, we may treat the code as immutable,
but allowing ourselves to move the code around (i.e. change the order of accesses to the fields)
unlocks more possibilities for optimizing layout.
Not all code motions are valid due to data dependencies in the traversal.
For instance, in a sequence of two \lstinline|let| binders, the second one may reference the binding introduced in the first one: in this case, the two binders cannot be reordered.

To decide which code motions are allowed, we classify each field with one or more of the attributes: \textit{recursive, scalar, self-recursive}, or \textit{inlineable}.
%
% Artem: the following needs a separate paragraph
% As there is a dependence between attributes, it may be possible to inherit multiple sub-attributes from a single attribute.
Some of these attributes are derived from the ADT definition and some from the code using the ADT.
%
A \emph{scalar} field refers to a datatype only made up of either other primitive types, such as \lstinline|Int|.
%
A \emph{recursive} field refers to a datatype defined recursively.
%the values constituting the field contain one or more recursive fields.
% \rn{Reword this --- fields have a type, but fields don't directly consist of other fields so this sounds a bit odd.}
%
A \emph{self-recursive} field is a recursive field that directly refers back to the datatype being defined (such as a \lstinline|List| directly referencing itself).
% similar to recursive fields but they are self-recursive since they contain fields that are the same type 
%% for instance the \lstinline|List| data type 
%% \begin{lstlisting}
%% data List = Nil | Cons Int List
%% \end{lstlisting}
%% Here \lstinline|List| is a recursive and a self-recursive field.
% \textit{Inlineable fields:}
Finally, we call a field \emph{inlineable} if the function being optimized makes a recursive call into this field \new{(i.e.\ taking the field value as an argument)}.
Hence, an inlineable field is necessarily a recursive field.
As we show in the example below, the inlineable attribute is especially important when choosing whether or not to do code motion.
%A field has this attribute based on the scope (that is, how it is used in a function.)
%In the running example, the \lstinline|BlogList| field is an inlineable field.

% For each function in the program, we introduce a new metadata field that stores the \new{attributes for all fields of all data constrcuctors used in that function.}
%% , for each data constructor, a mapping from each field index to all the possible attributes we can deduce about that particular field.
%
A single field can have multiple attributes.
For instance, a function \lstinline|traverse| doing a pre-order traversal on a \lstinline|Tree| makes recursive calls on both the
left and right children. The left and right children are recursive and self-recursive. Therefore, when looking at the scope of 
traverse, the left and right children have the attributes recursive, self-recursive and inlineable. 
%\vs Trying to talk about why having such attributes is helpful}

% Table to show the performance difference between List and List' 
% \ifx\ExtendedVersion\undefined
% \else
\begin{table}[t]
    \centering
    \caption{Running times for two traversals working with their corresponding matching layouts.}
    \begin{tabular}{ccc}
    \toprule
    datatype / traversal & \lstinline|List| / \lstinline|foo| & \lstinline|List'| / \lstinline|foo'| \\
    \midrule
    {1M elements} & 0.992s & 0.953s \\
    \bottomrule
    \end{tabular}
    \label{table:list-power}
\end{table}
%\fi

\begin{figure}[]
\centering
\begin{subfigure}{.5\textwidth}
    \centering
\begin{lstlisting}
  foo :: List -> List
  foo lst = case lst of
   Nil -> Nil
   Cons x rst ->
     let x' = x ^ 100
         rst' = foo rst
      in Cons x' rst'
\end{lstlisting}
\caption{Function \lstinline|foo| with \lstinline|List|.}
\label{fig:foo}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
    \centering
\begin{lstlisting}
  foo' :: List' -> List'
  foo' lst = case lst of
   Nil' -> Nil'
   Cons' rst x ->
     let rst' = foo' rst
         x' = x ^ 100
      in Cons' rst' x'
\end{lstlisting}
\caption{Function \lstinline|foo'| with \lstinline|List'|.}
\label{fig:foo'}
\end{subfigure}
\caption{Two different traversals on a list.}
\label{fig:two-diff-traversals}
\end{figure}

\textbf{Example.}
Consider the example of a list traversal shown in Figure~\ref{fig:foo}.
%
%We modify the \lstinline|List| type to contain a recursive field rather than an \lstinline|Int| to show an appreciable performance difference. 
%However, the core idea would be the same if the field were to be an \lstinline|Int| instead. 
%
%
%
Here the function \lstinline|foo| does some work on the \lstinline|Int| field (it raises the \lstinline|Int| to the power of 100) and then recurs on the tail of the list.
%
Since \system compiles to dense representations, a \lstinline|List|'s representation
in memory stores the \lstinline|Cons| tag (one byte) followed by the \lstinline|Int| (8 bytes) followed by
the next \lstinline|Cons| tag and so on. Hence, the \lstinline|Cons| tag and the \lstinline|Int| field are interleaved together in memory.
%
The function \lstinline|foo| becomes a stream processor that consumes one stream in memory and produces a dense output buffer of the same type.

Alternatively, another layout of a list follows from the following definition:
\begin{lstlisting}
  data List' = Nil' | Cons' List' Int
\end{lstlisting}
%
In memory, the list has all \lstinline|Cons'| tags next to each other \new{(a unary encoding of array length!)} and the \lstinline|Int| elements all next to each other.
%
In such a scenario, the performance of our traversal \lstinline|foo| on the \lstinline|List'| can improve 
% is a function of the work per element done and the size of the element field.
% 
%% As the work done on the element field increases or the length of the 
%% field itself increases, the cost to traverse the field reduces in the second representation because fields are packed next to each other.
traversal performance due to locality when accessing elements stored side-by-side\footnote{However, this effect can disappear if the elements are very large or the amount of work done per element becomes high, such that the percent of time loading the data is amortized.}.
%
However, this only works if we
can subsequently change the function that traverses the list to do recursion on the tail of the list first and then call the exponentiation
function on the \lstinline|Int| field after the recursive call. If there are no data dependencies between the recursive call and the exponentiation
function, then this is straightforward. We show \lstinline|foo'| with the required code motion transformation to function \lstinline|foo| accompanied
with the change in the data representation from \lstinline|List| to \lstinline|List'| as shown in Figure~\ref{fig:foo'}.

%% \rn{We also kill tail recursion! I don't think we can let that go by without mention... Our new function must have available stack space equal to list length. The original ``foo'' isn't tail recursive in the original sense either, but Gibbon can make it so because of how the prefix of the data constructor can be written BEFORE the recursion.}	     


				
% Consider the code snipped below, where we unroll the list and the recursive call to show what Inlining the recursive call looks like. Here we unroll the list to length 3 and call doWork 3 times. Although we have inlined the recursion, the data represenation is still interleaved, that is, the Integers are not packed next to each other as nicely as they would be in the List' representation of the List.
% With the foo' and List' representation, we are making all the recusive calls and then doing work on the Integers, albeit in the reverse order, However this still results in a friendlier memory access and runtime performance.

% \begin{lstlisting}
% foo :: List -> List 
% foo lst = case lst of 
% 	Nil -> Nil 
% 	Cons1 r1 Cons2 r2 Cons3 r3 ... rst -> 
% 	 let r1' = doWork r1 
% 	     r2' = doWork r2 
% 	     r3' = doWork r3 
%          .... 
%          rst ' = foo rst
%        in Cons r1' Cons r2' Cons r3' ... rst' 
% \end{lstlisting}

To optimize the layout, the tail of the list is assigned the attribute of inlineable. This attribute is used by the solver to
determine a least-cost ordering to the \lstinline|List| datatype in the scope of function \lstinline|foo|. 
Whenever such code motion is possible, \system will place the inlineable field first and use code-motion to change
the body of the function to perform recursion first if data flow dependencies allow such a transformation. 

% \ifx\ExtendedVersion\undefined
%\else
In fact, we made a similar program and ran \system on the program in the hope that it would be able to optimize the program by placing the inlineable
field first and use code-motion to change the traversal. We show the results in table~\ref{table:list-power}. We see a speedup of 4.1\% 
over our baseline datatype and traversal.
%\fi

\textbf{Structure of arrays.}
The transformation of
\lstinline|List|/\lstinline|foo| to \lstinline|List'|/\lstinline|foo'|
is similar to
%inlining the recursive call and
changing the representation of the \lstinline|List| datatype to a
\textit{structure of arrays}, which causes the same types of values to be next to each other in memory.
In particular, we switch from alternating constructor tags and integer values in memory to
an array of constructor tags followed by an array of integers.

Note that the traversals \lstinline|foo| and \lstinline|foo'| have access
patterns that are completely aligned with the data layout of \lstinline|List| and \lstinline|List'| respectively. The resulting speedup 
is solely a consequence of the \textit{structure of arrays} effect. This is an added benefit to the runtime in addition to ensuring that the 
access patterns of a traversal are aligned with the data layout of the datatype it traverses.

% Artem: we already considered the simpler example of List. Let's do the Blog example if we have space

% In the traversal from figure~\ref{fig:blog-traversal},
% the \lstinline|HashTags| field induces a data dependence through the \lstinline|if| statement caused by the call
% to \lstinline|search|. For that reason, we cannot change the code that causes the access to the \lstinline|HashTags|
% field. However, in the \lstinline|then| branch, the let expressions that cause the access to the content and tail of
% the list are not bound by any data dependence. We cannot move them out of the \lstinline|then| branch because of the
% data dependence from \lstinline|HashTags|, however, within the \lstinline|then| branch we can re-order the let expressions
% that access the content and the tail of the list respectively.

% For the running \lstinline|Blog| example, \system chooses
% a layout where \lstinline|HashTags| is followed by the tail pointer \lstinline|BlogList| and \lstinline|Content| respectively.
% \begin{lstlisting}
%     data BlogList = Nil | Blog HashTags BlogList Content
% \end{lstlisting}
% The traversal also changes such that the recursive call to the tail of the list \lstinline|BlogList| occurs first, followed by the call to emphasize
% the \lstinline|Content| in the \lstinline|then| branch. This layout and traversal transformation provides the best performance.

\subsection{Field Access Pattern Analysis}
\label{design:fieldgraph}

\begin{algorithm}[t]
        \caption{Recursive function for generating the field access graph}\label{alg:field-access-graph}
        \begin{algorithmic}[1]
            \small
            \Input
                \State cur: current CFG node from which to start processing
                \State dcon: data constructor for which we are searching the best layout
                \State edges: field-access graph built so far
                \State lastAccessedVar: last accessed variable name, initially None
                \State dfgMap: set of data-flow edges between variables
            \EndInput
            \Output
                \State Field access graph represented as a list of edges
                % \State \lsstinline|data Edge| = \lstinline|DfgEdge| ((var:\lstinline|String|, var:\lstinline|String|), likelihood:\lstinline|Int|)
                % \State             | \lstinline|CfgEdge| ((var:\lstinline|String|, var:\lstinline|String|), likelihood:\lstinline|Int|)
            \EndOutput
            \Function{FieldAccessGraph}{cur, dcon, edges, lastAccessedVar, dfgMap}

                \algorithmiclet{((expr, weight), successors) = cur} \label{line-likelihood-example}
                %\algorithmicletmutable{isFirstAccess = true}
                \algorithmicletmutable{lastAccessedVarMut = lastAccessedVar}
				\algorithmicletmutable{edges\textquotesingle = edges}
                \For{var : \Call{OrderedFreeVariables}{expr}} \label{line:lastAccessedVar-start}
                    \If{!\Call{BoundInPatternMatchOnDcon}{var, dcon}} \label{line:boundInDcon}
						\Continue
					\EndIf
                        \If{lastAccessedVarMut != None}
							\algorithmicmutate{edges\textquotesingle = \Call{addEdge}{edges\textquotesingle, ((lastAccessedVar, var), weight), ControlFlowTag}}\label{line:cfg-edge}
                            \If{\Call{lookup}{(lastAccessedVar, var), dfgMap}}
                                \algorithmicmutate{edges\textquotesingle = \Call{addEdge}{edges\textquotesingle, ((lastAccessedVar, var), weight), DataFlowTag}}\label{line:dfg-edge}
                            \EndIf
                        \EndIf
                        \algorithmicmutate{lastAccessedVarMut = var}
                \EndFor \label{line:lastAccessedVar-end}
                
                \For{succ : successors} \label{line:succ-rec-start}
                    \algorithmiclet{edges\textquotesingle\textquotesingle = \Call{FieldAccessGraph}{succ, dcon, edges\textquotesingle, lastAccessedVarMut, dfgMap}}
                    \algorithmicmutate{edges\textquotesingle = \Call{merge}{edges\textquotesingle, edges\textquotesingle\textquotesingle}}
                \EndFor \label{line:succ-rec-end}

                \State \Return edges\textquotesingle

            \EndFunction

            % \Function{AccessGraphDriver}{cfgMap, dfgMap, functions}
                
            %     \State letMutable accessGraphMap = newEmptyMap
            %     \For{funcName : functions}
            %         \State let dconsInFunc = \Call{getDataConstructors}{funcName}
            %         \State let funcCfg = \Call{Map.lookup}{cfgMap, funcName}
            %         \State let cfgRoot = \Call{getCfgRoot}{funcCfg}
            %         \State let funcDfg = \Call{Map.lookup}{dfgMap, funcName}
            %         \For{dcon : dconsInFunc}
            %             \State let edges = \Call{AccessGraph}{None, cfgRoot, dcon, [], None, funcDfg}
            %             \State \Call{Map.insert}{accessGraphMap, (funcName, dcon), edges}
            %         \EndFor
            %     \EndFor
            %     \State \Return accessGraphMap
            % \EndFunction

            % \Function{AddEdge}{edgeList, edge}
            %     \State let reversedEdge = \Call{reversedAccessEdge}{edge}
            %     \If{!\Call{exists}{reversedEdge, edgeList}}
            %         \State \Call{append}{edgeList, edge}
            %     \EndIf
            % \EndFunction
        \end{algorithmic}
    \end{algorithm}


After constructing the \CFG and \DFG for a function definition, we utilize them to inspect the type
of each of the function's input parameters---one data constructor at a time---and construct
a \emph{field-access graph} for it.
Algorithm~\ref{alg:field-access-graph} shows the psuedocode for generating the field-access graph. 
%
This graph represents the temporal ordering of accesses among its fields.

The fields of the data constructor form the nodes of this graph.
%
A directed edge from field $f_i$ to field $f_j$ is added if $f_i$ is accessed immediately before $f_j$. Lines~\ref{line:lastAccessedVar-start} to ~\ref{line:lastAccessedVar-end}
in Algorithm~\ref{alg:field-access-graph} show how we keep track of the last accessed field and form an edge if possible. 
A directed edge can be of two different types. In addition, each edge has a associated weight which indicates the likelihood of accessing $f_i$ before $f_j$, which is computed using the \CFG.
An edge can either be a data-flow edge or a control-flow edge (Lines~\ref{line:cfg-edge} and ~\ref{line:dfg-edge}). In \Figref{graph:running-access}, the red edge is a data flow edge and the blue edge is a control flow edge.

\textit{Data-Flow Edge} indicates an access resulting from a data flow dependence between the fields $f_i$ and $f_j$. In our source language, a data flow edge is induced by
% either an \lstinline|if| conditional or
a \lstinline|case| expression.
A data flow edge implies that the code that represents the access is rigid in structure and changing it can make our transformation invalid.

\textit{Control-Flow Edge} indicates an access that is not data-flow dependent. It is caused by the control flow of the program. Such an edge does not induce strict constraints on the code that induces the edge. The code is malleable in case of such accesses. This gives way to an optimization search space via code motion of \lstinline|let| expressions. The optimization search space involves transformation of the source code, i.e, changing the access patterns at the source code level.
%The transformation is possible because there is no data dependence that prevents changing the order of access between the fields. 
%
%% %
%% Branching in the \CFG leads to three possible scenarios of field accesses:
%% \begin{itemize}
%% \item todo.
%% \end{itemize}

%% \csk{stopped writing here.}

%% Loosely similar to Chilimbi~\etal~\cite{CSD, CSL, ccgarbage} we construct what we formally call a \textit{field access} graph (subsequently referred to as $G$) that captures the static temporal access patterns of the fields for a particular data constructor. Hence, in our current model, we store such a $G$ for a unique quadruple $(\PROG, \FD, \DD, \sDC)$. The graph $G(V, E)$ is a weighted directed graph where each vertex  $v \epsilon V$ is a field($\fields$) from the fields($\vectorize{\fields}$) of a data constructor($\sDC$). Each edge $e \epsilon E$ represents an access between two fields.

%% For now, we locally optimize the ordering of the fields ($\vectorize{\fields}$) of a data constructor $\sDC$ for a packed type $\DD$. The objective of the ordering problem is to match the data layout of each data constructor $\sDC$, that is, the layout of all fields $\vectorize{\fields} \epsilon \sDC$ to the
%% access patterns of the traversal $\FD$ operating on the fields of the data constructor.

%% To be able to match the data layout of a value constructor $\sDC$ in memory to the traversal order of the function whose performance we are optimizing (Such a function and the corresponding data type to be optimized is annotated by the user while writing the top level program) we need to have information about the temporal access patterns of each field in the data constructor.

%% There have been prior works that solve a similar problem~\cite{CSD, CSL, ccgarbage} but they are designed to work with imperative programming languages like \textit{C and C++}. In addition, the problem there is concerned with optimizing the memory layout of boxed data structures that are not statically and readily packed in memory like with \system.
 
The field-access graph $G$ is a directed graph, which consists of edges of the two types between fields of a datatype and can have cycles. The directed nature of the edges enforces a temporal relation between the corresponding fields. More concretely, assume that an edge $e$ that connects two vertices representing fields $\fields_{a}$ (source of $e$) and $\fields_{b}$ (target of $e$). We interpret $e$ as an evidence that field $\fields_{a}$ is accessed before field $\fields_{b}$. The weight $w$ for the edge $e$ is the probability that this access will happen based on statically analyzing a function. % $\FD$.

In our analysis, for a unique path through the traversal, we only account for the {\em first} access to any two fields. If two fields are accessed in a different order later on, the assumption is that the start address of the fields is likely to be in cache and hence it does not incur an expensive fetch call to memory. In fact, we tested our hypothesis by artificially making an example where say field $f_{a}$ is accessed first, field $f_{b}$ is accessed after $f_{a}$ after which we constructed multiple artificial access edges from $f_{b}$ to $f_{a}$, which might seem to suggest placing $f_{b}$ before $f_{a}$. However, once the cache got warmed up and the start addresses of $f_{a}$ and $f_{b}$ are already in cache, the layout did not matter as much. This suggests that prioritizing for the first access edge between two unique fields along a unique path is sufficient for our analysis.

Two fields can be accessed in a different order along different paths through a traversal. This results in two edges between the fields. (The edges are in reversed order.) We allow at most two edges between any two vertices with the constraint that they have to be in the opposite direction and come from different paths in the traversal. If two fields are accessed in the same order along different paths in the traversal, we simply add the probabilities and merge the edges since they are in the same direction.

In order to construct $G$, we topologically sort the control-flow graph of a function %$\FD$
and traverse it in the depth-first fashion via recursion on the successors of the current cfg node (Lines~\ref{line:succ-rec-start} to~\ref{line:succ-rec-end}).
%
As shown in line~\ref{line:boundInDcon}, we check if a variable is an alias to a field in the data
constructor for which we are constructing the field-access graph $G$.
%
As we process each node (i.e. a primitive expression such as a single
function call), we update the graph for any direct or indirect
references to input fields that we can detect.
%
We ignore new variable bindings that refer to newly allocated rather
than input data---they are not tracked in the access graph.
%
%% For the current node being processed in the control flow graph, ,
%% % i.e, instruction,
%% we back track each input variable to figure out if it is an alias to
%
%% Since we are in a functional programming paradigm, we restrict this
%% analysis for variables introduced in a \textit{case} binding or
%% function arguments since we assume that variables that are written
%% to are allocated in a fresh memory location. Hence, accesses to
%% newly written fields do not optimize the in memory layout of the
%% data constructor that is being read and is input to the traversal.
%
\auditme{We traverse the control-flow graph once, but we maintain the
  last-accessed information at each CFG node, so when we process a field
  access at an expression, we consult what was previously-accessed at
  the unique precedecessor of the current CFG node.}
%
\Figref{graph:running-access} shows the generated access graph from the control-flow graph in \figref{graph:running-cfg}. It also shows the probability along each edge obtained from the control-flow graph.

%% For each such variable which originates from one of the fields of the data constructor in scope, we traverse all the successor nodes in the control flow graph to see is there are any other fields that are accessed in the successor nodes. For the fields that are accessed, we add a directed edge from the current field to the successor field/s. We recursively do this for all the successors and terminate when we have completely traversed the graph in topological order.
%% \rn{This makes it sound like we do a bunch of repeated traversals -- traversing the downstream graph every time we have an access.}

As we are traversing the nodes of the control-flow graph and generating directed edges in $G$, we use the likelihood of accessing that cfg node as the weight parameter (Line~\ref{line-likelihood-example}).
%As mentioned previously, we can get more precise weights by dynamically profiling the traversal at runtime to obtain the frequency of taking a particular path through the traversal.
%However, for now, we restrict ourselves to static weights.

% \begin{figure}[]
%   \includegraphics[scale=0.45]{figures/access-graph-running}
%   \caption{Field access graph $G$ generated from \CFG of running
%     example~\ref{graph:running-cfg}.  Here we use field types to
%     uniquely name them, since Haskell record syntax was not used in
%     this example to give each field a name.}
%   \label{graph:running-access}
% \end{figure}

\subsection{Finding a Layout}
\label{design:genconstraints}

%% \vs{Goal: define how the constraints are generated from the access pattern graph. That is, the cost model and all its components.}

% \rn{This paragraph was pretty repetitive:}
%% The field access graph for a value constructor in the ADT captures the access patterns of the fields in the value constructor by statically analyzing the traversal $\FD$ that consumes the ADT. The access paths of the fields induce concrete edges in the access pattern graph $G$. These edges are directed in nature and hence signify a temporal access pattern between the fields making up the edge. Each edge in the access pattern graph has an associated weight which is calculated statically for now.

We use the field-access graph $G$ to encode the problem of finding a better layout as an Integer Linear Program (ILP). Solving the problem yields a cost-optimal field order for the given pair of a data constructor and a function.

\subsubsection{ILP Constraints}
In our encoding, each field in the data constructor is represented by a variable, $f_0, f_1, \dots$ As a part of the result, each variable will be assigned a unique integer in the interval $[0, n -1]$, where $n$ is the number of fields. Intuitively, each variable represents an index in the sequence of fields.

The ILP uses several forms of constraints, including two forms of \emph{hard} constraints:
%
\begin{gather}
  \forall_{0 \leq i < n}  \qquad 0 \leqslant f_{i}  < n \label{eq:valid}\\
  \forall_{0 \leq i < j < n} \qquad f_i \neq f_j   \label{eq:uniq}
\end{gather}
%
The constraints of form~\ref{eq:valid} ensure that each field is mapped to a valid index, while the constraints of form~\ref{eq:uniq} ensure that each field has a unique index.
Constraints of either form must hold because each field must be in a valid location.

Hard constraints define valid field orderings but not all such reorderings improve efficiency, \system's main goal.
%
To fulfil the goal, beside the hard constraints we introduce {\em soft} ones. Soft constraints come from the field access analysis. For example, assume that based on the access pattern of a function, we would {\em prefer} that field $a$ goes before field $b$. We turn such a wish into a constraint. If the constraint cannot be satisfied, it will not break the correctness. In other words, such constraints can be broken, and that is why we call them soft.

\subsubsection{Cost Model}
\system encodes these soft constraints in the form of an abstract cost model that assigns a cost to a given layout (assignment of fields to positions) based on how efficient it is expected to be given the field-access graph.

To understand the intuition behind the cost model, note that the existence of an edge from field $f_i$ to field $f_j$ in the field-access graph means that there exists at least one path in the control-flow graph where $f_i$ is accessed and $f_j$ is the next field of the data constructor that is accessed.
%
In other words, the existence of such an edge implies a preference {\em for that control-flow path} for field $f_i$ to be immediately before field $f_j$ in the layout so that the program can continue a linear scan through the packed buffer.
%
Failing that, it would be preferable for $f_j$ to be ``ahead'' of $f_i$ in the layout so the program does not have to backtrack in the buffer.
%
We can thus consider the costs of the different layout possibilities of $f_i$ and $f_j$:

\begin{description}
	\item[$C_{\mathit{succ}}$] ($f_j$ immediately after $f_i$): This is the best case scenario: the program traverses $f_i$ and then uses $f_j$.
	\item[$C_{\mathit{after}}$] ($f_j$ after $f_i$ in the buffer): If $f_j$ is after $f_i$, but not {\em immediately} after, then the code can proceed without backtracking through the buffer, but the intervening data means that either a shortcut pointer or a \new{extra traversal} must be used to reach $f_j$, adding overhead.
	\item[$C_{\mathit{pred}}$] ($f_j$ immediately before $f_i$): Here, $f_j$ is {\em earlier} than $f_i$ in the buffer. Thus, the program will have already skipped past $f_j$, and some backtracking will be necessary to reach it. This incurs {\em two} sources of overhead: skipping past $f_j$ in the first place, and then backtracking to reach it again.
	\item[$C_{\mathit{before}}$] ($f_j$ before $f_i$ in the buffer): If, instead, $f_j$ is farther back in the buffer than $f_i$, then the cost of skipping back and forth is greater: in addition to the costs of pointer dereferencing, because the fields are far apart in the buffer, it is less likely $f_j$ will have remained in cache (due to poorer spatial locality).
\end{description}

We note a few things. 
%
First, the {\em exact} values of each of these costs are hard to predict. 
%
The exact penalty a program would pay for jumping ahead or backtracking depends on a variety of factors such as cache sizes, number of registers, cache line sizes, etc.
%
%Second, one could imagine a more fine-grained cost model that distinguishes between, say, fields that are a constant distance apart versus those that have some other recursive (and hence potentially large) field between them.
%
%However, the inexact nature of the cost model means that this would be false precision.
%
%Instead, \system uses an abstract cost model with reasonably-chosen values satisfying the following:

However, we use our best intuition to statically predict these costs based on the previously generated access graph.
Note the existence of two types of edges in our access graph. An edge can either be a data-flow edge or a control-flow edge.
For a data flow edge, the code is rigid. Hence the only axis we have available for transformation is the datatype itself. For a data flow edge, the costs are showed in Eq~\ref{eq:costs-strong-edge}. Here, we must respect the access patterns in the original code which lead to the costs in Eq~\ref{eq:costs-strong-edge}.
%
\begin{equation}
C_{\mathit{succ}} < C_\mathit{after} < C_\mathit{pred} < C_\mathit{before}
\label{eq:costs-strong-edge}
\end{equation}

Note that a control-flow edge signifies that the direction of access for an edge is transformable. We could reverse the access in the code without breaking the correctness of the code. We need to make a more \textit{fine-grained} choice.
This choice involves looking at the attributes of the fields and making a judgement about the costs given we know the attributes of the fields. As shown in Sec~\ref{subsec:attributes} we would like to have the field with an \textit{inlineable} attribute placed first.
Hence, in our cost model, if $f_i$ is inlineable, then we follow the same costs in Eq~\ref{eq:costs-strong-edge}. However, if $f_j$ is inlineable and $f_i$ is not, we would like $f_j$ to be placed before $f_i$. For such a layout to endure, the costs should change to Eq~\ref{eq:costs-inlineable}.
For other permutations of the attributes, we use costs that prioritize placing the inlineable field/s first. 
\begin{equation}
C_\mathit{pred} < C_\mathit{before} < C_{\mathit{succ}} < C_\mathit{after}
\label{eq:costs-inlineable}
\end{equation}


\subsubsection{Assigning Costs to Edges}

\system uses the field-access graph and the cost model to construct an objective function for the ILP problem.
%
Each edge in the access graph represents one pair of field accesses with a preferred order. Thus, for each edge $e = (i, j)$, \system can use the indices of the fields $f_i$ and $f_j$ to assign a cost, $c_e$, to that pair of accesses following the rules below.
\begin{table}[h]
\centering
\begin{tabular}{ll}
If $f_j$ is right after $f_i$, then assign cost $C_\mathit{succ}$, i.e.:
&
$
(f_j - f_i) = \phantom{-}1 \implies c_e = C_\mathit{succ}
$.
\\
%
If $f_j$ is farther ahead of $f_i$, then assign cost $C_\mathit{after}$, i.e.:
&
$
(f_j - f_i) > \phantom{-}1 \implies c_e = C_\mathit{after}
$.
\\
%
If $f_j$ is immediately {\em before} $f_i$, then assign cost $C_\mathit{pred}$, i.e.:
&
$
(f_j - f_i) = -1 \implies c_e = C_\mathit{pred}
$.
\\
%
And if $f_j$ is farther before $f_i$, then assign cost $C_\mathit{before}$, i.e.:
&
$
(f_j - f_i) < -1 \implies c_e = C_\mathit{before}
$.
\end{tabular}
\end{table}

The cost of each edge, $c_e$ must be multiplied by the {\em likelihood} of that edge being exercised, $p_e$, which is also captured by edge weights in the field-access graph. Combining these gives us a total estimated cost for any particular field layout:
%
\begin{equation}
C = \sum_{e \in E} c_e \cdot p_e
\label{eq:objective}
\end{equation}
%
This is the cost that our ILP attempts to minimize, subject to the hard constraints~\ref{eq:valid} and~\ref{eq:uniq}.

\subsubsection{Greedy layout ordering}

\new{
Finding an optimal layout using an external solver hurts compile times.
To solve this tradeoff, we propose a simple algorithm that traverses the field access graph in a \emph{greedy} fashion.
The algorithm starts from the root node of the graph, which corresponds to the field accessed first in the function, and greedily visits the child nodes based on the edge weights.
}
We fix the edge order for a control-flow edge as the original order and do not look at field attributes. However, after the greedy algorithm picks a layout we match the let expressions to the layout order to make sure the code matches the layout order. The greedy algorithm is potentially sub-optimal when it comes to finding the best performing layout; however, the compile time is fast.

%Since there is a tradeoff in compile-times and run-times we wanted to ensure that we have a backend with a fast compile time in case compile time becomes a bottleneck.  

\subsection{Finding a global layout}
\label{design:global}

A data constructor can be used across multiple functions, therefore, we need to find a layout order that is optimal globally.
To do so, we take constraints for each function and data constructor pair and combine them uniformly, that is, a uniform weight for each function.
%\footnote{Dynamic profiling techniques can be used to get more precise weights, but we leave such efforts for future work.}.
We then feed the combined constraints to the solver to get a globally optimal layout for that data constructor. The global optimization finds a globally optimal layout for all data constructors in the program. Once the new global layout is chosen for a data constructor, we re-write the 
entire program such that each data constructor uses the optimized order of fields.
In the evaluation, we use the global optimization. However, we only show the data constructor that constitutes the major part of the program.

\subsection{Finding a layout for functions with conflicting access patterns}
\label{design:conflicting-access-patterns}
Consider the datatype definition \lstinline|D| with two fields \lstinline|A, B|:
\begin{lstlisting}
    data D = D A B
\end{lstlisting}
If two functions, \lstinline|f1| and \lstinline|f2|, access the fields of \lstinline|D| in the opposite orders,
we get conflicting access patterns for \lstinline|D|.
For instance, assume \lstinline|f1| accesses \lstinline|A| first and then \lstinline|B|, while \lstinline|f2|
accesses \lstinline|B| first and then \lstinline|A|. After combining edges across the two functions, we get two edges
in opposition to each other. Since we use uniform weights for all functions, the edges will also have a uniform weight.
As a result,
placing \lstinline|A| before \lstinline|B| or vice versa are equally good in our
cost model, and \system defers to the solver to get one of the two layouts.

\new{
With the two equally good layouts, \system's solver (the default mode) chooses the layout favoring the function it picked first. For instance, if \lstinline|f1| is defined earlier in the program, the order favoring \lstinline|f1| will be picked.
%
In the greedy mode, since both \lstinline|A| and \lstinline|B| are root nodes, \system will pick the
first root node in the list of root nodes, which is, again, dependent on the ordering of functions in the source code.
%
% If we determined that \lstinline|f2| has a greater weight than \lstinline|f1|, then the layout preferred by \lstinline|f2| would be chosen. % Artem: leaving hypoteticals to the discussion section
}

%Based on the relative positions of the two fields (in memory) making up an edge, the edge in the graph can take four different cost values
%% that we unfold in detail
%in our cost model.
%
%The objective of the ILP formulation is to minimize the sum of weighted costs for all the edges where the weight is the corresponding likelihood along each edge in the graph. 
%First we provide some definitions to describe our integer linear program. 
%
%\[ M = \text{The ILP model} \]
%\[ \sDC = \text{data constructor whose field order is being optimized} \]
%\[ n \equiv |\vectorize{\fields}| = \text{ total number of vertices in the graph G} \]
%\[ m = \text{ total number of edges in the graph G} \]
%\[ f_{1}, f_{2}, ... f_{n} \epsilon \vectorize{\fields}= \text{index variables for each field in $\sDC$} \]
%\[ c_{1}, c_{2}, ... c_{m} = \text{cost variables for edges }  e_{1}, e_{2} ... e_{m} \epsilon E \]
%\[ l_{1}, l_{2} ... l_{m} = \text{likelihood values for edges } e_{1}, e_{2} ... e_{m} \epsilon E \]
%
%\subsubsection*{Defining cost:}
% Let us assume the presence of a temporal access between two fields $f_1$ and $f_2$ in a function $\FD$ (assuming $f_1$ dominates $f_2$ in $G$). 
%Let us take a closer look at the time window when traversal $\FD$ has consumed field $f_1$ and is about to access field $f_2$. 
%
%There are two possibilities that can arise depending on how the fields $f_1$ and $f_2$ are laid out in the packed buffer. If field $f_2$ is serialized some fields after field $f_1$ {\em nonconsecutively}, then the traversal $\FD$ has to perform a \textit{forward pointer dereference} to get to field $f_2$.  On the other hand, if field $f_2$ is serialized before $f_1$ then the traversal has to \textit{backtrack} or do a \textit{backward jump} to get to field $f_2$.
%%
%\auditme{When moving forward, the size of the jump could be zero bytes (if the fields are consecutive), or an amount that depends on the size of what is skipped over (constant or variable).  Constant jumps are most efficient because they can be computed at compile time based on the ending byte of field $f_1$.}
%%
%%% \auditme{For the remainder of this paper we simply {\bf ignore fields with constant size (scalars)}. We leave them out of the analysis, and let the Gibbon compiler backend place them where it wants (which is currently directly after the tag byte identifying the data constructor).}
%\rn{TODO: make the above commented bit true...}
%
%In practice, for a forward pointer dereference, the packed representation provides the presence of a \textit{RAN} pointer (random access pointer or shortcut pointer) that the traversal can dereference to jump to the address $f_2$ is serialized at. For a backtrack, the traversal $\FD$ needs to know how to get to the start address of field $f_2$ in the packed buffer. This can be achieved by generating extra traversals over the packed buffer or storing the start address of $f_2$ as yet another \textit{RAN} pointer, \new{but the present Gibbon compiler infrastructure prefers the latter}.
%
%\begin{itemize}
%  \item \textit{forward pointer dereference:} The packed representation of the ADT provides the presence of a pointer which can be dereferenced to reach the location of the desired field we want to access. We store the cost of this pointer dereference as some \textit{p} in our model $M$.
%
%  \item \textit{backtrack or backward jump: } The function $\FD$ must rewind in the packed buffer to reach the start of the desired field. We store the cost of such a backward jump by function $\FD$ as \textit{b}. 
%\end{itemize}
%
%
%In our model $M$, we assign a cost for each edge $e$ based on the relative positions of fields $f_{i}$ and $f_{j}$. Let us assume this cost to be $c_{k}$; the cost $c_{k}$ can take four different values based on the relative positions of $f_{i}$ and $f_{j}$. These costs are constants known statically. These are derived based on the relative positions of the fields which induces a cost \textit{p} or \textit{b} or some combination of the two. These costs are shown below. The details of these costs are defined later on as we shall see. Currently in our model $M$, the costs \textit{p} and \textit{b} are assumed to be the same.
%
%\[ C_{1}, C_{2}, C_{3}, C_{4} \epsilon \mathbb{W} = \text{constant costs known statically, at compile time} \]
%
%\begin{equation}
%\centering
%C_{1} < C_{2} < C_{3} < C_{4}
%\tag{Cost relation}
%\label{eqn:constant-costs}
%\end{equation}
%
%Now that we have some definitions, we can generate some constraints for our model $M$. For an edge $e \epsilon E$ with an associated cost $c_{k}$ in the graph $G$, suppose fields $\fields_{i}$  and $\fields_{j}$ (represented by model variables $f_{i}$ and $f_{j}$ moving forward)  participate in that edge. Moreover, for the directed edge e, let $f_{i}$ dominate $f_{j}$ which implies that field $f_{i}$ is accessed prior to field $f_{j}$ along the path that goes through edge e in the graph $G$. We introduce four constraints (implications) for edge $e$ based on relative positions of $f_{i}$ and $f_{j}$ in the packed buffer. 
%
%The \textit{lhs} of the implication computes the difference of indices of the two fields (this emulates their relative position in memory) and the \textit{rhs} gives a cost based on the relative position. The following equations~\cref{eqn:imp1,eqn:imp2,eqn:imp3,eqn:imp4} define the constraints for an edge $e$ and we have these for each edge $e \epsilon E$.
%
%
%\begin{equation}
%\label{eqn:imp1}
%(f_{i} - f_{j}) =  -1  \Rightarrow (c_{k} = C_{1})      
%\tag{constr 1}
%\end{equation}
%
%\textit{If} fields $f_{i}$ and $f_{j}$ are right next to each other such that $f_{i}$ is to the left of field $f_{j}$ then such an arrangement induces an insignificant cost $C_{1}$ for the edge $e$. This is because the directed edge $e$ is interpreted as a temporal access from $f_{i}$ to $f_{j}$. A traversal that needs to access 
%$f_{i}$ right before $f_{j}$ would incur the least cost if $f_{i}$ was serialized right before $f_{j}$ in the packed buffer.
%
%\begin{equation}
%\label{eqn:imp2}
%(f_{i} - f_{j}) < -1  \Rightarrow (c_{k} = C_{2})  
%\tag{constr 2}
%\end{equation}
%
%\textit{If} field $f_{i}$ is to the left of $f_{j}$ and there are $t$ number of fields between them (where $t$ > 0) then the temporal access given by edge $e$ induces a cost $C_{2}$. The cost $C_{2}$ is greater that cost $C_{1}$ on account of the extra $t$ fields present between $f_{i}$ and $f_{j}$. In such a packed representation of the two fields, in order for a traversal to get from field $f_{i}$ to $f_{j}$ it needs to either forward jump or walk(using a dummy traversal) over the $t$ fields. This is the cost \textit{p} mentioned earlier. (in practice, \system provides a pointer to the starting address of field $f_{2}$)
%
%\begin{equation}
%\label{eqn:imp3}
%(f_{i} - f_{j}) =  1  \Rightarrow (c_{k} = C_{3})
%\tag{constr 3}
%\end{equation}
%
%\textit{If} fields $f_{i}$ and $f_{j}$ are right next to each other and $f_{i}$ is to the right of $f_{j}$ in the packed buffer, then, the edge $e$ induces a cost $C_{3}$ satisfying~\ref{eqn:constant-costs}.
%This cost is greater than $C_{1}$ and $C_{2}$. This is because in order for a traversal to first access $f_{i}$ in the packed buffer, it has to jump over the field $f_{j}$ serialized before it and then rewind (\textit{backtrack}) in the buffer to be able to access field $f_{j}$ again. This means that the traversal not only has to incur a cost of a forward pointer dereference but also incur an extra cost of a backtrack. Hence total cost is \textit{p + b}.
%
%\begin{equation}
%\label{eqn:imp4}  
%(f_{i} - f_{j}) >  1  \Rightarrow (c_{k} = C_{4})  
%\tag{constr 4}
%\end{equation}
%
%\textit{If} field $f_{i}$ is to the right of field $f_{j}$ and there are $t$ fields in between them in the packed representation (where $t$ > 0), then, the edge $e$ induces a cost $C_{4}$ which is the most expensive cost in our model $M$. Traversing such a packed buffer requires first a forward jump over $t$ fields to reach field $f_{i}$ and then backtrack to reach the start of field $f_{j}$. This is more costly than implication~\ref{eqn:imp3} since the traversal has to potentially jump across larger addresses in memory (especially if there is a recursive field in between). Such a jump will exhibit worse spatial locality. We can represent this cost as greater than implication~\ref{eqn:imp3} by multiplying it by a constant factor (i.e., \textit{c*(p + b)}, for some constant c). 
%
%
%The ILP model $M$ is a minimization problem where we solve for the optimal indices of the fields $\vectorize{\fields}$ such that it minimizes the total weighted costs along all the edges in the graph $G$. The weights are simply the likelihoods along each edge in the graph $G$ which are constants known statically.
%
%\begin{equation}
%\label{eqn:objective}
%\tag{obj. function}
%\min_{c} \sum_{i=1}^{m}{l_{i}*c_{i}}    % \equiv l_{1}*c_{1} + l_{2}*c_{2}...+ l_{k}*c_{k}...l_{m} * c_{m}
%\end{equation}
%%% \vs{true, without the eqiv looks neater.}
%%% \mv{Do we need the part after the $\equiv$? The reader will understand the summation without it being spelled out.}
%
%The exact values of the constant costs $C_{1}, C_{2}, C_{3}, C_{4}$ are not calculated using a clever algorithm as of the moment. In the future, we could use a heuristic which can reason about these costs by analyzing the type signature of the fields $f_{i}$ and $f_{j}$ and whether they are recursive or non nrecursive fields.
%%% This information is trivial to obtain and the compiler can tell it to us statically.\mv{Maybe be careful with claims like this, that we don't do something but it would totally be easy to do if we wanted to.}
%
%However, the more \textit{fine-grained} we make our cost analysis, the more time it will take for a solver to solve it.
%%% \mv{Are we in danger of this time being very long?} \vs{I have some solver times in the eval, they look reasonable i think. Figure 7.}
%%
%In the definition of the ILP model $M$, equation~\ref{eqn:constant-costs} needs to be satisfied. Note that equation~\ref{eqn:constant-costs} is not part of the constraints in the actual model $M$ but something that is known and satisfied before the model $M$ is invoked.
%
%%Each of the implications~\cref{eqn:imp1,eqn:imp2,eqn:imp3,eqn:imp4} relates the relative position of two fields participating in the edge $e$ with the associated cost if that relative position was to be satisfied in the model $M$. Before giving a rationale behind each implication, we define what we exactly mean by costs. 
%
%%\subsubsection*{Define costs: }
% 
%%Let us assume the presence of a temporal access between two fields $f_1$ and $f_2$(assuming $f_1$ dominates $f_2$ in $G$) in a function $\FD$. 
%%Let us take a closer look at the time window when traversal $\FD$ has consumed field $f_1$ and is about to access field $f_2$.
%%There are two types of costs that can arise depending on how the fields $f_1$ and $f_2$ are laid out in the packed buffer. If field $f_2$ is serialized some fields after field $f_1$(not next to each other), then the traversal $\FD$ has to perform a \textit{pointer dereference} to get to field $f_2$.  On the other hand, if field $f_2$ is serialized before $f_1$ then the traversal needs to \textit{backtrack} inside the packed buffer to get to field $f_2$.  
%%In practice, for a pointer dereference, the packed representation provides the presence of an shortcut pointer after the end of field $f_1$ so that the traversal can jump to the address $f_2$ is serialized at. 
%%For a backtrack, the traversal $\FD$ must be written in such a way that it can effectively traverse back to field $f_2$ in the packed buffer. In practice, this is can be achieved by generating extra traversals over the packed buffer.  
%
%%\begin{itemize}
%%  \item \textit{pointer dereference:} The packed representation of the ADT provides the presence of a pointer which can be dereferenced to reach the location of the desired field we want to access. We store the cost of this pointer dereference as some \textit{p} in our model $M$.
%
%%  \item \textit{backtracking: } The function $\FD$ must unwind in the packed buffer to reach the desired field. In practice, this can be achieved by generating extra traversals over the packed buffer. We store the cost of such a backtrack by function $\FD$ as \textit{b}. 
%%\end{itemize}
%
%%Currently in our model $M$, both the costs \textit{p} and \textit{b} are assumed to be the same. Below we give the rationale for each implication in detail.
%
%Using all the constraints described above, the model should minimize the weighted sum of the costs along each edge in the graph $G$. This is shown mathematically with equation~\ref{eqn:objective}. 

\section{Implementation}\label{sec:impl}

We implement \system{} in the open-source Gibbon compiler\footnote{https://github.com/iu-parfunc/gibbon/}.
Figure~\ref{figure:overall-pipeline} gives an overview of the overall pipeline. 
%
Gibbon is a whole-program micropass compiler that compiles a polymorphic,
higher-order subset of (strict) Haskell.

\begin{figure}[]
	\includegraphics[scale=0.4]{figures/OverallPipeline2}
	\caption{The overall pipeline of \system.}
	\label{figure:overall-pipeline}
\end{figure}
%
The Gibbon front-end uses standard whole-program compilation and monomorphization techniques~\cite{urweb-icfp}
to lower input programs into a first-order, monomorphic IR (\systemlang{}).
%
Gibbon performs location inference on this IR to convert it into a LoCal program,
which has regions and locations, essentially, buffers and pointer arithmetic.
%
Then a big middle section of the compiler is a series of LoCal $\rightarrow$ LoCal compiler passes that
perform various transformations.
%
Finally, it generates C code.
%\csk{perhaps this paragraph is unnecessary, but we don't say much about gibbon anywhere else.}
Our extension operates towards the front-end of the compiler, on \systemlang{}.
%
We closely follow the design described in Section~\ref{sec:design} to construct the
control-flow graph and field-access graph, and use the standard Haskell graph library\footnote{https://hackage.haskell.org/package/containers} in our implementation.

To solve the constraints, we use IBM's DOCPLEX (Decision Optimization CPLEX),
because its API allows high level modelling such as logical expressions like implications, negations, logical AND etc. with relatively low overhead. 
%
%% via its Python bindings
Unfortunately, there isn't a readily available Haskell library that can interface with DOCPLEX.
%
Thus, we use it via its library bindings available for Python.
%
Specifically, we generate a Python program that feeds the constraints to DOCPLEX and
outputs an optimum field ordering to the standard output,
which \system{} reads and parses, and then reorders the fields accordingly.
%
% The field ordering is output as a list of tuples, \il{[(Int, Int)]},
% where the first component is the original field index and the second component
% is that field's new index.

%% %
%% In the remainder of this section we outline 

% \mv{Do you need an implementation section, or can you just explain the implementation in the design section?}

% %% \subsection{Using an ILP solver to solve the generated constraints}
% \subsection{Solving Cost Model Constraints}
% \label{design:ilp}

% %% \vs{ILP solver.}

% We construct the field access graph and ILP (integer linear program) as detailed in Section~\ref{sec:design}. The abstract cost model works with four costs, subject to the constraints in Equation~\ref{eq:costs}. Because every term of the objective function (Equation~\ref{eq:objective}) is a multiple of one of these costs, the only thing that matters is the relative values of the costs, not their absolute value. Hence, we use a ratio of 1:2:3:4 for $C_\mathit{succ}$, $C_\mathit{after}$, $C_\mathit{pred}$ and $C_\mathit{before}$, respectively in case of a data flow edge. In case of a control flow edge, it depends on the attribute of the fields but the costs are integral multiples of each other. 

% \new{After constructing the ILP,
% we use a commercially available ILP solver, CPLEX~\cite{cplex},
% to obtain a minimum-cost ordering.}
% %% generated the constraints using the access graph $G$, we can directly generate code for these constraints targeted for a commercially available ILP solver.
% %
% The logical constraints described in section~\ref{design:genconstraints} cannot directly be given as an input to CPLEX.
% %% in a trivial ILP solver.
% %% However, we there are various known techniques to linearize these logical expressions to work with 
% %% %% work for a vanilla ILP solver.
% %% We show the linearized versions of these constraints in the appendix of our extended paper. 
% %
% To solve these constraints, we use IBM's DOCPLEX (Decision Optimization CPLEX),
% because its API allows high level modelling such as logical expressions like implications, negations, logical AND etc. with relatively low overhead. 
% %
% %% via its Python bindings
% Unfortunately, there isn't a readily available Haskell library that can interface with DOCPLEX.
% %
% Thus, we use it via its library bindings available for Python.
% %
% Specifically, we generate a Python program that feeds the constraints to DOCPLEX and
% outputs an optimum field ordering to the standard output,
% which \system{} reads and parses, and then reorders the fields accordingly.
% %
% The field ordering is output as a list of tuples, \il{[(Int, Int)]},
% where the first component is the original field index and the second component
% is that field's new index.

%% we use a staging compiler that uses the \textit{language-python} library in haskell to automatically generate python code for IBM's DO (decision optimization) CPLEX~\cite{cplex} library. 
%% %
%% We specifically use DOCPLEX since its object oriented API allows high level modelling (such as logical expressions like implications, negations, logical AND etc.) with relatively low overhead. 
%% %
%% The DOCPLEX solver gives us a mapping from the old fields of the data constructor to the new index positions in the data constructor that locally optimize the performance of traversal $\FD$. We use this index map to re-order the fields in the data constructor and repair the code which we talk about next.   

% \subsection{Reordering Fields of a Datatype}
% \label{design:shufflefields}

% Once we obtain an optimum field ordering for a specific data constructor globally, we update that data constructor to have this new field order.
% %
% %% The ILP solver returns the new field ordering for the data constructor and function pair we are trying to locally optimize the program for. We use this field order to change the instantiated order of fields of the corresponding data constructor ($\sDC$) of value type $T$.
% Consequently, we need to repair the complete program to adhere to the updated data constructor.

%% A
%% % \textit{L1}
%% compiler pass, operating on the \systemlang{} IR, uses the optimal field ordering to permute the fields of the data constructor $d$ and modifies its type $T'$. We then recursively traverse each function and permute the case bindings and all expressions where the data constructor $\sDC$ is being written to so that the program type checks. Doing so ensures that we generate correct code. Performing this transformation
%% % at the \textit{L1} level
%% early in the compiler
%% is beneficial since downstream compiler passes like \textit{inferLocations}
%%   (which does the major work of converting to location calculus)
%% are able to implement the serialized data operations just as if the
%% programmer had writen the desired the data layout in the original source code of their program.
%% %% correctly reason about the region and location calculus as if the programmer instantiated the correct layout at the top level.
%% % \mv{This sentence is likely to not be understood by a reader unfamiliar with LoCal.}

% % \subsection{Using annotation pragmas to allow the user to specify various constraints over the fields of a data constructor.}
% \subsection{Annotation Pragmas for Optional, Manual Ordering Constraints}
% \label{sec:annotation-pragmas}
% %% \vs{Annotation pramas to give the user control to define the layout of fields + different kinds of constraints and how contraints are generated for the them.}
% %


% % -- User requsets the compiler optimize the Cons constructor
% % -- based on the access patters of fields in traversal foo.
% % {-# ANN foo Cons #-}

% \begin{figure}% [H]
% 	\begin{lstlisting}[]
       
%                 -- User defines some absolute constraints as assignments of field indices.
% 		{-# ANN Cons (foo, (0 ~> 3, 1 ~> 2)) #-}    
		
% 		-- User defines some relative (``after'') constraints.
% 		{-# ANN Cons (foo, (4 :> 5, 3 :> 2)) #-}
		
% 		data List = Nil | Cons F0 F1 F2 F3 F4 F5 List

% 		foo :: List -> List 
% 		foo lst = case lst of 
% 		                Cons f1 f2 f3 f4 f5 f6 rst -> ...

% 	\end{lstlisting}
% 	\caption{User annotations in \system to define constraints over fields of a data constructor. The annotations are defined as ANN annotations for a specific function and data constructor that function uses. }
% 	\label{fig:userAnnotations}
% \end{figure}

% Optional, manual control over data layout has uses beyond second guessing the automatic optimizer.
% %% Allowing users to specify constraints over the layout of fields in a data constructor is a useful capability. This allows the user to match the layout of the data constructor to certain specifications they may have.
% %
% For instance, the user may wish to store the data in a certain format on disk or provide information for ordering that may affect performance downstream for reasons the user has information about. In addition, the user may want to read existing data in a certain format residing on disk. We allow the user to specify the layout of fields in \system through annotations (pragmas). Currently, our compiler allows these specifications to be defined for a specific function and data constructor[s].
% %% However, we plan to extent our model to specify these constraints for multiple functions and even globally across functions.
% %
% We allow the user to specify two kinds of constraints over the fields of a data constructor. These are shown in figure~\ref{fig:userAnnotations}. 

% \begin{itemize}
% \item \textbf{Absolute Constraints:} These constraints allow the user to specify an exact position for a field in a data constructor. The \textit{ANN} annotation names a specific data constructor, a function name, and a list of field (indices) as well as their assigned positions.
% % $Cons (foo, (0 \sim~> 3))$ says to   
% %%   contains the data constructor to be optimized and the tuple contains the function name followed by the ordering specified in the inner tuple. The ordering in the nested (inner) tuple uses a special infix operator ``$\sim>$'' to determine the new index position for the field in the index on the left hand side of the infix operator.
%   Hence $0 \sim> 3$ in the ANN annotation assigns the field at position $0$ to position $3$ in the data constructor. This is parsed by the compiler and added as metadata in the function body
%   % of the function the ordering is defined for.
%  The constraint solver honors these constraints, while freely moving around the other fields.
% For example, $0 \sim> 3$ will generate the following constraints in the constraint solver :  ${F0}_{index} = 3$

% \item \textbf{Relative Constraints:} These constraints allow the user to specify the relative ordering of fields in a data constructor. Currently we support ``Immediately After'' constraints but these can be extended to other types of relative constraints in the future. Immediately After constraints allow the user to place one field right after another one. For instance, ``$4 :> 5$'' can be interpreted as placing field at index position $4$ right after the field at index position $5$. Such a specification by the user will generate the following constraint in the constraint solver : ${F4}_{index} = {F5}_{index} + 1$ for the example shown in figure~\ref{fig:userAnnotations}.

% % \item \textbf{Activating optimization:}
% % \item \textbf{Optimization Hints:}
% %   \new{The user can specifically invoke \system on a particular combination of function and data constructor(s).
% % %
% %     This is a hint from \system to process the function, and may be subsumed by future strategies that automatically apply (and cache solver results for) the optimization.
% % %
% %  In any case, the performance optimization search previously described
% %  will always respect any other hard constraints that have been
% %  annotated.}
  
% % \item \textbf{Soft Constraints (automatic performance optimization):}
% % 
% %% The user can specify the automatic layout optimization for performance using yet another ANN annotation pragma shown in figure~\ref{fig:userAnnotations}. This instructs \system to perform the automatic optimization for a specific function and data constructor that we have already discussed. We call these generated constraints defined in section~\ref{design:genconstraints} as ``soft constraints''. They are called soft since they do not impose a strict ordering as would be by the absolute and relative constraints but is rather driven by the costs induced by the access patterns of the traversal. These constraints would essentially take a back seat if the user has defined a stricter constraint for a field used in the function body. However, these can work in tandem with the strict orderings(if provided) to better optimize the layout for the traversal. In the absence of user specified relative and absolute orderings, \system will optimize the layout for performance as discussed before.

% \end{itemize}




==> discussion.tex <==
\section{Future Work}
\label{sec:discussion}

\system could allow the user to provide optional constraints on the layout
(either relative or absolute) through pragmas.
A relative constraint would allow the user to specify if a field \lstinline|A| comes immediately after
field \lstinline|B|. An absolute constraint would specify an exact index in the layout for a field.
Such pragmas may be useful if the user requires a specific configuration of a data
type for external reasons or has information about performance bottlenecks.


Although the performance optimization is currently statically driven, there are many avenues for future
improvement. For instance, we can get better edges weights for the access graphs
using dynamic profiling techniques. The profiling can be quite detailed, for
instance, which branch in a function is more likely, which function takes the
most time overall in a global setting (the optimization would bias the layout
towards that function), how does a particular global layout affect the
performance in case of a pipeline of functions.

We could also look at a scenario where we optimize each function locally and 
use ``shim'' functions that copy one layout to another (the one required by the
next function in the pipeline). Although the cost of copying may be high, it warrants
further investigation. Areas of improvement purely on the implementation side include 
optimizing whether \system dereferences a pointer to get to a field or uses the end-witness
information as mentioned in section~\ref{sec:overview}. Lesser pointer dereferencing 
can lower instruction counts and impact performance positively. We would also like to 
optimize the solver times as mentioned in~\ref{subsec:heuristic-tradeoffs}.

We envision that the \textit{structure of arrays} effect that we discovered may help 
with optimizations such as vectorization, where the performance can benefit significantly
if the same datatype is close together in memory. Regardless, through the case studies, we see 
that \system shows promise in optimizing the layout of datatypes and may open up 
the optimization space for other complex optimizations such as vectorization.


==> editingmarks.tex <==

% \usepackage[usenames,dvipsnames]{xcolor}
% \usepackage[dvipsnames]{xcolor}
\usepackage[]{xcolor}

% [2024.05.20] doesn't seem to work with the LIPIcs format currently. A low-key reimplementation goes below.
% [2016.10.23] Switching to margin notes for peanut gallery:
\usepackage{todonotes}
% \presetkeys{todonotes}{inline}{}  % Activate to turn-off margin notes.

% [2016.05.26] This can just be a growing list from paper to paper:
%% \newcommand{\rn}[1]{\pgwrapper{RRN}{#1}}  % Ryan Newton

%% \newcommand{\tlm}[1]{\pgwrapper{TLM}{#1}} % Trevor
%% \newcommand{\bjs}[1]{\pgwrapper{BJS}{#1}} % Bo Joel Svenson
%% \newcommand{\chc}[1]{\pgwrapper{CHC}{#1}} % Chao-Hong Chen
%% \newcommand{\vc}[1]{\pgwrapper{VC}{#1}} % Vikraman Choudhury
%% \newcommand{\bc}[1]{\pgwrapper{BC}{#1}} % Buddhika Chamith
%% \newcommand{\mv}[1]{\pgwrapper{MV}{#1}} % Michael Vollmer
%% \newcommand{\osa}[1]{\pgwrapper{OSA}{#1}} % Omer Agacan
%% \newcommand{\mm}[1]{\pgwrapper{MM}{#1}} % Madan Musuvathi
%% \newcommand{\rgs}[1]{\pgwrapper{RGS}{#1}} % Ryan Scott
%% \newcommand{\csk}[1]{\pgwrapper{CSK}{#1}} % Chaitanya Koparkar
%% \newcommand{\mr}[1]{\pgwrapper{MR}{#1}} % Mike Rainey
%% \newcommand{\sth}[1]{\pgwrapper{STH}{#1}} % Sam Tobin-Hochstadt

%% \newcommand{\mk}[1]{\pgwrapper{MK}{#1}} % Milind Kulkarni
%% \newcommand{\ls}[1]{\pgwrapper{LS}{#1}} % Laith Sakka
%% \newcommand{\vs}[1]{\pgwrapper{VS}{#1} } % Vidush Singhal
%% \newcommand{\ap}[1]{\pgwrapper{AP}{#1} } % Artem Pelenitsyn

%% \newcommand{\spall}[1]{\pgwrapper{SS}{#1}} % Sarah Spall

%% \newcommand{\jd}[1]{\pgwrapper{JD}{#1}} % Joe Devietti
%% \newcommand{\onl}[1]{\pgwrapper{ONL}{#1}} % Omar Navarro-Leija

% ATTENTION passenger, to switch off the comments...
\newcommand{\metacomment}[3]%
% {}
{{\scriptsize\color{#1}{\bf #2}:\ #3}}
% ... switch between the previous two lines to hide/show all visible comments in the PDF
\newcommand{\rn}[1]{\metacomment{blue}{Ryan}{#1}}
\newcommand{\mk}[1]{\metacomment{teal}{Milind}{#1}}
\newcommand{\csk}[1]{\metacomment{orange}{Chaitanya}{#1}}
\newcommand{\mv}[1]{\metacomment{orange}{Michael}{#1}}
\newcommand{\mr}[1]{\metacomment{orange}{Mike}{#1}}
\newcommand{\vs}[1]{\metacomment{olive}{Vidush}{#1}}
\newcommand{\ap}[1]{\metacomment{purple}{Artem}{#1}}

% Add co-authors here or in a downstream file.

\InputIfFileExists{activateeditingmarks}{
}{
    \def\noeditingmarks{}
}

\definecolor{comment-red}{rgb}{0.8,0,0}
\definecolor{dark-green}{rgb}{0.0,0.4,0}
\definecolor{dark-blue}{rgb}{0.0,0.0,0.55}
\definecolor{very-dark-green}{rgb}{0.0,0.3,0}

\ifx\noeditingmarks\undefined
   %% This means someone else should take a look:
   \newcommand{\auditme}[1]{{\color{comment-red}{#1}}}

   %% This means there's a serious problem that must be fixed before
   %% the paper goes out:
   \newcommand{\fixme}[1]{{\color{comment-red}{#1}}}

   %% This is for outlining, i.e., psuedotext that must be converted
   %% to real text:
   \newcommand{\noteus}[1]{{\begin{itemize}\item \textcolor{blue}{#1} \end{itemize}}}

   %% A very poor-man's version of ``track changes'':
   \newcommand{\new}[1]{{\color{very-dark-green}{#1}}}
   \newcommand{\nnew}[1]{{\color{dark-blue}{#1}}}

   \newcommand{\const}[1]{\textred{#1}}
   %\definecolor{mygrey}{rgb}{0.6,0.6,0.6}
   \definecolor{mygrey}{rgb}{0.7,0.7,0.7}

   \newcommand{\textred}[1]{{\color{comment-red}{#1}}}

   % Old version was inline:
   % \newcommand{\pgwrapper}[2]{\textred{(#1: #2)}}
   % New version is in the margin:
   \setlength{\marginparwidth}{1.3cm}
   \newcommand{\pgwrapper}[2]{\todo[size=\tiny]{#1: #2}}

   %% RRN: Dim the background for Ryan's eyes:
   %% Hack: do this ONLY on Ryan's machine.
   %%  I don't know a way based on user or host name, so...
   %%  instead I just signal on a file, activategreybg.tex which I
   %%  don't then checkin.
   \InputIfFileExists{activategreybg}{
       \definecolor{comment-red}{rgb}{0.5,0,0}
       \pagecolor{mygrey}
   }{}

  % When they are their own para, todonotes annoyingly take up vertical space:
  \newcommand{\rnfloat}[1]{\pgwrapper{RRN}{#1}\vspace{-4mm}}  % Ryan Newton

\else
%   \newcommand{\textred}[1]{#1}
% Keep it on so we catch stuff to fix:
   \newcommand{\textred}[1]{{\color{comment-red}{#1}}}
   \newcommand{\textgreen}[1]{{\color{dark-green}{#1}}}
   \newcommand{\auditme}[1]{#1}
   % This is more severe and should not go away:
   \newcommand{\fixme}[1]{\textred{#1}}
   \newcommand{\pgwrapper}[2]{}
%   \newcommand{\note}[1]{}
   \newcommand{\new}[1]{#1}
   \newcommand{\nnew}[1]{#1}
   \newcommand{\const}[1]{#1}

   \newcommand{\rnfloat}[1]{}  % Ryan Newton
\fi

% Just an alias because sometimes we use this:
\newcommand{\Red}[1]{\textred{#1}}
\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
\newcommand{\Green}[1]{\textgreen{#1}}

% These probable should be elsewhere:
\newcommand{\ie}{{i.e.,}}
\newcommand{\eg}{{e.g.,}}
\newcommand{\etal}{\textit{et al.}}

\def\scrunchit{}
\ifx\scrunchit\undefined
  \newcommand{\captionscrunch}{}
\else
%  \newcommand{\captionscrunch}{\vspace{-4mm}}
  \newcommand{\captionscrunch}{\vspace{-3mm}}
\fi

%% \newcommand{\secref}[1]{section~\ref{#1}}
%% \newcommand{\Secref}[1]{Section~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\Secref}[1]{\secref{#1}}
\newcommand{\Figref}[1]{Figure~\ref{#1}\xspace}
\newcommand{\figref}[1]{Figure~\ref{#1}\xspace}
\newcommand{\tabref}[1]{Table~\ref{#1}\xspace}
\newcommand{\Tabref}[1]{Table~\ref{#1}\xspace}



==> eval.tex <==
\section{Evaluation}

We evaluate \system on three applications.
First is a pair of microbenchmarks (Section~\ref{subsubsec:length})
---a list length function and a logical expression evaluator---
that help us explore performance penalties imposed by a sub-optimal data layout.
%
Second is a small library of operations with binary trees (Section~\ref{subsec:trees}).
Third is a blog management software based on the \lstinline|BlogList| example from the
Sections~\ref{sec:overview}--\ref{sec:design} (Section~\ref{subsect:blog}).
Besides the run times, we take a closer look at how \system affects
cache behavior (Section~\ref{subsec:cache}) and compile times (Section~\ref{subsec:heuristic-tradeoffs}).
Finally, we discuss evaluation and its scale (Section~\ref{subsec:scale-eval}).

We detail the impact of various datatype layouts on the performance.
As the baseline, we use \gibbon, the most closely related prior work.
We also compare \system with \mlton (Section~\ref{subsec:mlton}).
%\footnote{The reader should keep in
%  mind that \ghc solves a much harder task of compiling the giant Haskell
%  language with dozens of extensions. Our goal in the brief account of GHC's
%  performance relative to \system is to show the potential of using a dense
%  representation of recursive datatypes with automatic layout management,
%  a technique that could be incorporated in part into GHC.
  % that improvements in GHC could be
  % possible if dense representation of recursive datatypes with automatic layout
  % management was introduced there. That would be a big engineering challenge, or course.
%}.\mv{not sure we want to imply we are advocating for GHC to adopt this strategy}
% Artem: I don't love ''where appropriate`` but we should try to manage
%        expectations: there is only one figure out of many that talks about GHC...
%        If someone can describe better where exactly we decided it be
%        appropriate, that would be appreciated!
For each benchmark, we run 99 iterations and report the run-time mean and
the 95\% confidence interval.

\subsection{Experimental Setup}
We run our benchmarks on a server-class machine with
64 CPUs, each with two threads. The CPU model is AMD Ryzen Threadripper 3990X with 2.2 GHz clock speed. The L1 cache size is 32 KB, L2 cache size is 512 KB and L3 cache size is 16 MB.
%
We use \gibbon's default C backend and call GCC 10.2.0 with \texttt{-O3} to generate binaries.

\subsection{Micro Benchmarks}
\label{subsubsec:length}
\label{subsubsec:logic}

\new{
\begin{description}
\item[ListLength]
This benchmark computes the length of a linked-list and demonstrates the cost of de-referencing memory addresses that are not present in the cache.
%
It uses the linked list datatype:
}
%
\begin{lstlisting}
  data List = Nil | Cons Content List
\end{lstlisting}
%
\new{
If each element of the list is constructed using \lstinline{Cons},
the traversal has to de-reference a pointer---to {\em jump over} the content---each time to access the tail of the list.
%
This is an expensive operation, especially if the target memory address is not present in the cache.
%
%On the contrary, \lstinline{Snoc} lays out the tail of each list next to tag corresponding to \lstinline{Snoc}.
In contrast, if the \lstinline{Content} and \lstinline{List} fields were swapped,
%
then to compute the length, the program only has to traverse $n$ bytes for a list of length $n$---one byte
per \lstinline{Cons} tag---which is extremely efficient.
%
Essentially, \system transforms program to use the
following datatype, while preserving its behavior:}
\begin{lstlisting}
  data List' = Nil' | Cons' List' Content
\end{lstlisting}
In our experiment, the linked list is made of 3M elements and each element contains
an instance of the \textit{Pandoc} \lstinline|Inline| datatype that occupies roughly 5KB.
%\csk{wanted to say something like: 5KB is much bigger than a cache line which makes the pointer de-refrence expensive for \lstinline{Cons}-list and having 3M elements ensures that even the \lstinline{Snoc} tags overflow, so it's not like Snoc cheats by fitting everything in a cache line.}
%
As seen in table~\ref{table:Measure-Length}\footnote{The performance of \lstinline|List'| layout compiled with \gibbon differs from \system as code motion to reorder let expressions results in different code. In addition to a noisy server.}, the performance of the list constructed using the original \lstinline{List} is $\sim$42$\times$ worse than the performance with the \system-optimized, flipped layout.
%
Not only does \lstinline{List} have poor data locality and cache behavior,
but it also has to execute more instructions to de-reference the pointer.
Both \systemGreedy and \systemSolver choose the flipped layout \lstinline|List'|.
%
%% \system is able to identify that the \lstinline{Snoc} constructor has an
%% optimal layout for computing the length of a linked-list and rightly
%% updates the program use this constructor.

%% This is because in the Cons list, the traversal has to do expensive pointer de-references to jump over the Content field serialized after the Cons tag. This adds more instructions and results in poor locality. On the other hand, the Snoc list has all the Snoc cells recursively laid out next to each other. Since the measure length traversal simply has to traverse this Tag field to determine the count, having all Snoc tags serialized right next to each other results in lesser instructions to execute while calculating the length and good spatial locality.
%% \system is able to identify the layout that gives the best performance by analyzing the body of the traversal and rightly places the \textbf{List} field next to the data constructor tag, thus optimizing performance.
%
%% This traversal simply counts the length of a list where the list is either a recursive Cons list or Snoc List storing a Content field. The Content field is a recurve list of Strings. 

\begin{table}[]
    \small
	\centering
	\caption{Run-time mean and 95\% confidence interval (ub, lb) for different
    layouts (seconds).
	The last two columns show the run time for the layouts chosen by
	\systemGreedy and \systemSolver. The numbers in \textcolor{\myblue}{blue}
	correspond to the lowest running time and the numbers in \textcolor{\myred}{red}
	correspond to the highest running time. Legend: l -- left subtree, r -- right subtree of the tree.}%
    \label{table:Right-Most-Tree}\label{table:Measure-Length}\label{table:Logical-Expression-Evaluator}
	\centering
	\begin{tabular}{@{}lrrrrr@{}}
	 \toprule
     \multirow{2}[2]{*}{\thead[l]{Benchmark\\name}}
	 & \multicolumn{2}{c}{{\gibbon}}
	 & \multicolumn{2}{c}{{\system}}\\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}

	 & \multicolumn{1}{c}{{List}}
	 & \multicolumn{1}{c}{{List'}}
	 & \multicolumn{1}{c}{\small{\systemGreedy}}
	 & \multicolumn{1}{c}{\small{\systemSolver}}\\ 
	 \midrule
      \thead[l]{%
      \benchname{ListLength}
      \\\vspace{0cm}}
	         &  \thead{\textcolor{\myred}{62.34}\\ \scriptsize{(62.26, 62.41)}}
			 & \thead{{1.51}\\ \scriptsize{(1.44, 1.59)}}
			 & \thead{\textcolor{\myblue}{1.49}\\ \scriptsize{(1.41, 1.56)}}
	         &  \thead{{1.50}\\ \scriptsize{(1.42, 1.58)}}
	  		\\\midrule
    &
			\multicolumn{1}{c}{{lr}} &
			\multicolumn{1}{c}{{rl}} &
            \multicolumn{1}{c}{\small{\systemGreedy}} &
            \multicolumn{1}{c}{\small{\systemSolver}}
			\\\midrule

      \thead[l]{%
	  \benchname{LogicEval}
      \\\vspace{0cm}}
	        &  \thead{\fnumtwo{4.45199507070707}\\ \scriptsize{(\fnumtwo{4.421091032316951}, \fnumtwo{4.482899109097188})} }
			& \thead{\textcolor{\myred}{\fnumtwo{6.597977737373738}}\\ \scriptsize{(\fnumtwo{6.587444262502335}, \fnumtwo{6.6085112122451415})} }
			&  \thead{{\fnumtwo{3.5554980606060598}}\\ \scriptsize{(\fnumtwo{3.5330752325507118}, \fnumtwo{3.577920888661408})} }
			&  \thead{\textcolor{\myblue}{\fnumtwo{3.5515789595959597}}\\ \scriptsize{(\fnumtwo{3.550932274913144}, \fnumtwo{3.5522256442787756})}}
			\\

      \thead[l]{%
      \benchname{Rightmost}
      \\\vspace{0cm}}
	        &  \thead{\textcolor{\myred}{{384.4}}\\ \scriptsize{(368.4, 400.3)}}
			&   \thead{{{314.5}}\\ \scriptsize{(303.7, 325.3)}}
			&   \thead{{{306.9}}\\ \scriptsize{(295.6, 318.2)}}
			&   \thead{\textcolor{\myblue}{{303.1}}\\ \scriptsize{(292.6, 313.6)}}
			\\
	\bottomrule
	\end{tabular}
\end{table}


\new{
\item[LogicEval]
This microbenchmark implements a short-circuiting logical expressions evaluator
and runts it over synthetically generated, balanced syntax-trees with the height of 30.
The intermediate nodes can be one of \lstinline{Not}, \lstinline{Or}, or \lstinline{And}, selected at random, and
the leaves hold boolean values. % wrapped in a \lstinline{Val}. % Artem -- there
								% should be explanation wrapping somewhere and
								% it should be referenced from here. Or we can
								% just skip this detail for now.
%
}
%
%% This micro benchmark has two traversals, one does short-circuiting of And logical expressions and one does short-circuiting of Or logical expressions. It constructs an AST of a few logical expressions and populates the AST with some random logical values through random selection of expressions.
The syntax-tree datatype is defined as follows:
%
\begin{lstlisting}
  data Exp = Val Bool | Not Exp | Or Exp Exp | And Exp Exp
\end{lstlisting}
%
We measure the performance of the evaluator for differeent orders of the left and right subtrees.
Since the short circuiting evaluates from left to right order of the \lstinline{Exp}, changing the order of the left and right subtrees would affect the performance of the traversal. As can be seen in Table~\ref{table:Logical-Expression-Evaluator},
the layout where the left subtree is serialized before the right subtree results in better performance compared to the tree where the right subtree is serialized before the left one. This is as expected since in the latter case, the traversal has to jump
over the right subtree serialized before the left one in order to evaluate it first and then depending on the result of the left subtree possibly jump back to evaluate the right subtree. This results in poor spatial locality and hence worse performance. \systemGreedy and \systemSolver are able to identify the layout transformations that would give the best performance, which matches the case where the left subtree is serialized before the right subtree
(Table~\ref{table:Logical-Expression-Evaluator}\footnote{The layout chosen by \systemGreedy and \systemSolver
is same as lr, the performance differs from the lr layout compiled with \gibbon as \system does code motion 
which results in different code.}).
\end{description}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/TreeShapedData.pdf}
	\caption{Rightmost: access patterns for, left-to-right (top) and right-to-left (bottom) serializations}
	\label{fig:treeShapedData}
\end{figure}

\subsection{Binary Tree Benchmarks}%
\label{subsec:trees}\label{subsec:eval:trees:rightmost}

We evaluate \system on a few binary tree benchmarks: adding one to all values in a tree,
exponentiation on integers stored in internal nodes, copying a tree and getting the right-most leaf value in the tree.
For the first three benchmarks, the tree representation we use is:
\begin{lstlisting}[]
  data Tree = Leaf | Node Int Tree Tree
\end{lstlisting}
For right-most, the tree representation we use is:
\begin{lstlisting}[]
  data Tree = Leaf Int | Node Tree Tree
\end{lstlisting}

\input{figures/table-bench-trees.tex}

\begin{description}

\item[AddOneTree]
This benchmark takes a full binary tree and increments the values stored in the internal nodes of the tree.
We show the performance of an aligned preorder, inorder and postorder traversal in addition to a misaligned 
preorder and postorder traversal of the tree. Aligned traversals are ones where the data representation exactly
matches the traversal order, for instance, a preorder traversal on a preorder representation of the tree. 
A misaligned traversal order is where the access patterns of the traversal don't match the data layout of the tree.
For instance, a postorder traversal on a tree serialized in preorder. 
Table~\ref{table:Add-one-Tree} shows the performance numbers.
\systemSolver picks the aligned postorder traversal order which is best performing. It makes the recursive calls to the left and right children of the
tree first and increments the values stored in the internal nodes once the recursive calls return. The tree representation is also changed to a postorder
representation with the \lstinline|Int| placed after the left and right children of the tree. 
This is in part due to the structure of arrays effect, as the \lstinline|Int| are placed closer to each other.
\systemGreedy on the other hand picks the 
aligned preorder traversal because of its greedy strategy which prioritizes placing the \lstinline|Int| before the left and right subtree.
The tree depth is set to 27. At this input size, the \misalignedPost traversal failed due to memory errors, and
\misalignedPre runs $\sim$35$\times$ slower than aligned versions because of the skewed access patterns of the traversal.

\item[ExpTree]
This traversal does exponentiation on the values stored in the internal nodes of the tree. It is more computationally intensive than incrementing the value.
We raise the \lstinline|Int| to a power of 10 on a tree of depth 27. Table~\ref{table:Exponentiation-Tree} shows the performance of the different layout and traversal orders.
\systemSolver picks the \alignedPost representation which is the best performing, whereas \systemGreedy picks the \alignedPre representation. 

\item[CopyTree]
Copy-tree takes a full binary tree and makes a fresh copy of the tree in a new memory location.
We use a tree of depth 27 in our evaluation. Table~\ref{table:Copy-Tree} shows the performance of different layout and traversal orders. 
We see that \alignedPost traversal performs the best. Indeed, \systemSolver picks the \alignedPost representation, whereas, \systemGreedy chooses the 
\alignedPre representation.

\item[Rightmost]%
This traversal does recursion on the right child of the tree and returns the \lstinline|Int| value stored in the right-most leaf of the tree.
%
Figure~\ref{fig:treeShapedData} shows an example of a tree with two different serializations of the tree: left-to-right (top) and right-to-left (bottom).
The right-to-left serialization is more efficient because the constant-step movements (blue arrows) are usually more favorable than variable-step ones (red arrows) on modern hardware.
%
Both \systemSolver and \systemGreedy pick the right-to-left serialization, and
Table~\ref{table:Right-Most-Tree} shows that this choice performs better in the benchmark.
%
% As the input, we use the largest tree size (depth of 32) we can on the testing machine.
% The running time of the benchmark is significantly lower than the time it takes to build the tree.
% It is \textit{logarithmic} in the number of nodes in the tree.
\end{description}

%\rn{And why was it a linked list of strings instead of a markup tree or a single string?}
%\vs{I'm not sure why it was entered as a list but its a Pandoc Blovk type.}
\subsection{Blog Software Case Study}
\label{subsect:blog}

The Blog software case study serves as an example of a realistic benchmark, representing a sample of components 
from a \new{blog management web service}. The main data structure \new{is a linked list of blogs where each blog
contains fields} such as header, ID, author information, content, hashtags and date. The fields are a mix
of recursive and non-recursive datatypes. For instance, \lstinline{Content} is a recursive type 
\new{(the Pandoc \lstinline|Block| type)}, but \lstinline{Author} is a single string wrapped in a data
constructor.\footnote{At times, we have to wrap scalars in data constructors to make them packed fields.~\gibbon
does not always support mixing scalar and packed fields due to compiler bugs.}
%\csk{clarify reasoning packed/non-packed fields.}
One possible permutation of fields in the blog is:
%
\begin{lstlisting}[ ]
  data Blogs = Empty|HIADCTB Header Id Author Date Content HashTags Blogs
\end{lstlisting} 
%
%% This datatype is recursive and essentially represents a list of blogs present in the Blog service. 
%% A packed representation of this datatype packs all the fields as close to each other in memory as possible.
%% We perform a few traversals over this data type and show that the layout in which fields are instantiated matters.

We evaluate \system{}'s performance using three different traversals over a list of blogs.
%
Overall, the traversals accept a keyword and a list of blogs; in the
blogs, the traversals inspect either of the three fields: \lstinline{Content},
\lstinline{HashTags}, and the tail of the linked-list, \lstinline{Blogs}.
(Since \lstinline{Blogs}, \lstinline{Content}, and \lstinline{HashTags} are
recursive fields, changing their layout should represent greater differences in performance.)
%
The fields used by an individual traversal are referred as {\em active fields}
and the rest are referred as {\em passive fields}, and we specify these per-traversal below.

In Table~\ref{table:blog-traversals}, we report the performance of the six
possible layouts obtained by permuting the order of the three recursive fields,
and two additional layouts (Columns 1 and 2).
%
The column names indicate the order of fields used;
%
for example, the column \lstinline{hiadctb} reports numbers for the layout with fields ordered as:
\lstinline{Header}, \lstinline{Id}, \lstinline{Author}, \lstinline{Date}, \lstinline{Content}, \lstinline{HashTags}, and \lstinline{Blogs}.
%
All run times are gathered with \gibbon{}, and
%% \footnote{Since \system builds on \gibbon, this is equivalent to running \system with a flag that disables its field reordering optimization.} 
%
%% The column named \system{}
last two columns show the run times for code compiled using \system's greedy
and solver-based optimization, respectively.
%
%\system picks a layout tailored to each traversal, which we specify below.
%
%% We show the run-times of different traversals over a subset permutation of layouts for the Blog data structure when compiled with \gibbon . We compile the Blog data type with \system and show its performance for comparison.


\begin{table}[]
\small
\setlength{\tabcolsep}{1pt} %% default is 6pt
\centering
	\caption{Run-time mean and 95\% confidence interval (ub, lb) for different layouts in the blog software benchmarks (seconds).
		Several possible permutations of layout are shown.
		Layout names abbreviations: h -- Header, t -- HashTags, b -- Blogs, i -- TagID, c -- Content, a -- Author, d -- Date.}%
\label{table:blog-traversals}
\begin{tabular}{@{}p{7mm}rrrrrrrrrrr@{}}
\toprule
\multirow{2}[2]{*}{\thead[l]{\scriptsize Bench.\\\scriptsize name}}
 & \multicolumn{7}{c}{{\gibbon}}
 & \multicolumn{2}{c}{{\system}}\\
 \cmidrule(lr){2-8}\cmidrule(lr){9-10}
 %
 & \multicolumn{1}{c}{\small{{hiadctb}}}
 & \multicolumn{1}{c}{\small{{ctbhiad}}}
 & \multicolumn{1}{c}{\small{{tbchiad}}}
 & \multicolumn{1}{c}{\small{{tcbhiad}}}
 & \multicolumn{1}{c}{\small{{btchiad}}}
 & \multicolumn{1}{c}{\small{{bchiadt}}}
 & \multicolumn{1}{c}{\small{{cbiadht}}}
 & \multicolumn{1}{c}{\small{\systemGreedy}}
 & \multicolumn{1}{c}{\small{\systemSolver}}\\ 
\midrule
\benchname{FilterBlogs} \\
        &  \thead{\fnumtwo{0.2247852661971830}\\ \scriptsize{(\fnumtwo{0.22474188311863516}, \fnumtwo{0.22482864927573096})} }       
		&  \thead{\fnumtwo{0.2243197802816901}\\ \scriptsize{(\fnumtwo{0.22373525904937216}, \fnumtwo{0.22490430151400806})} }
		&  \thead{{\fnumtwo{0.08109379788732393}}\\ \scriptsize{(\fnumtwo{0.08082428580616613}, \fnumtwo{0.08136330996848173})} }
		&  \thead{\fnumtwo{0.26502487464788727}\\ \scriptsize{(\fnumtwo{0.26470682674275325}, \fnumtwo{0.2653429225530213})} }
		&  \thead{\fnumtwo{0.28165434366197184}\\ \scriptsize{(\fnumtwo{0.28142152424862715}, \fnumtwo{0.2818871630753165})} }
		&  \thead{\textcolor{\myred}{\fnumtwo{0.29489771690140854}}\\ \scriptsize{(\fnumtwo{0.29456292511661414}, \fnumtwo{0.29523250868620293})} }
		&  \thead{{\fnumtwo{0.2125426746478873}}\\ \scriptsize{(\fnumtwo{0.2122561149597799}, \fnumtwo{0.21282923433599468})} }
		&  \thead{{\fnumtwo{0.07244831014084505}}\\ \scriptsize{(\fnumtwo{0.07198399286596101}, \fnumtwo{0.07291262741572908})} }
		&  \thead{\textcolor{\myblue}{\fnumtwo{0.05624464183098592}}\\ \scriptsize{(\fnumtwo{0.05621462653189447}, \fnumtwo{0.056274657130077364})} }
		\\
        \\
\benchname{EmphContent}\\
&  \thead{\fnumtwo{0.6727033126760564}\\ \scriptsize{(\fnumtwo{0.6722382387120264}, \fnumtwo{0.6731683866400865})} }
&  \thead{\fnumtwo{0.6501001084507042}\\ \scriptsize{(\fnumtwo{0.6498550137449516}, \fnumtwo{0.6503452031564568})} }
&  \thead{\fnumtwo{1.5980927323943663}\\ \scriptsize{(\fnumtwo{1.5977151332795287}, \fnumtwo{1.598470331509204})} }
&  \thead{\fnumtwo{0.6631653633802816}\\ \scriptsize{(\fnumtwo{0.6629708671325513}, \fnumtwo{0.663359859628012})} }
&  \thead{\textcolor{\myred}{\fnumtwo{1.6327312253521127}}\\ \scriptsize{(\fnumtwo{1.6322556594551008}, \fnumtwo{1.6332067912491246})} }
&  \thead{\fnumtwo{1.6106063239436619}\\ \scriptsize{(\fnumtwo{1.6100967763696805}, \fnumtwo{1.6111158715176432})} }
&  \thead{\fnumtwo{0.4718713577464788}\\ \scriptsize{(\fnumtwo{0.4717313650476324}, \fnumtwo{0.4720113504453252})} }
&  \thead{\textcolor{\myblue}{\fnumtwo{0.4662895661971831}}\\ \scriptsize{(\fnumtwo{0.4661310844342112}, \fnumtwo{0.466448047960155})} }
&  \thead{\fnumtwo{0.6406900507042251}\\ \scriptsize{(\fnumtwo{0.640593687233358}, \fnumtwo{0.6407864141750923})} }
\\
\\
\benchname{TagSearch} \\
&  \thead{\fnumtwo{1.9893401126760561}\\ \scriptsize{(\fnumtwo{1.9890376935881537}, \fnumtwo{1.9896425317639586})} }
&  \thead{\fnumtwo{1.9794032253521132}\\ \scriptsize{(\fnumtwo{1.979185046541394}, \fnumtwo{1.9796214041628324})} }
&  \thead{\fnumtwo{3.2946498450704222}\\ \scriptsize{(\fnumtwo{3.2926928080206848}, \fnumtwo{3.2966068821201597})} }
&  \thead{\fnumtwo{1.6800026760563378}\\ \scriptsize{(\fnumtwo{1.679670088341037}, \fnumtwo{1.6803352637716387})} }
&  \thead{\textcolor{\myred}{\fnumtwo{3.3090972676056336}}\\ \scriptsize{(\fnumtwo{3.308674578901536}, \fnumtwo{3.3095199563097313})} }
&  \thead{\fnumtwo{3.3028858732394366}\\ \scriptsize{(\fnumtwo{3.302365980422784}, \fnumtwo{3.3034057660560894})} }
&  \thead{\fnumtwo{1.8170195492957746}\\ \scriptsize{(\fnumtwo{1.8164916768029753}, \fnumtwo{1.8175474217885739})} }
&  \thead{\fnumtwo{1.7559784788732393}\\ \scriptsize{(\fnumtwo{1.7555039213525125}, \fnumtwo{1.756453036393966})} }
&  \thead{\textcolor{\myblue}{\fnumtwo{1.736654943661972}}\\ \scriptsize{(\fnumtwo{1.736380487003441}, \fnumtwo{1.7369294003205031})} }
\\
\bottomrule
\end{tabular}
\end{table}


%\subsubsection{{\bf FilterBlogs}}

\begin{description}

\item[FilterBlogs]
filters the list of blogs and only retains those which contain the given
keyword in the \lstinline{HashTags} field. %\csk{should describe what HashTags field is above.}
%% This traversal searches for a word queried by the user and returns all the blogs from the list of blogs in the service that have that keyword in the list of HashTags maintained by a blog. This traversal is essentially a \textit{map} over the blogs with the function (\textit{f}) that is passed to map having the type signature of \textit{(String -> Blogs -> Maybe Blogs)}. \textit{f} takes the queried keyword, the old Blog and returns the old Blog if this keyword is present in the HashTags list.
%
%%  Therefore, in table~\ref{table:blog-traversals} we show the performance of the permutations of the layouts where these fields are shuffled around when compiled with \gibbon. The last column shows the performance of the layout chosen by \system.
%
%% This traversal makes use of only the \lstinline{HashTags} and \lstinline{Blogs} fields. We refer to these fields as ``active fields''. The rest of the fields are unused and we call these ``passive fields''.
%
\new{The {\em active fields} for this traveral are \lstinline{HashTags} and \lstinline{Blogs}.}
%
Theoretically, the performance of this traversal is optimized when the \lstinline{HashTags} field is serialized before \lstinline{Blogs} on account of the first access to \lstinline{HashTags} in the traversal.
%
%% As expected the layout \textbf{\textit{tbchiad}} gives the best performance when compiled with \gibbon.
This is confirmed in practice with the layout \textbf{\textit{tbchiad}} being the fastest.
%
% The access to \lstinline{HashTags} comes first since its serialized first in memory and once HashTags is fully traversed, the traversal can access blogs in an optimal manner without unnecessary movement in the packed buffer.
%
\system chooses the layout with \lstinline{HashTags} serialized first and followed by \lstinline{Blogs};
\new{
  the order of other fields remains unchanged compared to the source program,
  but this has no effect on performance since they are {\em passive fields}.
}
%% does not matter since they are passive fields and \new{their new order depends on their initial order specified in the program.}
%% it depends on the order of these fields in the initial layout given to \system to optimize.
Table~\ref{table:blog-traversals} also shows that layout chosen by \system performs similar to the layout \textbf{\textit{tbchiad}}.
Both \systemSolver and \systemGreedy pick the layout \textbf{\textit{tbhiadc}} when compiled from the initial layout \textbf{\textit{hiadctb}}.

%% \subsubsection{Traversal2: Emphasize a word queried in the content:}
%\subsubsection{{\bf EmphContent}}

\item[EmphContent]
%This traversal takes a keyword and a list of blogs as input. It then
searches the content of each blog for the keyword and emphasizes all its occurrences there (if any).
%
%% This traversal does this recursively for all the blogs in the program. This traversal is a map where the supplied function(\textit{f}) has the type signature of \textit{(String -> Blogs -> Blogs)}. It takes a keyword to be emphasized in the Content fields, the old Blogs and returns the Blogs with either the new content if the keyword is present or leave the content unchanged if it is not present in the content. 
%
The active fields in this traversal are \lstinline{Content} and \lstinline{Blogs}.
Based on the access pattern (\lstinline{Content} accessed before \lstinline{Blogs}),
the layout with the best performance should place \lstinline{Content} first followed by \lstinline{Blogs}.
In practice, the layout with the best performance is \textbf{\textit{cbiadht}}.
In contrast, \systemSolver prioritizes the placement of \lstinline{Blogs} before \lstinline{Content}, but
it also changes the traversal to recurse on the blogs first and then emphasize content.
%% placing it Content first followed by Blogs.
The passive fields are placed afterwards.
The layout chosen by \systemSolver is \textbf{\textit{bchiadt}}, whereas the layout chosen by \systemGreedy is \textbf{\textit{cbhiadt}} when compiled from the initial layout \textbf{\textit{hiadctb}}.
The performance of \systemGreedy and
\systemSolver differ because datatypes other than \lstinline{Blogs} differ in their layout choices.

%% \subsubsection{Traversal3: Search a keyword in HashTags and emphasize it in content:}
% \subsubsection{{\bf TagSearch}}

\item[TagSearch]
% This traversal takes a keyword and a list of blogs as input and
looks for the presence of the keyword in the \lstinline{HashTags} field, and
if the keyword is present, the traversal emphasizes the keyword in the \lstinline{Content}.
%
%% and depending on if its present or not emphasizes or leaves it unchanged in the Content field. This traversal does this recursively for all the blogs in the program. 
%
%% This traversal is a map over the blogs with the supplied function(\textit{f}) having the type signature of \textit{(String -> Blogs -> Blogs)}. It takes a keyword, searches it 
%% in the HashTags and if it is present in the HashTags, emphasizes it in the Content field. The active fields in this traversal are HashTags, Content and Blogs. 
%
The layout with the best performance is
\textbf{\textit{tcbhiad}} because of the
access pattern, which inspects \lstinline{HashTags} followed by \lstinline{Content} followed by \lstinline{Blogs}.
\systemSolver chooses the layout \textbf{\textit{tbchiad}}---which places \lstinline|HashTags| followed by \lstinline|Blogs|
followed by \lstinline|Content|---and changes the traversal to recurse on \lstinline|Blogs| first and later emphasize
\lstinline|Content| in the \lstinline|then| branch.
On the other hand, \systemGreedy chooses \textbf{\textit{tcbhiad}}
when compiled from the initial layout \textbf{\textit{hiadctb}}.
%\system's performance is better and shows the effectiveness of the optimization.

%The layout \system chooses also places these fields in the same order. The performance as shown in Table~\ref{table:blog-traversals} and is similar to \textbf{\textit{tcbhiad}}. 

\end{description}

\subsubsection{\bf Globally optimizing multiple functions}

%\vs{TODO: add layout of solver and greedy version.}
We use \system to globally optimize the three blog traversals we discussed above such that we pick one layout for all traversals that minimizes the overall runtime. Table~\ref{table:global-blog-traversals} shows the runtime for a layout we compiled using \gibbon (\textit{\textbf{hiadctb}}), \systemSolver(\textit{\textbf{tbchiad}}) 
and \systemGreedy(\textit{\textbf{tbchiad}}). We see that \systemGreedy and \systemSolver do a good job in reducing the traversal time globally. 
All the three traversals are run in a pipelined fashion sequentially. Although, \systemSolver does worse with \textit{TagSearch} when run in a pipelined manner, 
it is actually better performing with \systemSolver when run alone as seen in table~\ref{table:blog-traversals}. 
Note that \systemSolver changes more that one data constructor based on the \textit{inlineable} attribute that \systemGreedy does not.
For instance, \systemSolver uses a packed \lstinline|Inline| list in the \lstinline|Content| with the tail serialized before \lstinline|Inline|.
Whereas, \systemGreedy uses a conventional packed list. In a pipelined execution of the traversals, although this helps reduce the runtime in the case 
of the content search traversal, it inadvertently increases the runtime in case of the tag search traversal due to a cache effect
that can benefit from runtime information.

\begin{table}
	\centering
	\caption{Run-time mean and 95\% confidence interval (ub, lb) for the blog
	  software benchmarks when \system optimizes the data layout globally (seconds).
           The input parameters are different from the single-function
		   optimization case.}%
\label{table:global-blog-traversals}
\begin{tabular}{@{}lrrr@{}}
	\toprule
    \multirow{2}[2]{*}{\thead[l]{Benchmark\\name}}
	& \multicolumn{1}{c}{{\gibbon}}
	& \multicolumn{2}{c}{{\system}}\\
    \cmidrule(lr){2-2}\cmidrule(lr){3-4}

	& \multicolumn{1}{c}{{hiadctb}}
	& \multicolumn{1}{c}{\small{\systemGreedy}}
	& \multicolumn{1}{c}{\small{\systemSolver}}\\
	\midrule
      \thead[l]{%
		\benchname{FilterBlogs}
		\\\vspace{0cm}}
			&  \thead{\textcolor{\myred}{\fnumtwo{2.230235366197183}}\\ \scriptsize{(\fnumtwo{2.2296601843214643}, \fnumtwo{2.230810548072902})}}
			& \thead{\fnumtwo{0.11155572676056338}\\ \scriptsize{(\fnumtwo{0.11129754268785376}, \fnumtwo{0.11181391083327301})}}
			& \thead{\textcolor{\myblue}{\fnumtwo{0.09500013323943661}}\\ \scriptsize{(\fnumtwo{0.0949635646349502}, \fnumtwo{0.09503670184392302})}}
			 \\
      \thead[l]{%
		\benchname{EmphContent}
		\\\vspace{0cm}}
		   &  \thead{\fnumtwo{1.5747499154929574}\\ \scriptsize{(\fnumtwo{1.5742668530634656}, \fnumtwo{1.5752329779224492})} }
		   & \thead{\textcolor{\myred}{\fnumtwo{1.3836891549295773}}\\ \scriptsize{(\fnumtwo{1.3835601882499424}, \fnumtwo{1.3838181216092122})} }
		   &  \thead{\textcolor{\myblue}{\fnumtwo{1.3222079577464787}}\\ \scriptsize{(\fnumtwo{1.3220798547722914}, \fnumtwo{1.322336060720666})} }
		   \\
      \thead[l]{%
		\benchname{TagSearch}
		\\\vspace{0cm}}
		   &  \thead{{\fnumtwo{2.196739676056339}}\\ \scriptsize{(\fnumtwo{2.196016148977572}, \fnumtwo{2.197463203135106})}}
		   &   \thead{\textcolor{\myblue}{\fnumtwo{1.830104352112676}}\\ \scriptsize{(\fnumtwo{1.828666212218745}, \fnumtwo{1.8315424920066072})}}
		   &   \thead{\textcolor{\myred}{\fnumtwo{2.3503619154929574}}\\ \scriptsize{(\fnumtwo{2.350152096698425}, \fnumtwo{2.35057173428749})}}
		   \\
   \bottomrule
   \end{tabular}
\end{table}


% \vs{The examples we have with the new cost model, this seems like a redundant section, maybe we remove this given 25 page limit for camera ready.}
% \subsubsection{{\bf tagSearch: varying likelihood of paths taken}}
% %
% % Traversal 3's
% TagSearch's source code is similar to our running example~\ref{fig:blog-travesal} where we
% %
% take different code paths
% % are traversing different paths
% based on if a keyword is present in the tags of the blog post or not. Thus, depending on which branch is more likely, different layouts of the Blog value can have different runtime performance. 

% This information cannot be inferred statically since the contents of the Blog is known only at runtime. This means that \system may not be able to generate an optimal layout on its own since it does not have the information about which branch is more likely via statically analyzing the structure of the program.
% %
% (As mentioned in \secref{sec:design}, we assume uniform likelihoods for branches if no information is provided.)

%\begin{table}[]
%\setlength{\tabcolsep}{0.1pt} %% default is 6pt
%\centering
%\ra{1}
%\begin{tabular}{@{}p{0.5in}rcrcr@{}}\toprule
%& \multicolumn{1}{c}{\textit{$Layout_{\tiny{\system(without\:\:pragma)}} $ }} & 
% & \multicolumn{1}{c}{$Layout_{\tiny{\system(with\:\:pragma)}}$ }\\ \midrule
%$Mdn$ & 0  &&   0 \\
%\bottomrule
%\end{tabular}
%\caption{Biasing the ``Then'' Branch for traversal 3: runtime in seconds for a subset permutation of different layouts when compiled with \gibbon .
%$Layout_{\system(without\:\:pragma)}$  shows the run-time for the layout chosen by \system without user supplied pragmas and $Layout_{\tiny{\system(with\:\:pragma)}}$ shows the run-time when the user supplies pragmas to branches. Legend: h - Header, t - HashTags, b - Blogs, i - TagID, c - Content, a - Author, d - Date}
%\end{table}


% \begin{table}[]
% \setlength{\tabcolsep}{0.1pt} %% default is 6pt
% \centering
% \ra{1}
% \begin{tabular}{@{}p{0.5in}rcrcr@{}}\toprule
% & \multicolumn{1}{c}{\textit{{\small{\systemSolver(without\:\:pragma)}} }} & 
%  & \multicolumn{1}{c}{{\textit{\small{\systemSolver(with\:\:pragma)}}} }\\ \midrule
% $Tag Search$ \\
% $Then$ & 1.707  &&  1.707 \\

% $Tag Search$ \\
% $Else$ & 0.0292  &&  0.0292 \\
% \bottomrule
% \end{tabular}
% \caption{Performance of traversal 3 (Tag Search) when the input is biased for either the ``Then'' or ``Else'' branch through the traversal. 
% {\small{\system(without\:\:pragma)}} shows the run-time for the layout chosen by \system without user supplied pragmas and {\small{\system(with\:\:pragma)}} shows the run-time when the user supplies likelihood values through pragmas in branches. The layout chosen in both the cases (with and without pragma is the same). Legend: h - Header, t - HashTags, b - Blogs, i - TagID, c - Content, a - Author, d - Date}
% \label{table:biasBranch}
% \end{table}


% \begin{table}[]
% \setlength{\tabcolsep}{0.1pt} %% default is 6pt
% \centering
% \ra{1}
% \begin{tabular}{@{}p{0.5in}rcrcr@{}}\toprule
% & \multicolumn{1}{c}{\textit{{\small{\system(without\:\:pragma)}} }} & 
%  & \multicolumn{1}{c}{{\textit{\small{\system(with\:\:pragma)}}} }\\ \midrule

% \bottomrule
% \end{tabular}
% \caption{Biasing the ``Else'' Branch for traversal 3 (TagSearch): Here we show the difference in performance when be bias the else branch of the traversal.
% {\small{\system(without\:\:pragma)}} shows the run-time for the layout chosen by \system without user supplied pragmas and {\small{\system(with\:\:pragma)}} shows the run-time when the user supplies likelihood values through pragmas in branches. Legend: h - Header, t - HashTags, b - Blogs, i - TagID, c - Content, a - Author, d - Date}
% \label{table:biasBranch}
% \end{table}




%\begin{table}[t]
%\centering
%\ra{1.3}
%\begin{tabular}{@{}rrrcrr@{}}\toprule
%& \multicolumn{2}{c}{Bias then branch} & & \multicolumn{2}{c}{Bias else branch} \\ 
%\cmidrule{2-3} \cmidrule{5-6}
%& \gibbon(s) & \system(s) && \gibbon & \system  \\ \midrule
%HIADCTB\\
%$M$     &    &     &&    &      \\
%$Mdn$ &    &      &&   &     \\
%CTBHIAD\\
%$M$     &    &      &&   &    \\
%$Mdn$ &   &      &&    &    \\
%\bottomrule
%\end{tabular}
%\caption{Runtime in seconds for case study where we vary the likelihood of branches in Traversal3. Legend: H - Header, T - HashTags, B - Blogs, I - TagID, C - Content, A - Author, D - Date}
%\vspace{-3em}
%\end{table}


%% However if the programmer has knowledge of which branch is more likely, we can use this knowledge to our advantage when ordering the fields of the data constructor. To this end, we could allow the programmer to specify which branch is more likely through \textit{annotation pragmas}\footnotemark{} in the source code. The programmer may specify the likelihood of particular branches while writing the traversal. If provided, \system could parse these and use them while generating the optimal layout of fields in the data constructor. 
%% \footnotetext{Currently \system does not provide the presence of such pragmas. Pragmas for the user to provide likelihoods are under development. The user provided likelihoods are currently hardcoded in the compiler in order to get the results}
% \rn{I don't like the speculative likelihood annotation thing... we would more likely just use profile data.}

% As a case study, we show the performance of the Blog data type for an input which biases both the ``Then'' and ``Else'' branch of the traversal separately. Without information on which branch is likely, \system produces a layout which has sub-optimal performance in the ``Else'' branch. The performance of this layout is shown in Table~\ref{table:biasBranch} in the {\small{\system(without\:\:pragma)}} column. This layout places HashTags first, followed by Content, Blogs and then the passive fields. Since the traversal goes to the ``Else'' branch, it has to jump over the Content fields serialized in between HashTags and Blogs resulting in poor performance. 

% When \system is given the information about which branch is likely, it generates a different layout where it places the HashTags field first, followed by Blogs, Content and finally the passive fields. This gives better performance as shown in the column {\small{\system(with\:\:pragma)}}  of table~\ref{table:biasBranch}.
% % 
% Since branch frequency from profiling data is a reasonable assumption, 
% % \system can be engineered easily to reason about the likelihoods if passed, it
% \system{} can generate more optimal layouts when compared to \gibbon. We also show the performance of the optimal layout generated by \system for the ``Then'' branch in \Figref{table:biasBranch}.

%\subsubsection*{When then branch is more likely in traversal~\ref{fig:blog-traversal}:}

%Here we provide a higher weight to the then branch in the source code which prioritizes the layout for the then branch. 


%\subsubsection*{When else branch is more likely in traversal~\ref{fig:blog-traversal}:}

%Here we provide a higher weight to the else branch in the source code which prioritizes the layout for the else branch.

%\subsubsection{Delete a keyword in HashTags: }
%
%This traversal takes a keyword to be deleted from the hash-tags of a Blog and a list of blogs as input. It traverses the hash-tags which is a linked-list of keywords and deletes the queried keyword in the hash-tags. 
%It does this recursively for all the blogs in the program. 

\begin{figure}[t]
\begin{minipage}[h]{.53\linewidth}
		\benchname{FilterBlogs}\\
		\includegraphics[width=\textwidth]{plots/SpeedupMarmosetSmlFilterBlogs}

		\benchname{EmphContent}\\
		\includegraphics[width=\textwidth]{plots/SpeedupMarmosetSmlContentSearch}

		\benchname{TagSearch}\\
		\includegraphics[width=\textwidth]{plots/SpeedupMarmosetSmlTagSearch}

	   \caption{Performance comparison of \systemSolver with \mlton.
	   The pair of numbers on top of each bar shows the median runtime in seconds of \systemSolver followed by the corresponding layout when compiled with \mlton.}
	   \label{fig:speedupghc}
\end{minipage}
\hfill
\begin{minipage}[h]{.44\linewidth}
		\includegraphics[width=.9\textwidth]{plots/CompileTimes-legend}

		\benchname{FilterBlogs}\\
		\includegraphics[width=\textwidth]{plots/FilterBlogCompileTimes-nolegend}

		\benchname{EmphContent}\\
		\includegraphics[width=\textwidth]{plots/ContentSearchCompileTimes-nolegend}

		\benchname{TagSearch}\\
		\includegraphics[width=\textwidth]{plots/TagSearchCompileTimes-nolegend}

	   \caption{
	             Average compile times (99 runs) in seconds for different layouts and traversal combinations
	   			 when compiled with \gibbon and when optimized by \systemGreedy and \systemSolver.
				 % The bar in \textit{Blue} is the time for \systemSolver after subtracting the
				 % time for solver IO and the bar in \textit{Red} is the time taken to do the IO call to the
				 % DOCPLEX solver. The total compile time for \systemSolver includes the time for doing the CFG
				 % analysis, generating the access graph, the solver time, reordering the datatype and repairing
				 % the code, The majority of which is added by the solver IO.
				 }
	   \label{table:compiletimes}
\end{minipage}
\end{figure}


\subsubsection{{\bf Comparison of \system against \mlton}}
\label{subsec:mlton}

We compare \system{}'s performance to \mlton{}, which compiles programs
written in Standard ML, a strict language, to executables that are small
with fast runtime performance.

\Figref{fig:speedupghc} shows the the speedup of \system over \mlton.
As shown, the performance of \system is better than \mlton by significant margins for all the layouts and traversals.
Since ADTs in \mlton are \textit{boxed} -- even though native integers or native arrays are \textit{unboxed} -- such a behavior is expected 
because it adds more instructions (pointer de-referencing) and results in worse spatial locality.

\subsubsection{{\bf Comparison of \system against \ghc}}
\label{subsec:ghc}

We compare \system{}'s performance to GHC, which is especially
optimized to run functional programs.

\begin{figure}
	\centering
	\begin{subfigure}[]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{plots/SpeedupMarmosetGhcFilterBlogs}
		\caption{Filter Blogs Traversal.}
		\label{table:speedupghc-filterblogs}
	\end{subfigure}
	\hfill
	\begin{subfigure}[]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{plots/SpeedupMarmosetGhcContentSearch}
		\caption{Content Search Traversal.}
		\label{table:speedupghc-contentsearch}
	\end{subfigure}
	\hfill
	\begin{subfigure}[]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{plots/SpeedupMarmosetGhcTagSearch}
		\caption{Tag Search Traversal.}
		\label{table:speedupghc-tagsearch}
	\end{subfigure}
	   \caption{Performance comparison of \systemSolver with \ghc.}
	   \label{fig:speedupghc}
\end{figure}

\Figref{fig:speedupghc} shows the the speedup of \system over \ghc when evaluated strictly for an apples to apples comparison. We pass the optimization option \textit{-O2} to \ghc while compiling. As shown, the performance of \system is better than \ghc by significant margins for all the layouts and traversals. Since the types in \ghc are \textit{boxed}, such a behavior is expected because it adds more instructions (pointer de-referencing) and results in worse spatial locality.

\subsection{Cache behavior}%
\label{subsec:cache}

% \begin{table}[]
% \setlength{\tabcolsep}{0.0pt} %% default is 6pt
% \centering
% \ra{1}
% \begin{tabular}{@{}p{0.6in}rcrcrcrcrcrcrcrcr@{}}\toprule
% & \multicolumn{1}{c}{\textit{hiadctb}} & 
%  & \multicolumn{1}{c}{\textit{ctbhiad}} &
%  & \multicolumn{1}{c}{\textit{tbchiad}} &
%  & \multicolumn{1}{c}{\textit{tcbhiad}} &
%  & \multicolumn{1}{c}{\textit{btchiad}} &
%  & \multicolumn{1}{c}{\textit{bchiadt}} &
%  & \multicolumn{1}{c}{\textit{cbiadht}} &
%  & \multicolumn{1}{c}{\textit{\systemGreedy}} &
%  & \multicolumn{1}{c}{\small{\systemSolver}}\\ \midrule
% $Filter Blogs$ \\
% $L3\:misses$      &  \textcolor{\myred}{\snum{13688949.333333334}}           &&  \snum{13647736.111111112}  		   &&  {\snum{1670928.0}}   		     &&  {\snum{14134971.666666666}} 									&& \snum{13415231.777777778} 			  && \snum{13646276.888888888} 		 	 &&  \snum{8470132.555555556}      && \textcolor{\myblue}{\snum{1635723.2222222222}} && \snum{1646244.3333333333} \\
% $L3\:accesses$    & \textcolor{\myred}{\snum{17151877.333333332}}            &&  \snum{16509412.777777778}  		   &&  {\snum{7615203.0}}   		     && {\snum{17010157.888888888}} && \snum{15951598.444444444} 			  && \snum{16256262.333333334} 			 &&  \snum{13084325.444444444}               					&& \snum{7555649.111111111}						 && \textcolor{\myblue}{\snum{7549853.444444444}}      	\\
% $L3\:miss\:rate$  & {\fnumthree{0.7981021008545771}} 	&&  \fnumthree{0.8266639337700382}  &&  {\fnumthree{0.21942002071382732}}	 && {\fnumthree{0.8309723965525149}} && \textcolor{\myred}{\fnumthree{0.8409960810197036}}  && \fnumthree{0.8394473839725942}   &&  \fnumthree{0.6473495780519539}     				&& \textcolor{\myblue}{\fnumthree{0.21649009875495365}}		 &&  \fnumthree{0.2180498397018185}    \\
% $Ins$    & {\snum{583470105.5555556}}          				&&  \snum{582533028.4444444}  		   && {\snum{583515820.7777778}}   		 	 && {\snum{581535328.1111112}} 									&& \textcolor{\myblue}{\snum{579646835.3333334}} 		  && \snum{578594445.4444444} 		 	 &&   \textcolor{\myred}{\snum{586877323.4444444}}              		&& \snum{583515815.6666666}									 &&   \snum{583515815.2222222}      \\
% \\
% $Content Search$\\
% $L3\:misses$ 		& {\snum{18901820.666666668}}  								&&  \snum{16680031.111111112}  				&&  {\snum{19447606.444444444}}   					&& {\snum{17056085.111111112}} 					&& \textcolor{\myred}{\snum{21874690.444444444}}    					 		&& {\snum{21780863.777777776}}  			    &&   {\snum{12162521.222222222}}     			&& \textcolor{\myblue}{\snum{11750799.0}}				&& \snum{14249030.333333334}\\
% $L3\:accesses$  	& {\snum{34914340.11111111}}  								&&  \snum{32917716.222222224}  				&&   {{\snum{33649045.222222224}}}  				 	&& {\snum{33867834.88888889}} 					&& \textcolor{\myred}{\snum{36013492.88888889}}     		 					&& {\snum{35869930.44444445}}     		 	&&  {\snum{30606836.666666668}}     			&& \snum{29779038.333333332}				&& \textcolor{\myblue}{\snum{28204429.555555556}} 	\\
% $L3\:miss\:rate$ 	& \fnumthree{0.5413769988638957}        					&&  \fnumthree{0.5067189655110609}  	    &&  {\fnumthree{0.5779541831279367}}         	&& {\fnumthree{0.503607188563056}}       	&& \textcolor{\myred}{\fnumthree{0.6074026341164304}}                     &&  {\fnumthree{0.6072178983316431}}      &&   {\fnumthree{0.39737923113982554}}  		&& \textcolor{\myblue}{\fnumthree{0.39459968009936297}}			&& 	\fnumthree{0.5052054077274056}\\
% $Ins$ 		&  {\snum{5848090746.222222}}				&&  \snum{5837088833.111111}  				&&  {\snum{6776502981.222222}}   					&& {\snum{5844075395.222222}} 					&& \snum{6779241987.666667}   			 				&& \textcolor{\myred}{\snum{6779244909.888889}}            				    &&  \snum{5840089571.111111}     		&& \snum{5840081527.0}					&& \textcolor{\myblue}{\snum{5837021466.666667}}	\\
% \\
% $Tag Search$ \\
% $L3\:misses$ 		& \textcolor{\myred}{\snum{44582803.0}}    							&&  {\snum{43328252.0}}    				&& {\snum{42657869.0}}       && {\snum{39958549.55555555}}   					    && \snum{38454909.55555555} 	    			  			&& {\snum{42618967.666666664}}  		 			&&  \snum{39621576.44444445}  		 	    && \snum{34350961.88888889}			&& \textcolor{\myblue}{\snum{23895872.444444444}}  \\
% $L3\:accesses$ 		& \snum{129939475.33333333}   						 	&&  {\snum{130000024.1111111}}   				&&  \textcolor{\myred}{\snum{212150507.33333334}}      &&  {\snum{134590067.2222222}}   					&& \snum{182445264.2222222} 	      						&& {\snum{148496853.1111111}}   		 			&& {\snum{129647905.44444445}}  			&& \snum{130411896.44444445} 					&& \textcolor{\myblue}{\snum{80664682.55555555}}  \\
% $L3\:miss\:rate$ 	& \textcolor{\myred}{\fnumthree{0.343104379062882}} 					&&  {\fnumthree{0.3332941843377453}}  			&&  \textcolor{\myblue}{\fnumthree{0.20107361295618048}} 			 && {\fnumthree{0.29689077641650796}} 			&& {\fnumthree{0.210775049270211}}  				&& {\fnumthree{0.2870024971827349}}    		&& {\fnumthree{0.30560907489109207}}  && \fnumthree{0.2634035914317251}  	&& \fnumthree{0.29623711006346337}\\
% $Ins$ 		& \snum{22501467492.88889}  							&&  \textcolor{\myblue}{\snum{22497197160.555557}}  	 				&& {\snum{23043358952.11111}}    				 && {{\snum{22497861297.88889}}} 					&& \textcolor{\myred}{\snum{23043512418.0}} 	  						&& {\snum{23041810439.555557}} 	&&  \snum{22498728619.333332} 			 && \snum{22498730120.0}					&& \snum{22487660868.333332}  \\
% \bottomrule
% \end{tabular}
% \caption{Various performance stats (\textit{PAPI}) for different traversals for a subset permutation of different layouts when compiled with \gibbon.
% The last two columns show the cache misses for the layout chosen by \small{\systemGreedy} and \small{\systemSolver} respectively. Legend: h - Header, t - HashTags, b - Blogs, i - TagID, c - Content, a - Author, d - Date. The numbers in \textcolor{\myblue}{Blue} correspond to the min in the row and the numbers in \textcolor{\myred}{Red} correspond to the max in the row.}
% \label{table:filterblogs-papi}
% \end{table}

\begin{table}[t]
	\setlength{\tabcolsep}{3.5pt} %% default is 6pt
	\centering
	\caption{PAPI performance counter statistics (average of 99 runs) for different blog traversals.}
	\begin{tabular}{@{}lrrrrrrrrr@{}}
	\toprule
    \multirow{2}[2]{*}{\thead[l]{Benchmark\\name or metric}}
	  & \multicolumn{7}{c}{{\gibbon}}
      & \multicolumn{2}{c}{{\system}}\\
    \cmidrule(lr){2-8}\cmidrule(lr){9-10}

	 & \multicolumn{1}{c}{\small{{hiadctb}}}
	 & \multicolumn{1}{c}{\small{{ctbhiad}}}
	 & \multicolumn{1}{c}{\small{{tbchiad}}}
	 & \multicolumn{1}{c}{\small{{tcbhiad}}}
	 & \multicolumn{1}{c}{\small{{btchiad}}}
	 & \multicolumn{1}{c}{\small{{bchiadt}}}
	 & \multicolumn{1}{c}{\small{{cbiadht}}}
	 & \multicolumn{1}{c}{\small{{\systemGreedy}}}
	 & \multicolumn{1}{c}{\small{\systemSolver}}\\ 
	\midrule
	\benchname{FilterBlogs} \\
	Ins    & {\snum{583007860.8888888}} &  \snum{582007417.2222222} & {\snum{583006557.5555556}}   & {\snum{581007422.0}} & \textcolor{\myblue}{\snum{579006542.1111112}} & \snum{578007431.3333334} &   \textcolor{\myred}{\snum{586007412.4444444}} & \snum{583006551.4444444} &   \snum{583006570.4444444}    \\
	Cycles    & {\snum{989222808.8888888}} &  \snum{959711380.1111112} & \textcolor{\myblue}{\snum{285081123.8888889}}   & {\snum{1052921958.2222222}} & {\snum{1200439241.3333333}} & \textcolor{\myred}{\snum{1248215771.1111112}} &   {\snum{877792663.1111112}} & \snum{279146331.4444444} &   \snum{289017037.7777778}    \\
	L2\:DCM    & {\snum{11185155.333333334}} &  \snum{11510078.222222222} & {\snum{938489.3333333334}}   & \textcolor{\myred}{\snum{13337049.333333334}} & {\snum{12928602.222222222}} & \snum{13065840.0} &   {\snum{7789525.777777778}} & \snum{889989.7777777778} &   \textcolor{\myblue}{\snum{874607.7777777778}}    \\
	\\
	\benchname{EmphContent}\\
	Ins    & {\snum{5845022229.888889}} &  \snum{5834021360.444445} & {\snum{6776362325.666667}}   & {\snum{5841021767.888889}} & {\snum{6779241706.444445}} & \textcolor{\myred}{\snum{6779244615.888889}} &   \textcolor{\myblue}{\snum{5837021292.777778}} & \snum{5837021295.333333} &   \snum{5837021366.222222}    \\
	Cycles   & {\snum{2892647565.888889}} &  \snum{2738456405.4444447} & {\snum{4272337912.0}}   & {\snum{2842427055.6666665}} & \textcolor{\myred}{\snum{4340585270.333333}} & \snum{4291414051.5555553} &   \textcolor{\myblue}{\snum{2056621185.3333333}} & \snum{2061807292.6666667} &   \snum{2812417391.5555553}    \\
	L2\:DCM    & {\snum{12800140.0}} &  \snum{10780195.333333334} & {\snum{20295265.222222224}}   & {\snum{13283107.333333334}} & \textcolor{\myred}{\snum{20549853.111111112}} & \snum{20994551.666666668} &   \textcolor{\myblue}{\snum{7727582.888888889}} & \snum{7663269.0} &   \snum{10702561.555555556}    \\
	\\
	\benchname{TagSearch} \\
	Ins    & {\snum{22490860539.77778}} &  \textcolor{\myblue}{\snum{22487260185.555557}} & \textcolor{\myred}{\snum{23043358250.333332}}   & {\snum{22487260291.333332}} & {\snum{23043009879.0}} & \snum{23041811630.22222} &   {\snum{22488060134.77778}} & \snum{22487659963.444443} &   \snum{22487659965.0}    \\
	Cycles    & {\snum{8587261902.555555}} &  \snum{8593729939.88889} & {\snum{9609104561.222221}}   & \textcolor{\myblue}{\snum{7288093434.666667}} & {\snum{9607367711.666666}} & \textcolor{\myred}{\snum{9748577539.11111}} &   {\snum{7883183997.666667}} & \snum{7609921682.888889} &   \snum{7568236436.222222}    \\
	L2\:DCM    & {\snum{20227011.777777776}} &  \snum{20621886.333333332} &  \textcolor{\myred}{\snum{39956792.44444445}}   & \textcolor{\myblue}{\snum{10612695.222222222}} & {\snum{28602975.777777776}} & \snum{26479819.222222224} &  {\snum{16392591.777777778}} & \snum{12885043.444444444} &   \snum{12753814.333333334}    \\
	\bottomrule
	\end{tabular}
	\label{table:filterblogs-papi}
	\end{table}

The results from earlier sections demonstrate that \system's layout choices improve run-time performance. This section investigates {\em why} performance improves. The basic premise of \system's approach to layout optimization is to concentrate on minimizing how often a traversal needs to backtrack or skip ahead while processing a buffer. By minimizing this jumping around, we expect to see improvements from two possible sources. First, we expect to see an improvement in instruction counts, as an optimized layout should do less pointer chasing. Second, we expect to see an improvement in L2 and L3 cache utilization: both fewer misses (due to improved spatial locality and prefetching) and fewer accesses (due to improved locality in higher level caches).

Table~\ref{table:filterblogs-papi} shows that our main hypothesis is borne out and the optimal layout has fewer
%To substantiate this hypothesis we collect performance counters for various layouts
%L3 accesses and L3 misses:
L2 data cache misses%
\footnote{Since PAPI, the processor counters framework, does not completely support latest AMD processors yet, we were unable to obtain L3 cache misses, only the L2 DCM counter was available.}:
a better layout promotes better locality. Interestingly, we do not observe a similar effect for instruction count. While different layouts differ in instruction counts, the difference is slight. We suspect this light effect of a better layout may be due to \gibbon's current implementation, which often dereferences pointers even if a direct access in the buffer would suffice.

\subsection{Tradeoffs between \system's solver and greedy optimization}%
\label{subsec:heuristic-tradeoffs}

To understand the difference between the layout chosen by \systemSolver and \systemGreedy we now take a closer look at the tag search traversal shown in Table~\ref{table:blog-traversals}.
Here, both versions choose two different layouts with different performance implications. \systemSolver chooses the layout \textbf{\textit{tbchiad}} whereas \systemGreedy chooses 
the layout \textbf{\textit{tcbhiad}}. The mechanics of why can be explained using our running example (Figure~\ref{fig:blog-traversal}) which is essentially a simplified version of the 
traversal shown in the evaluation. Figure~\ref{graph:running-access} shows the access graph for this traversal. \systemSolver generates constraints 
outlined in Section~\ref{design:genconstraints} that lead to the layout \textbf{\textit{tbchiad}}. On the other hand, \systemGreedy starts at the root node of the graph and greedily chooses the next child to traverse. 
The order in which nodes of the graph are visited fixes the order of fields in the data constructor. In this case, the root node is \lstinline|HashTags| which makes it the first field in the greedy 
layout, next, the greedy heuristic picks the \lstinline|Content| field making it the second field and finally followed by the \lstinline|BlogList| field.

In \figref{table:compiletimes} (p.~\pageref{table:compiletimes}), we show the compile times for different layout and traversal combinations when compiled with \gibbon, \systemGreedy and \systemSolver respectively as
a measure of relative costs. The compile times for \systemSolver include the time to generate the control flow graph, the field access graph, the solver time and the time to re-order the datatype in the code.
The solver times are in the order of the number of fields in a data constructor and not the program size. Hence, the solver adds relatively low overhead.
Since the compiler does an IO call to the python solver, there is room for improvement in the future to lower these times. 
For instance, we could directly perform \textit{FFI} calls to the CPLEX solver by lowering the constraints to C code. 
This would be faster and safer than the current implementation. In addition, during the global optimization, we call the solver on each data constructor as of the moment, 
we could further optimize this by sending constraints for all data constructors at once and doing just one solver call. 

Although the cost of \system's solver based optimization is higher than the greedy approach, it is a complementary approach 
which may help the user find a better layout at the cost of compile time. On the other hand, if the user wishes to optimize 
for the compile time, they should use the greedy heuristic.


\subsection{Discussion: Scale of Evaluation}%
\label{subsec:scale-eval}

\system's approach for finding the best layout for densely presented
data is language agnostic, but the evaluation has to be language specific.
Hence, we implemented the approach inside a most-developed (to our
knowledge) compiler supporting dense representations of recursive datatypes, the
Gibbon compiler. Our evaluation is heavily influenced by this.

At the time of writing, the scale of evaluation is limited by a number of
Gibbon-related restrictions.
Gibbon is meant as a tree traversal accelerator~\cite{gibbon} and
its original suite of benchmarks served as a basis and inspiration for
evaluation of \system.
``Big'' end-to-end projects (e.g. compilers, web servers, etc.)
have not been implemented in Gibbon and, therefore, are out of reach for us.
If someone attempted to implement such a project using Gibbon,
they would have to extend the compiler to support many realistic features:
modules, FFI, general I/O, networking.
Alternatively, one could integrate Gibbon into an existing realistic compiler
as an optimization pass or a plugin.
For instance, the Gibbon repository has some preliminary work for integrating as a
GHC plugin\footnote{%
  \url{https://github.com/iu-parfunc/gibbon/tree/24c41c012a9c33bff160e54865e83a5d0d7867dd/gibbon-ghc-integration}
}, but it is far from completion.
In any case, the corresponding effort is simply too big.
%
%Overall, we do not see a feasible way to offer a larger-scale evaluation.
Overall, the current \system evaluation shows that our approach is viable.


==> figures/blog-polymorphic.tex <==
\begin{lstlisting}
    type BlogList = [Blog]
    data Blog = Blog Content HashTags
\end{lstlisting}


==> figures/table-bench-trees.tex <==
\begin{table}
    \small
    \setlength{\tabcolsep}{4pt} %% default is 6pt
    \centering
	\caption{Run-time mean and 95\% confidence interval (ub, lb) for different
      layouts and traversal orders in the binary tree benchmarks (seconds).
              \misalignedPre{} -- post-order traversal on the pre-order layout of the tree.
              \misalignedPost{} -- pre-order traversal on the post-order layout of the tree.
              \alignedPre{} -- pre-order traversal on the pre-order layout of the tree.
              \alignedIn{} -- in-order traversal on an in-order layout of the tree.
              \alignedPost{} -- post-order traversal on the post-order layout of the tree.
              }
    \begin{tabular}{@{}lrrrrrrr@{}}
        \toprule
        \multirow{2}[2]{*}{\thead[l]{Benchmark\\name}}
        & \multicolumn{5}{c}{{\gibbon}}
        & \multicolumn{2}{c}{{\system}}\\
        \cmidrule(lr){2-6}\cmidrule(lr){7-8}
        & \multicolumn{1}{c}{\scriptsize{\misalignedPre}}
        & \multicolumn{1}{c}{\scriptsize{\misalignedPost}}
        & \multicolumn{1}{c}{\scriptsize{\alignedPre}}
        & \multicolumn{1}{c}{\scriptsize{\alignedIn}}
        & \multicolumn{1}{c}{\scriptsize{\alignedPost}}
        & \multicolumn{1}{c}{\scriptsize{\systemGreedy}}
        & \multicolumn{1}{c}{\scriptsize{\systemSolver}}\\
     \midrule
      \thead[l]{%
        \benchname{AddOneTree}
		\\\vspace{0cm}}
            & \thead{\textcolor{\myred}{{45.51}}\\ \scriptsize{(45.35, 45.66)}}
            &   \thead{memory\\error}
            &   \thead{{{1.29}}\\ \scriptsize{(1.29, 1.29)}}
    		&   \thead{{{1.30}}\\ \scriptsize{(1.30, 1.30)}}
    		&   \thead{{{1.29}}\\ \scriptsize{(1.29, 1.29)}}
    		&   \thead{{{1.29}}\\ \scriptsize{(1.29, 1.29)}}
            &   \thead{\textcolor{\myblue}{{1.28}}\\ \scriptsize{(1.28, 1.28)}}
            \\
      \thead[l]{%
        \benchname{ExpTree}
		\\\vspace{0cm}}
            & \thead{\textcolor{\myred}{{45.52}}\\ \scriptsize{(45.34, 45.70)}}
            &   \thead{memory\\error}
            &  \thead{{\fnumtwo{1.3119424788732397}}\\ \scriptsize{(\fnumtwo{1.3118021074983999}, \fnumtwo{1.3120828502480795})}}
    		&   \thead{{\fnumtwo{1.3128224647887325}}\\ \scriptsize{(\fnumtwo{1.312729018973989}, \fnumtwo{1.312915910603476})}}
    		&   \thead{{\fnumtwo{1.2938285633802817}}\\ \scriptsize{(\fnumtwo{1.2937382563056141}, \fnumtwo{1.2939188704549494})}}
    		&   \thead{{\fnumtwo{1.3117947323943662}}\\ \scriptsize{(\fnumtwo{1.311661357137603}, \fnumtwo{1.3119281076511293})}}
            &   \thead{\textcolor{\myblue}{\fnumtwo{1.292822605633803}}\\ \scriptsize{(\fnumtwo{1.2919551360395027}, \fnumtwo{1.2936900752281033})}}
            \\
      \thead[l]{%
        \benchname{CopyTree}
		\\\vspace{0cm}}
            & \thead{\textcolor{\myred}{{45.52}}\\ \scriptsize{(45.37, 45.67)}}
            &   \thead{memory\\error}
            &  \thead{{\fnumtwo{1.2870960563380283}}\\ \scriptsize{(\fnumtwo{1.286875053013491}, \fnumtwo{1.2873170596625656})}}
    		&   \thead{{\fnumtwo{1.2969579436619716}}\\ \scriptsize{(\fnumtwo{1.2967934277469406}, \fnumtwo{1.2971224595770026})}}
    		&   \thead{{\fnumtwo{1.2786742816901409}}\\ \scriptsize{(\fnumtwo{1.2785930976634212}, \fnumtwo{1.2787554657168605})}}
    		&   \thead{{\fnumtwo{1.2858431830985915}}\\ \scriptsize{(\fnumtwo{1.2857585274482104}, \fnumtwo{1.2859278387489725})}}
            &   \thead{\textcolor{\myblue}{\fnumtwo{1.2766249295774648}}\\ \scriptsize{(\fnumtwo{1.2765012665588478}, \fnumtwo{1.2767485925960818})}}
            \\
    \bottomrule
    \end{tabular}
    \label{table:Add-one-Tree}
    \label{table:Exponentiation-Tree}
	\label{table:Copy-Tree}
\end{table}


==> formal_grammar.tex <==


\begin{displaymath}
  \begin{aligned}
  &\DC \in \; \textup{Data Constructors},\:\: \TYP \in \; \textup{Type Constructors},\\
  &\var, \yvar,\fvar \in \; \textup{Variables},\:\:
  \loc, \locreg{l}{r} \in \; \textup{Symbolic Locations},\\
  &\reg \in \; \textup{Regions},\:\: \ind, \indj \in \; \textup{Region Indices},\\
  &\concreteloc{r}{i}{l} \in \; \textup{Concrete Locations}
  \end{aligned}
\end{displaymath}
\begin{displaymath}
  \begin{aligned}
    \textup{Top-Level Programs} && \PROG && \gramdef & \vectorize{\DD} \;; \vectorize{\FD} \;; \EXPR \\
    \textup{Field of a Data Constructor} && \fields && \gramdef & \sTYP  \\
    \textup{Datatype Declarations} && \DD && \gramdef & \DATA\;\TYP = \vectorize{\DC \; \vectorize{\fields}\;} \\
    \textup{Function Declarations} && \FD && \gramdef & \fvar : \TS ; \fvar \vectorize{\var} = \EXPR \\
    %\textup{Data Location} && \RP && \gramdef & \loc^{\reg} \\
%    \textup{Types} && \TYP && \gramdef & \ldots \gramor \TC \gramor \ldots \\
    %\gramor \ldots \\ % maybe don't even talk about int, is it confusing to have non-packed data?
    \textup{Located Types} && \hTYP && \gramdef & \tyatlocreg{\TYP}{\loc}{\reg} \\
    \textup{Type Scheme} && \TS && \gramdef &
      \forall _{\vectorize{\locreg{l}{r}}}.
      \vectorize{\hTYP} \ARROW \hTYP \\
    \textup{Values} && \VAL && \gramdef & \var \gramor \concreteloc{\reg}{\ind}{\locreg{\loc}{\reg}}\\
    \textup{Expressions} && \EXPR && \gramdef & \VAL\\[-5pt]
    && && \gramor & \fapp{\vectorize{\locreg{l}{r}}}{\vectorize{\VAL}} \\
    && && \gramor & \datacon{\DC}{\keywd{\locreg{\loc}{\reg}}}{\vectorize{\VAL}}\\
    %% && && \gramor & \datacon{\DC}{\keywd{\locreg{\loc}{\reg}}}{\overline{\var}} \gramor \litcon{\locreg{\loc}{\reg}}{\EXPR} \\
    && && \gramor & \letpack{\var:\hTYP}{\EXPR}{\EXPR} \\
    && && \gramor & \letloc{\locreg{\loc}{\reg}}{\LE}{\EXPR} \\
    && && \gramor & \letreg{\reg}{\EXPR} \\
    && && \gramor & \case{\VAL}{\vectorize{\pat}} \\
    \textup{Pattern} && \pat && \gramdef &
    \caseclause{\datacon{\DC}{}{(\vectorize{\var : \hTYP})}}{\EXPR} \\
    \textup{Location Expressions} && \LE && \gramdef
    & \startr{\reg} \\
    && && \gramor & (\locreg{\loc}{r} + 1) \\
    && && \gramor & \afterl{\hTYP}   \\        
    \textup{Copying Calls} && \cpy && \gramdef & \copyPacked{\var:\hTYP}
  \end{aligned}
\end{displaymath}


==> formal_grammar2.tex <==


\begin{displaymath}
  \begin{aligned}
  &\DC \in \; \textup{Data Constructors},\:\: \TYP \in \; \textup{Type Constructors},
  \:\: \var, \yvar,\fvar \in \; \textup{Variables}%% ,\:\:
%%   \loc, \locreg{l}{r} \in \; \textup{Symbolic Locations},\\
%%   &\reg \in \; \textup{Regions},\:\: \ind, \indj \in \; \textup{Region Indices},\\
%%   &\concreteloc{r}{i}{l} \in \; \textup{Concrete Locations}
  \end{aligned}
\end{displaymath}
\begin{displaymath}
  \begin{aligned}
    \textup{Top-Level Programs} && \PROG && \gramdef & \vectorize{\DD} \;; \vectorize{\FD} \;; \EXPR \\
    \textup{Field of a Data Constructor} && \fields && \gramdef & \sTYP  \\
    \textup{Datatype Declarations} && \DD && \gramdef & \DATA\;\TYP = \vectorize{\DC \; \vectorize{\fields}\;} \\
    \textup{Function Declarations} && \FD && \gramdef & \fvar : \vectorize{\TYP} \ARROW \TYP ; \fappnoloc{\vectorize{\var}} = \EXPR \\
    %% \textup{Located Types} && \hTYP && \gramdef & \tyatlocreg{\TYP}{\loc}{\reg} \\
%%     \textup{Type Scheme} && \TS && \gramdef &
%%       \forall _{\vectorize{\locreg{l}{r}}}.
%%       \vectorize{\hTYP} \ARROW \hTYP \\
    \textup{Values} && \VAL && \gramdef & \var \\ %% \gramor \concreteloc{\reg}{\ind}{\locreg{\loc}{\reg}}
    \textup{Expressions} && \EXPR && \gramdef & \VAL\\[-5pt]
%%     && && \gramor & \fappnoloc{\vectorize{\VAL}} \\
%%     && && \gramor & \dataconnoloc{\DC}{\vectorize{\VAL}}\\
%%     && && \gramor & \copynoloc{\vectorize{\VAL}}\\
    && && \gramor & \letpack{\var:\TYP}{\fappnoloc{\vectorize{\VAL}}}{\EXPR} \\
    && && \gramor & \letpack{\var:\TYP}{\dataconnoloc{\DC}{\vectorize{\VAL}}}{\EXPR} \\
%%     && && \gramor & \letloc{\locreg{\loc}{\reg}}{\LE}{\EXPR} \\
%%     && && \gramor & \letreg{\reg}{\EXPR} \\
    && && \gramor & \case{\VAL}{\vectorize{\pat}} \\
    \textup{Pattern} && \pat && \gramdef &
    \caseclause{\datacon{\DC}{}{(\vectorize{\var : \TYP})}}{\EXPR} \\
%%     \textup{Location Expressions} && \LE && \gramdef
%%     & \startr{\reg} \\
%%     && && \gramor & (\locreg{\loc}{r} + 1) \\
%%     && && \gramor & \afterl{\hTYP}   \\        
%%     \textup{Copying Calls} && \cpy && \gramdef & \copyPacked{\var:\hTYP}
  \end{aligned}
\end{displaymath}


==> haskell_style.tex <==

\usepackage{upquote}
\usepackage{listings}
% This is used in the acmart.cls, leading to problems with option clash:
% \usepackage[usenames,dvipsnames]{xcolor}
% \usepackage[dvipsnames]{xcolor}
\usepackage[]{xcolor}

% [2017.01.16] Work around option clash:
\definecolor{MidnightBlue}{rgb}{0.1, 0.1, 0.44}
\definecolor{Bittersweet}{rgb}{1.0, 0.44, 0.37}
\definecolor{Cinnamon}{rgb}{0.82, 0.41, 0.12}
\definecolor{ForestGreen}{rgb}{0.0, 0.27, 0.13}
\definecolor{Gray}{rgb}{0.5, 0.5, 0.5}
\definecolor{RoyalPurple}{rgb}{0.47, 0.32, 0.66}
\definecolor{Maroon}{rgb}{0.5, 0.0, 0.0}
\definecolor{OtterBrown}{rgb}{0.4, 0.26, 0.13}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{blush}{rgb}{0.87, 0.36, 0.51}

\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkred}{rgb}{0.5,0,0}
\definecolor{darkbrown}{rgb}{0.4, 0.26, 0.13}

\definecolor{hsblue}{HTML}{2d3497}
\definecolor{hsgreen}{HTML}{3f7e32}
%% \renewcommand{\ttdefault}{txtt}

%% emacs color scheme
\definecolor{emacspink}{HTML}{a241f6}
\definecolor{emacsgreen}{HTML}{3c8625}
\definecolor{emacsbrown}{HTML}{a86a2c}
\definecolor{emacsblue}{HTML}{1b38f5}


% Define the language styles we will use
%
\lstset{%
    frame=none,
    rulecolor={\color[gray]{0.7}},
    numbers=none,
    basicstyle=\footnotesize\ttfamily,
    %% basicstyle=\scriptsize\ttfamily,
    numberstyle=\color{Gray}\tiny\it,
    commentstyle=\color{Maroon}\it,
    stringstyle=\color{Maroon},
    keywordstyle={[1]},
    keywordstyle={[2]\color{emacsbrown}},
    keywordstyle={[3]\color{OtterBrown}},
    keywordstyle=[4]\color{RoyalPurple},
    keywordstyle={[5]\color{emacspink}},
    keywordstyle={[6]\color{emacsgreen}},
    captionpos=b,
    aboveskip=1\medskipamount,
    xleftmargin=0.5\parindent,
    xrightmargin=0.5\parindent,
    flexiblecolumns=false,
%   basewidth={0.5em,0.45em},           % default {0.6,0.45}
%    escapechar={\%},
    escapechar={\@},
    mathescape=true,
    texcl=true,                          % tex comment lines
    showstringspaces=false
}

\lstloadlanguages{Haskell}
\lstdefinestyle{haskell}{%
    language=Haskell,
    upquote=true,
    backgroundcolor=\color{white},
    deletekeywords={case,class,data,default,deriving,do,in,instance,let,of,type,where,IO,ST,STM,if,then,else,tail,List,Int},
    morekeywords={[5]class,data,default,deriving,family,instance,type,where,fun,while,global,return,match,for},   morekeywords={[5]in,let,case,of,do,letpacked,letloc,letregion,start,after,if,then,else,spawn,sync,sizeof,cilk_spawn,cilk_sync,continuation_stolen, size_of,tie,addrOf},
    morekeywords={[4]IORef,IO,ST,STM,STRef,TVar},
    morekeywords={[6]Cons,Nil,Int,List,RNG,Ind,Node,Leaf,Empty},
    %% morekeywords={[5]spawn,sync,sizeof,cilk_spawn,cilk_sync,continuation_stolen},
    literate=
        %% {\\}{{$\lambda$}}1
        {::}{{\textcolor{emacsbrown}{::}}}2
        {=}{{\textcolor{emacsbrown}=}}1
        {Lambda}{{$\Lambda$}}1
        {\\\\}{{\char`\\\char`\\}}1
        {>->}{{>->}}3
        {>>=}{>>=}3
        {->}{{$\rightarrow$}}2
        {>=}{{$\geq$}}2
        {<-}{{$\leftarrow$}}2
        {<=}{{$\leq$}}2
        {=>}{{$\Rightarrow$}}2
        {|}{{\textcolor{emacsbrown}{$\mid$}}}1
        {forall}{{{$\pmb{\forall}$}}}1
        {exists}{{$\exists$}}1
        {...}{{$\cdots$}}3        
%       {`}{{\`{}}}1
%       {\ .}{{$\circ$}}2
%       {\ .\ }{{$\circ$}}2
%
%    deletekeywords={insert},
%    deletekeywords={map,sort,zipWith,replicate,Num,Char,Bool,Array,Int,Double
%                   ,sqrt,not,filter,IO,Maybe,Either,quot,scanl,scanr,reverse,fst,id},
%    literate=
%        {+}{{$+$}}1
%        {/}{{$/$}}1
%        {*}{{$*$}}1
%        % {=}{{$=$}}1
%        {>}{{$>$}}1 {<}{{$<$}}1
%        {\\}{{$\lambda$}}1
%        {\\\\}{{\char`\\\char`\\}}1
%        {->}{{$\rightarrow\;$}}2
%        {>=}{{$\geq$}}2
%        {<-}{{$\leftarrow\;$}}2
%        {<=}{{$\leq$}}2
%        {=>}{{$\Rightarrow\;$}}2
%        {\ .}{{$\circ$}}2
%        {\ .\ }{{$\circ$}}2
%        {>>}{{>>}}2
%        {>>=}{{>>=}}2
%        {=<<}{{=<<}}2
%        {|}{{$\mid$}}1
%        {dotdotdot}{{$\ldots$}}3
}

\lstdefinestyle{inline}{%
    style=haskell,
    basicstyle=\footnotesize\ttfamily,
    %% keywordstyle=[1],
    %% keywordstyle=[2],
    %% keywordstyle=[3],
    %% keywordstyle=[4],
    escapechar={\@},
    mathescape=true,
    literate=
        {\\}{{$\lambda$}}1
        {Lambda}{{$\Lambda$}}1        
        {\\\\}{{\char`\\\char`\\}}1
        {>->}{>->}3
        {>>=}{>>=}3
        {->}{{$\rightarrow$\space}}3    % include forced space
        {>=}{{$\geq$}}2
        {<-}{{$\leftarrow$}}2
        {<=}{{$\leq$}}2
        {=>}{{$\Rightarrow$}}2
        {|}{{$\mid$}}1
%        {~}{{$\sim$}}1
        {forall}{{$\forall$}}1
        {exists}{{$\exists$}}1
        {...}{{$\cdots$}}3
}

\lstnewenvironment{code}
    {\lstset{style=haskell}%
      \csname lst@SetFirstLabel\endcsname}
    {\csname lst@SaveFirstLabel\endcsname}
    {}

% Default all listings to Haskell style
\lstset{style=haskell}

% \newcommand{\inl}[1]{\lstinline[style=inline];#1;}
\newcommand{\il}[1]{\lstinline[style=inline,mathescape=true];#1;}

\newcommand{\makeatcode}{\lstMakeShortInline[style=inline]@}
\newcommand{\makeatchar}{\lstDeleteShortInline@}

\lstloadlanguages{C}
\lstdefinestyle{c}{%
    language=C,
    upquote=true,
    escapechar={\@},
    deletekeywords={typedef,struct,char,return,if,else},
    morekeywords={[5]typedef,struct,return,if,else},
    morekeywords={[6]Location,shadowstack_frame,ShadowstackFrame,
                     GibCursorProd3,GibCursor,GibBool,GibInt,GibPackedTag,GibCursorProd3_struct,
                     uint8_t, int64_t, bool, char,uint32_t
                     },
}

\newcommand{\ilc}[1]{\lstinline[style=c,mathescape=true];#1;}

\lstnewenvironment{ccode}
    {\lstset{style=c}%
      \csname lst@SetFirstLabel\endcsname}
    {\csname lst@SaveFirstLabel\endcsname}
    {}

% \lstloadlanguages{Rust}
% \lstdefinestyle{Rust}{%
%     language=Rust,
%     upquote=true,
%     deletekeywords={typedef,struct,type,static,enum},
%     morekeywords={[5]typedef,type,static,struct,enum},
%     morekeywords={[6]DataconEnv,DatatypeEnv,DataconInfo,DatatypeInfo,Scalar,Packed,InfoTable},
% }

% \lstnewenvironment{rustcode}
%     {\lstset{style=Rust}%
%       \csname lst@SetFirstLabel\endcsname}
%     {\csname lst@SaveFirstLabel\endcsname}
%     {}

% \newcommand{\ilr}[1]{\lstinline[style=Rust,mathescape=true];#1;}


==> intro.tex <==
\section{Introduction}

%% \note{ Fortunately, programmers need not worry about the placement of
%%   data in memory: variables and fields are ordered statically by the
%%   compiler, and linked structures use pointers and are ordered
%%   in the heap by a runtime allocator.
%%   %
%%   Yet this tradition is rigid in its static/dynamic boundary, and
%%   inflexible in where shortcut occurs, with little or no {\em
%%     compile-time information} informing {\em runtime allocation} and
%%   placement.}
  
   
%% \note{Compilers optimize code, but usually data representations are
%%   fixed. Changing the data representation to fit the way the data is
%%   consumed in a specific program is an underexplored area.}

%% \note{One place where this underexplored area is brought to the fore
%%   is when considering denser (serialized) representations of data.
%%   %
%%   High level languages hide the data representation and in fact use
%%   inefficient, boxed representations: a kind of
%%   lowest-common-denominator representation that makes things easy for
%%   the compiler but is rarely the absolute most efficient.
%%   %
%%   If we want dense data, today we can write error prone low-level
%%   code.  Or, recently, we gained the ability to use the Gibbon
%%   compiler, which introduces compiler-optimized serialization, but is
%%   still inflexible with respect to {\em data ordering}.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% When programmers write code, they rely on compilers to
% % optimize many aspects of the code
% make the low level decisions: which instructions to select, when instructions are scheduled to improve register and cache usage, where variables are placed on the stack, etc.
% %
% But one area where programmers typically cannot rely on compiler support is in creating efficient data representations for complex data structures.
% %
% While a compiler might tweak field placement in a structure to improve memory alignment, basic decisions like field ordering are typically chosen to simplify code generation rather than with an eye to efficiency.
% %
% In high level languages, where data is ``boxed'', elements in a structure may, indeed, be scattered throughout memory due to the decisions of runtime memory allocators.
% %
% The problem is compounded with recursive, heap-allocated data structures: a program that simply traverses a linked list may ultimately hop randomly through memory, destroying cache locality and obviating the benefits of hardware prefetchers.
% %
% The performance difference between a data layout that is well-matched to a program's access patterns and one that is not can be vast.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Over the years, there has been some work exploring the space of more-intelligent data representations, tackling the problem from different angles.
% %
% Some work targets memory management, making either memory allocation~\cite{poolallocation} or copying garbage collectors~\cite{ccgarbage} sensitive to program behavior, allowing object locations to match access patterns.
% %
% Other work modifies structure layouts to re-order fields and influence placement decisions~\cite{truong,CSL,CSD}.
% %
% However, these approaches only tackle one aspect of data representation---where objects are located---and primarily target non-recursive structures.
% %
% Further, they fundamentally operate at the level of boxed data, requiring pointer chasing to access non-primitive data.
% %
% When processing recursive, linked data structures, such approaches cannot (and do not attempt to) improve the efficiency of program by placing elements of data structures in such a way so as to improve traversal efficiency.
% \mk{I don't feel great about this last sentence...}
% \vs{changed this a bit.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Recent work has tackled this problem from another direction: the Gibbon language and whole-program compiler~\cite{gibbon, Local} focuses on the problem of chasing pointers haphazardly through memory when accessing recursive, linked structures.
% %
% Gibbon produces {\em dense}, {\em packed} representations of algebraic datatypes where {\em unboxed} data is accessed directly, without pointer chasing.
% %
% For example, tree data will be serialized in pre-order into a buffer, and traversing the tree (e.g., to sum all of its elements) will result in, essentially, a linear scan of an array, resulting in no pointer dereferencing and highly-efficient, predictable access patterns.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Gibbon has many benefits: programmers no longer need to take control of low-level data representation and allocation to serialize linked structures; and rather than writing error-prone index math to access data, the Gibbon compiler automatically translates idiomatic data structure accesses into operations on the serialized representation.
% %
% However, Gibbon suffers from drawbacks complementary to the other approaches mentioned above.
% %
% It does not attempt to match data layout to the access patterns of a program.
% %
% If the particular serialization decisions for a datatype chosen by Gibbon do not correspond to the behavior of functions accessing that data, then pathological behavior can result.
% %
% Consider a tree laid out in left-to-right pre-order with a program that accesses that tree right-to-left.
% %
% Rather than scanning straightforwardly through the structure, the program would have to jump back and forth through the buffer to access the necessary data.
% %
% When encountering such cases, Gibbon does not break: instead, it inserts {\em shortcut pointers} to allow more-random access to structures~\cite{Local}.
% %
% But this defeats the purpose of a dense, packed representation: not only are accesses no longer nicely strided through memory, but the pointers and pointer-chasing of boxed data have returned.
% %
% Indeed, when Gibbon is presented with a program whose access patterns do not match the chosen data layout, the generated code can be {\em significantly slower} than plain, pointer-based representations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% What we want is the best of both worlds: Gibbon's dense, packed data layouts combined with access pattern--aware decisions of {\em how} to lay out that data.
% %
% %
% To that end, this paper introduces \system, an extension of the Gibbon compiler that creates dense, packed data representations that match the way a program accesses that data. \system can also reason about recursive fields in a way that prior work cannot. Since the data we operate on is packed, \system has insights on how to place recursive fields such that it aids traversal performance.

Recursive data structures are
% popular in many domains and are
readily available in most programming languages. Linked lists, search trees, tries and others
provide efficient and flexible solutions to a wide class of problems---both in low-level languages with direct
memory access (C, \cpp, Rust, Zig) as well as high-level ones (Java, \csharp, Python).
Additionally, in the purely functional (or {\em persistent}~\cite{okasaki}) setting, recursive,
tree-like data structures largely replace array-based ones.
%
Implementation details of recursive data structures are not necessarily known to
application programmers, 
%% The clients of libraries containing recursive data structures
%% % only get access to convenient APIs
%% often access them through a high-level container API,
who can only hope that the library authors and the
compiler
% optimize extensively to
achieve good performance.
Sadly, recursive data structures are a hard optimization target.

% The hope for a good performance of recursive data structures is limited in

High-level languages represent recursive structures with pointers to small
objects allocated sparsely on the heap. An algorithm traversing such a
\emph{boxed} representation spends much time in pointer
chasing, which is a painful operation for
modern hardware architectures. Optimizing compilers for these languages and architectures have
many strengths but optimizing memory representation of user-defined data
structures is not among them. One alternative is resorting to manual memory
management to achieve maximum performance, but it has the obvious drawback of
leaving convenience and safety behind.
% Is there another alternative?

A radically different approach is representing recursive datatypes as dense structures
(basically, arrays) \new{with the help of a library or compiler}.
% has been studied recently.
% \ap{TODO: add citations}
% \mv{not many citations beyond Gibbon for recursive data packed into arrays}
% \mk{If Gibbon is the only real example, I'm dropping ``for example'' from the next sentence...}
The \gibbon{} compiler tries to improve the performance of recursive data
structures by embracing dense representations by default~\cite{gibbon}. This choice has
practical benefits for programmers: they no longer need to take control of
low-level data representation and allocation to serialize linked structures; and
rather than employing error-prone index arithmetic to access data, they let \gibbon{}
automatically translate idiomatic data structure accesses into operations on
the dense representation.

Dense representations are not a panacea, though. They can suffer a complementary problem due to their inflexibility.
A particular serialization decision for a data structure made by the compiler
can misalign with the behavior of functions accessing that data.
%
Consider a tree laid out in left-to-right pre-order with a program that accesses that tree right-to-left.
%
Rather than scanning straightforwardly through the structure, the program would have to jump back and forth
through the buffer to access the necessary data.

One way to counter the inflexibility of dense representations is to introduce
some pointers.
For instance, \gibbon{} inserts {\em shortcut pointers} to allow random access to recursive structures~\cite{Local}.
%
But this defeats the purpose of a dense representation: not only are
accesses no longer nicely strided through memory, but the pointers and pointer
chasing of boxed data are back.
%
Indeed, when \gibbon{} is presented with a program whose access patterns do not match the chosen data layout,
the generated code can be {\em significantly slower} than a program with favorable access patterns. 

Are we stuck with pointer chasing when processing recursive data structures?
% This paper argues ``no'';
We present \system{} as a counter example. \system{} is our program analysis
and transformation approach that spots misalignments of algorithms and data
layouts and fixes them where possible. Thus, our slogan is:
\begin{quote}
Algorithms + Data Layouts = Efficient Programs
\end{quote}

% Artem: not a fan of this paragraph below. It repeats things that are also
% mentioned below. It's too detailed for giving the first impression. And it's
% too gibbon-specific in the second point.
% \system's key insight is twofold.
% %
% First, that a compile-time analysis can yield insights into how a program is {\em likely} to access the fields of a data structure, including recursive traversal patterns.
% %
% Second, that Gibbon's dense, serialized representation is ideal for taking advantage of this access information.
% %
% Gibbon's compilation strategy~\cite{Local} makes explicit when field references will result in sub-optimal access patterns, making it possible to statically estimate the costs of different layout choices.
% %
% This cost model can be used to drive a search process for a minimum-cost layout, subject to any additional constraints provided by the programmer.

\system analyzes the data access patterns of a program and synthesizes a data layout that corresponds to that behavior.
%
It then rewrites the datatype and code to produce more efficient code that
operates on a dense data representation in a way that matches access patterns.
This co-optimization of datatype and code results in improved locality and, in the context of \gibbon,
avoidance of shortcut pointers as much as possible.

We implement \system{} as an extension to \gibbon---a
compiler based on dense representations of datatypes.
% including extending the source language to support (optional) layout hints.
% Artem: ^^--this is not implemented so let's not tlak about it just yet.
That way, \system can be either a transparent compiler optimization, or semi-automated tool for exploring different layouts during the programmer's optimization work.
%
% Our approach is fairly general:
Our approach has general applicability because of the minimal and common nature of the core language:
%
the core language of \system (\figref{fig:grammar})
is a simple first-order, monomorphic, strict, purely functional language.
Thanks to the succinct core language,
we manage to isolate \system from \gibbon-specific, complicated (backend) mechanics of converting a program
to operate on dense rather than boxed data.
%
% Artem: vv--this is too much Gibbonn-specific detail that will scare reviewers.
% Rather, in terms of phase ordering, \system does its work early in the compiler, after monomorphization, but before explicit regions-and-pointer-arithmetic serialization transformations.
%

%% We show across several microbenchmarks, as well as on a larger case study of a blog management service, that \system finds optimal data structure layouts,.
%% %
%% \system-generated programs outperform alternative Gibbon layouts for the same program, as well as optimized GHC implementations.

Overall, in this paper:
\begin{itemize}
\item We provide a static analysis capturing the temporal access patterns of a
  function towards a datatype it processes. As a result of the analysis, we
  generate a {\em field access graph} that summarizes these patterns.

\item We define a cost model that, together with the field access graph, enables
  formulating the field-ordering optimization problem as an integer linear program.
  We apply a % commercially available % Artem: I don't see why it's relevant that
            % it's proprietary. If anything, that's a downside that I wouldn't
            % put forward.
  linear solver to the problem and obtain optimal positions of fields in the
  datatype definition relative to the cost model.
  %, consistent with any constraints provided by the programmer.
  % Artem: ^^-- obvious
  
\item We extend the \gibbon{} compiler to synthesize new datatypes based on the
solution to the optimization problem, and transform the program to use these new,
optimized types, adjusting the code where necessary.
  
\item Using a series of benchmarks, we show that our implementation, \system,
  can provide speedups of 1.14
  % \lstinline|rightmost| tree traversal
  to 54 times
  %for a simple \lstinline|length| function on a \lstinline|List|)
  over the best prior work on dense representations, \gibbon.
%
% through our evaluation on a realistic blog software application
% Artem: ^^-- I wouldn't call it realistic, and OOPSLA reviewers too.
%
  \new{\system outperforms \mlton on these same benchmarks by a factor of 1.6 to 38.}
  %, a strict 
  %compiler targeting Standard ML.}
  % On the same benchmarks, \system outperforms the standard Haskell compiler GHC,
  % which uses boxed representations, when compiling in strict \new{(call-by-value)} mode
  % 3 to 6 times.
  %% .\mv{Can we be more precise here? Like, not \emph{everything} is boxed in Haskell}.

%% \item \system can automatically generate the different permutations of the
%%   algebraic datatype in a type safe way. In addition, it allows the programmer
%%   to manually specify these constraints thereby making it easy for the
%%   programmer to conform the data to their specifications.
\end{itemize}


%% \section*{OLD INTRO}

%% \mk{Material to cut starts here}
%% When programmers write programs, they do not necessarily think
%% about the \new{location} of the corresponding data in memory. The
%% layout of data is mostly an implementation detail left for the
%% language runtime to handle. For this reason, programmers are
%% agnostic to the combinative effects of the structural properties of
%% the code (i.e, control flow and data access patterns) to the in
%% memory \new{layout} of the data which does not guarantee optimal
%% performance due to the memory hierarchy in modern architectures.

%% This gap in knowledge in conjunction with the difficulty to reason about the particular choices of transformations (either in the source code, or the in-memory layout of data) makes writing optimal code a tough challenge. Most languages resort to allocating data through pointers by utilizing libraries like \textit{malloc} which rely on system calls like \textit{sbrk or mmap} under the hood to allocate data. Although this allows for relatively cheap updates in the data representation, mallocing does not provide any guarantees on whether the allocated data will exhibit good spatial locality. In addition, \textit{malloc} is completely incognizant about the structural properties of the source code and just returns the smallest memory block available in the allocation tree.

%% \mv{Need some more motivation here before jumping into discussing other papers.}

%% \mk{This paragraph is probably redundant with RW}
%% There has been work on solving this problem, by, for example, modifying data structures to promote locality~\cite{truong}, or modifying memory allocators~\cite{poolallocation} and garbage collectors to ensure objects will be placed in certain relative positions in memory.
%% Chilimbi~\etal~\cite{CSL} employ clustering and coloring techniques on data structures to identify contemporaneously accessed elements and to segregate heavily accessed with non-heavily accessed elements in non-conflicting cache regions respectively. They use this information together with a smart allocator that attempts to fit contemporaneously accessed elements in the same cache block. 

%% \mk{This paragraph is probably redundant with RW}
%% For data structures greater than half the size of the cache block, Chilimbi~\etal~\cite{CSD} introduces more techniques like structure splitting and field reordering to optimize the layout of the data structure in memory. They also utilize their cache conscious garbage collector~\cite{ccgarbage} to optimize the layout of the live objects at runtime. 

%% Although these techniques work well for pointer based programs in languages like C, we are in a different optimization space. We want to optimize the data layout of \textit{packed and recursive} algebraic datatypes in memory written in a functional programming language and for a compiler that compiles code for a functional programming language.

%% \mk{this paragraph, or the contents of it, would be good for the background.}
%% We utilize the existing lanuage LoCal~\cite{Local} (and the Gibbon compiler~\cite{gibbon}) that packs ADTs in memory and use it to reason about the optimal layout of the fields in an algebraic datatype. LoCal (short for \textit{location calculus}) \textit{eschews} the traditional pointer representation of ADTs and serializes \textit{tree-like} ADTs in memory by fixing a particular traversal order of the ADT.
%% %
%% The programmer can write various ADTs and define functions in a higher-order, polymorphic subset of Haskell. Their type system encodes a layout for an algebraic datatype in memory at the byte level. This makes it possible for the program to operate over a dense serialized representation of the data in memory in a type safe manner.
%% %
%% This dense serialized representation provides good spatial locality, however it is still limited because it does not optimize the fine grained layout of the \textit{ADT} (the fields within the datatype) to the access patterns of the fields induced by the structure of the program.

%% A major use case for Gibbon's approach to data representation is operating directly on serialized data. There are instances where applications require serializing or de-serializing data for specific purposes. Serialized data is omnipresent in file systems, where objects are converted into a stream of bytes or \textit{serialized} to be stored on disk. A \textit{deserialization} happens when there in an impedance mismatch arising from a program requiring the data to be in a specific format and the incoming data existing in an alien format.
%% %
%% Similarly, microservices architectures often rely on remote procedure calls (RPC)\footnote{Such as Thrift ({\url{https://thrift.apache.org}}), Finagle ({\url{https://twitter.github.io/finagle/}}), gRPC ({\url{https://grpc.io}})} or RESTful APIs that convert data to a specific format like JSON to serialize and deserialize data over network when sending data to other microservices.
%% %
%% By having the ability to operate directly on serialized data, it becomes much easier to bring the program closer to the data rather than mutating the data representation to fit the program~\cite{Local}; thus reducing the overhead of transforming the data from one layout to another and even avoiding expensive network calls. 

%% \mv{I don't think we need to bring up Cogent/Dargent right here. That can be in the related work section.}

%% This paper makes the following contributions:
%% \begin{itemize}
%% \item We introduce a new framework, \system, which can reason about the locally optimal layout of fields in an algebraic datatype by statically analyzing the function that consumes the ADT. By statically analyzing the control flow of the function, we generate a field access graph to capture the temporal access patterns of the ADT for that function.

%% \item We formulate the ordering of the fields as an Integer Linear Program and use a commercially available linear solver to get a mapping from fields to the optimal indices in the algebraic datatype.

%% \item We show through our evaluation on a realistic blog software application and various synthetic benchmarks that \system can provide greater speedups than the best prior work Gibbon. We also compare our implementation against GHC where all ADTs are boxed in nature.

%% \item  \system can automatically generate the different permutations of the algebraic datatype in a type safe way. In addition, it allows the programmer to manually specify these constraints thereby making it easy for the programmer to conform the data to their specifications.



%% % Another line of work, Dargent~\cite{Dargent} is a data layout descriptive language that allows programmers to specify the data layout of an algebraic datatype. It is built on top of the Cogent~\cite{o2016cogent}  language which is a first order polymorphic functional programming language. Dargent targets C code and provides proofs for formally verifying the correctness of the data layout transformations.

%% % Their work however, is set in a different environment and does not evaluate the data layout transformations in terms of performance. They do not automatically optimize their program for the best layout and neither do they support recursive algebraic datatypes.

%% \end{itemize}



==> macros.tex <==

%% Reference listings https://github.com/snowleopard/united/blob/main/paper/main.tex

\definecolor{canaryblue}{HTML}{2916F5}
\definecolor{darkgreen}{HTML}{006400}
\definecolor{darkpink}{HTML}{CD00CD}
\definecolor{graygreen}{rgb}{0.3,0.5,0.3}
\definecolor{grayblue}{rgb}{0.2,0.2,0.6}
\definecolor{grayred}{rgb}{0.5,0.2,0.2}
\definecolor{crimsonred}{HTML}{990000}
\definecolor{irishgreen}{HTML}{08A04B}
\definecolor{darkviolet}{HTML}{9400D3}
\newcommand{\myblue}{NavyBlue}
\newcommand{\myred}{BrickRed}

\lstset{
  backgroundcolor=\color{white},     % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  % identifierstyle=\color{red},
  basicstyle=\footnotesize\ttfamily,      % the size of the fonts that are used for the code
  breakatwhitespace=false,              % sets if automatic breaks should only happen at whitespace
  breaklines=false,                     % sets automatic line breaking
  captionpos=b,                         % sets the caption-position to bottom
  abovecaptionskip=-2 mm,
  commentstyle=\itshape\color{graygreen}, % comment style
  % escapeinside={(:}{:)},             % if you want to add LaTeX within your code
  escapechar={!},
  % extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  % firstnumber=1000,                % start line enumeration with line 1000
  % frame=tb,                        % adds a frame around the code
  % keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle={[1]\color{canaryblue}},     % keyword style
  keywordstyle={[2]\color{crimsonred}},
  keywordstyle={[3]\color{darkviolet}},
  keywordstyle={[4]\color{irishgreen}},
  language=Haskell,                  % the language of the code
  morekeywords={[1]Int, Float}, %primitives
  morekeywords={[2]Leaf, Node, Sub, Add, Eq, Leq, Geq, Neq, And, Or, IntType, FloatType, Boolean, Implication, Blog, Nil, HIADCTB, Empty, Cons, Snoc, Not, Val, T, E}, % data constructors
  morekeywords={[3]data, class, instance, where, type}, %some more keywords
  morekeywords={[4] F0, F1, F2, F3, F4, F5, Tree, IntExpr, FloatExpr, BoolExpr, Constraint, BlogList, Content, HashTags, Header, Id, Author, Date, Ast, Blogs, Exp},  %packed types
  deletekeywords={instance, data, where, class, filter, type, insert, delete, union, map, Eq},      % if you want to delete keywords from the given language
  numbers=none,                      % where to put the line-numbers; possible values are (none, left, right)
  % numbersep=5pt,                   % how far the line-numbers are from the code
  % numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
  % rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  % showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  % showstringspaces=false,          % underline spaces within strings only
  % showtabs=false,                  % show tabs within strings adding particular underscores
  % stepnumber=2,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{grayred},     % string literal style
  % tabsize=2,                       % sets default tabsize to 2 spaces
  % title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
  xleftmargin=2pt,
  aboveskip=2pt,
  belowskip=1pt
}


%system name
\newcommand{\system}{{\sc Marmoset}\xspace}

\newcommand{\ribbit}{{\sc Ribbit}\xspace}

\newcommand{\systemSolver}{{\sc M$_{\mathit{solver}}$}\xspace}
\newcommand{\systemGreedy}{{\sc M$_{\mathit{greedy}}$}\xspace}


\newcommand{\alignedPre}{{\sc Algn$_{\mathit{pre}}$}\xspace}
\newcommand{\alignedIn}{{\sc Algn$_{\mathit{in}}$}\xspace}
\newcommand{\alignedPost}{{\sc Algn$_{\mathit{post}}$}\xspace}


\newcommand{\misalignedPost}{{\sc Misalgn$_{\mathit{post}}$}\xspace}
\newcommand{\misalignedPre}{{\sc Misalgn$_{\mathit{pre}}$}\xspace}

\newcommand{\misalignedGen}{{\sc Misalgn}\xspace}
\newcommand{\alignedGen}{{\sc Algn}\xspace}



% \newcommand{\systemlang}[0]{MLANG}
\newcommand{\systemlang}[0]{\ensuremath{\lambda_{M}}}

\newcommand{\gibbon}{{\sc Gibbon}\xspace}

\newcommand{\relc}{{\sc RELC}\xspace}

\newcommand{\ghc}{{\sc Ghc}\xspace}

\newcommand{\mlton}{{\sc MLton}\xspace}

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}


\newcommand{\snum}[1]{{\num[round-precision=3,round-mode=figures,scientific-notation=true,output-exponent-marker = e]{#1}}}
\newcommand{\snumfour}[1]{{\num[round-precision=4,round-mode=figures,scientific-notation=true,output-exponent-marker = e]{#1}}}

\newcommand{\fnumthree}[1]{{\num[round-mode=places,round-precision=3, scientific-notation=false]{#1}}}
\newcommand{\fnumtwo}[1]{{\num[round-mode=places,round-precision=2, scientific-notation=false]{#1}}}

\def\cpp{{C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\footnotesize\bf ++}}}
\def\csharp{C\tikz[x=1em,y=\baselineskip]%
  \draw (0.125,0.15) -- ++(0.15,0.5)%
        (0.325,0.15) -- ++(0.15,0.5)%
        (0.05,0.3) -- ++(0.45,0.0)%
        (0.1,0.5) -- ++(0.45,0.0);}

% benchname style copied from lipics' style, descriptionlabel macro sans an hskip
\newcommand{\benchname}[1]{\textcolor{lipicsGray}{\sffamily\small\bfseries\mathversion{bold}#1}}


==> notes.tex <==
\section{NOTES Arena for scratch work: Remove Later!}

% \begin{abstract}
% Serialization of pointer based data structures in memory is a performance oriented optimization. When we allocate data structures in a traditional imperative language like C, the memory allocator, usually "malloc" 
% isn't guaranteed to provide space for allocation at contiguous addresses. This is not ideal since chasing pointers is known to result in poor data locality. There has been prior work (cite gibbon) that focuses on removing
% this pointer based representation of data structures like trees in memory and serialize them in a specific order (for instance, a preorder traversel). Though this results in better data locality, (the complete tree is
% serialized in a contiguous memory buffer), it is rigid when it comes to the fine-grained choice of field ordering with-in the data structure. We present a new framework where we define an ordering on the layout of the data structure. 
% This ordering helps us in maximizing performance since it can affect locality depending on the choice of traversal on that data structure. We specifically developed a blog management infrastructure where we run multiple (real world like)
% passes and showcase how the choice of field-ordering can affect the performance of these passes...
% \end{abstract}


%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>10010520.10010553.10010562</concept_id>
%   <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010575.10010755</concept_id>
%   <concept_desc>Computer systems organization~Redundancy</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010553.10010554</concept_id>
%   <concept_desc>Computer systems organization~Robotics</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10003033.10003083.10003095</concept_id>
%   <concept_desc>Networks~Network reliability</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
% \keywords{datasets, neural networks, gaze detection, text tagging}
%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

%%
%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.
%\maketitle

\subsection{Introduction}


\subsection{Problem Definition}

We want to develop an algorithm that takes some \textit{inputs} and returns some \textit{output}, based on \textit{costs and constraints}.
This algorithm should minimize these \textit{costs}.   

\subsubsection{Define inputs: }

\begin{itemize}
  \item $Input_a$: A function \textit{F} for which we want to optimize the ordering of fields $f_1$, $f_2$, $f_3$ \dots
                   for each data Constructor $d_1$, $d_2$, $d_3$, $d_4$ \dots that this function uses. Where $f_1$ is a list containing some fields used in 
                   data constructor $d_1$. 

  \item $Input_b$: A list \textit{l} where each element is a tuple (\textit{data constructor}, \textit{list(fields)}) that we 
                   want to optimize. 
                   
  \item $Input_c$: Hash table $H_c$ of costs.
\end{itemize}

\subsubsection{Define output: }

\begin{itemize}

  \item $List_{out}$: A list where each element is a tuple (\textit{data constructor}, \textit{list(fields)})
                      where \textit{list(fields)} defines the correct ordering on the fields for each data layout
                      used by the function \textit{F}.

\end{itemize}

\subsubsection{Define costs: }

We define two possible types of costs for a particular access to occur in a function \textit{F} between the time frame two fields
 $f_1$ and $f_2$ are accessed by \textit{F}; 
 Let us say that function \textit{F} has consumed field $f_1$ and is now going 
 to access field $f_2$.
 Either the traversal \textit{F} has to perform a \textit{pointer dereference} to get to field $f_2$ 
 or the traversal must \textit{backtrack} inside the data layout to get to field $f_2$.  
 For a pointer dereference the data layout must provide the presence of such an indirection pointer after the end of field $f_1$
 such that the traversal can jump to the location $f_2$ is serialized at. 
 For a backtrack to occur, the traversal \textit{F} must be written in such a way that it can effectively traverse back to field $f_2$ in the 
 data layout.  

\begin{itemize}
  \item \textit{pointer dereference:} The data layout provides the presence of a pointer which can be dereferenced to 
                                      reach the location of the desired field we want to access. We store the cost of this 
                                      pointer dereference as some \textit{p}.

  \item \textit{backtracking: } The function \textit{F} must traverse back to reach the desired field. Either the function \textit{F}
                                is already written in such a way that it backtracks to the desired field or it must be re-written so 
                                that is can effectively backtrack in the given data layout is it processing. 
                                We store the cost of such a backtrack by function \textit{F} to reach a particular field as \textit{b}. 
\end{itemize}


\subsection{Graph definition}

To optimize a particular data constructor \textit{d} for a given traversal \textit{F}. 
We will construct a graph which consists of nodes and edges.

Each node in the graph represents a particular field $f_1$, $f_2$, $f_3$ \dots in the given data constructor \textit{d} we are optimizing. 
The graph also consists of edges connecting these nodes. These edges capture the \textit{access patterns} of the 
traversal \textit{F} amongst the fields of data constructor \textit{d}.

\begin{itemize}
\item \textit{Edge definition:} An edge e in the graph is a control flow \textit{CFG} edge with an associated probability \textit{p}.
                                This edge e follows the control/data flow of the traversal {F}.
                                The probability \textit{p} associated with the edge e comes from the likelihood of the traversal \textit{F}
                                accessing the particular fields $f_1$, $f_2$, $f_3$ \dots 
                                For now, we will statically assign these probabilities. These probabilities will be uniformly distributed. 
                                For an \textit{if \dots else} branch it is 50 \% for each branch. 
                                For a case clause with n branches it is (100/n) \% for each branch. 

\item \textit{Node definition:} The nodes n $\epsilon$ fields $f_1$, $f_2$, $f_3$ \dots in the given data constructor. 
                                Each field is a unique node in the graph.

\end{itemize}


\subsection{Benchmarks/Examples: }

\subsection{Tree copy}

\begin{figure}[H]
  \begin{lstlisting}[]

  type Left  = Tree
  type Right = Tree
  data Tree  = Leaf Int | Node Left Right

  copy :: Tree -> Tree 
  copy tree = 
    case tree of 
        Leaf val -> Leaf val 
        Node left right  -> Node (copy left) (copy right)
  
  \end{lstlisting}
  \caption{Copying a tree to a new location}
  \label{fig:tree-copy}
\end{figure}


\begin{figure}[H]
  \includegraphics[scale=1]{figures/treeCopy}
  \caption{Graph constructed from copy traversal~\ref{fig:tree-copy} for data constructor \textit{Node}}
  \label{graph:blog1}
\end{figure}


\subsection{Left most} 


\begin{figure}[H]
  \begin{lstlisting}[]
  
  type Left  = Tree
  type Right = Tree
  data Tree  = Leaf Int | Node Left Right

  leftmost :: Tree -> Int 
  leftmost tree = 
    case tree of 
        Leaf val -> val 
        Node left right -> leftmost left
  
  \end{lstlisting}
  \caption{Getting the leftmost value in the tree.}
  \label{fig:leftmost}
\end{figure}

\begin{figure}[H]
  \includegraphics[scale=1]{figures/leftmostGraph}
  \caption{Graph constructed from leftmost traversal~\ref{fig:leftmost} for data constructor \textit{Node}}
  \label{graph:blog1}
\end{figure}


\subsection{Right most}

\begin{figure}[H]
  \begin{lstlisting}[]

  type Left  = Tree
  type Right = Tree
  data Tree  = Leaf Int | Node Left Right

  rightmost :: Tree -> Int 
  rightmost tree = 
    case tree of 
        Leaf val -> val 
        Node left right -> rightmost right
  
  \end{lstlisting}
  \caption{Getting the rightmost value in the tree.}
  \label{fig:rightmost}
\end{figure}

\begin{figure}[H]
  \includegraphics[scale=1]{figures/rightmostGraph}
  \caption{Graph constructed from rightmost traversal~\ref{fig:rightmost} for data constructor \textit{Node}}
  \label{graph:blog1}
\end{figure}


\subsection{Blog traversals}

\subsubsection{emphasize a keyword in a blog: }

\begin{figure}[H]
\begin{lstlisting}[]

data BlogList = Blog Id Date Author Header Tags Content BlogList   
  
emphasizeKeyword :: String -> BlogList -> BlogList 
emphasizeKeyword keyword bloglist = 
        case bloglist of
              Blog _id date author header tags content rst -> 
                  let present = search tags keyword
                    in if (present) then 
                          let newcontent = emphasizeContent content keyword
                              newNext    = emphasizeKeyword keyword rst
                            in Blog _id date author header tags newcontent newNext
                       else 
                          let newNext = emphasizeKeyword keyword rst
                            in Blog _id date author header tags content newNext
              End -> End

\end{lstlisting}
\caption{Emphasizing a keyword over blog contents}
\label{fig:emph-keyword}
\end{figure}


\begin{figure}[H]
  \includegraphics[scale=0.65]{figures/CFG_emphKeyword}
  \caption{CFG constructed from blog traversal~\ref{fig:emph-keyword} for data constructor \textit{BlogList}}
  \label{CFG:blog1}
\end{figure}


\begin{figure}[H]
  \includegraphics[scale=1]{figures/blog1Graph}
  \caption{Field dependence Graph constructed from blog traversal~\ref{fig:emph-keyword} for data constructor \textit{BlogList} using CFG}
  \label{graph:blog1}
\end{figure}

For the traversal~\ref{fig:emph-keyword} we construct graph~\ref{graph:blog1} using the above terminology.

\subsection{SMT solver}

We use an SMT solver to find an optimal solution to the layout ordering problem.
The compiler will generate constrains for each edge in the layout graph that we generate using the field dependence graph of the program along with 
other necessary constraints.
We encode this problem as an ILP model, where each field is an \textit{Int} which can reside in the domain 0 to \textit{num fields - 1}.
Each edge in the layout graph has an associated cost C$_i$ unique to that edge. 
This cost can be either a backtrack, pointer dereference or a combination of both the costs. 
for each edge, the difference in the index's of the fields making up that edge decide this cost C$_i$ and we use the compiler to generate 4 constraints for each edge in the graph. 

The following python code shows the encoding for the graph~\ref{graph:blog1} generated by our compiler.

% \textbf{NOTE: This will be in haskell later, for now this is just for a proof of concept.}

% \begin{lstlisting}[language=Python]

% from z3 import * 

% #Constraints for tag search example

% #Fields that are being used, based on the graph
% tags, content, blogList = Ints('tags content blogList')

% #costs across each edge in the graph
% c1 , c2, c3 = Ints('c1 c2 c3')

% s = Optimize() 

% # Costs c1, c2 and c3 are costs to backtrack, pointer deference or more than one. 

% #####################################################################
% # Constraints for edge tags -> blogList
% # If fields are adjacent then no cost to traverse from tags to blogList
% s.add(Implies(tags - blogList == -1, c1 == 0))  

% # If there are more than 1 fields in between
% # then we pay a constant cost to go from tags 
% # to blogList by doing a pointer dereference.
% s.add(Implies(tags - blogList  < -1, c1 == 100)) 

% # If tags is after blogList, we do a pointer dereference
% # In addition, we need to backtrack to go back to blogList
% s.add(Implies(tags - blogList ==  1, c1 == 200)) 

% # If tags is after blogList and there are more than 1 fields
% # in between then we again do a pointer dereference.
% # In addition, we backtrack 
% # However, since there are more fields than 1 in between
% # this should be higher. For now, we assume same as prior case.
% s.add(Implies(tags - blogList   > 1, c1 == 200))
% #######################################################################


% #######################################################################
% # Constraints for edge tags -> content 
% # No cost
% s.add(Implies(tags - content == -1, c2 == 0))

% # Pointer dereference cost to jump to the content field
% s.add(Implies(tags - content  < -1, c2 == 100)) 

% # Pointer dereference cost to jump to tags then
% # backtrack to get to beginning of tags
% s.add(Implies(tags - content  == 1, c2 == 200)) 

% # Pointer dereference cost to jump to tags then 
% # backtrack to get to beginning of tags (This should be higher)
% s.add(Implies(tags - content   > 1, c2 == 200))   
% ########################################################################


% ########################################################################
% # Constraints for edge content -> blogList
% #No cost
% s.add(Implies(content - blogList == -1, c3 == 0))   

% # Pointer dereference cost to jump to blogList
% s.add(Implies(content - blogList  < -1, c3 == 100))

% # Pointer dereference cost to jump to content then 
% # backtrack to get to beginning of content
% s.add(Implies(content - blogList  == 1, c3 == 200)) 

% # Pointer dereference cost to jump to blogList
% # then backtrack to get to beginning of content 
% # (This should be higher but for now assume same as prior step)
% s.add(Implies(content - blogList   > 1, c3 == 200)) 
% ########################################################################


% #define the domain, the compiler should generate these constraints out
% #Since the number of fields in use are 3, we define domain from 0 to (3 - 1)

% # 0 <= 
% s.add(0 <= tags)
% s.add(0 <= content)
% s.add(0 <= blogList)

% # <= 2 
% s.add(tags <= 2)
% s.add(content <= 2)
% s.add(blogList <= 2)

% # Constraint that all indexes should be unique. 
% s.add(tags ~= content)
% s.add(tags ~= blogList)
% s.add(content ~= blogList)


% # Constraint all costs are greater than equal to 0 
% s.add(c1 >= 0)
% s.add(c2 >= 0)
% s.add(c3 >= 0)

% # Minimize the costs along all the edges
% # Multiply by likelihood percentage along that edge.
% s.minimize((c1*50) + (c2*50) + (c3*50))


% print(s.check())
% print(s.model())

% \end{lstlisting}


% This the the output generated. 
% This tells us that tags should occupy index 0, followed by content then the rest of the BlogList. 
% The cost of 100 is incurred along the edge Tags -> BlogList in graph~\ref{graph:blog1} in the optimal solution found by z3. 

% \begin{lstlisting}
%   sat
% [c3 = 0,
%  c2 = 0,
%  c1 = 100,
%  blogList = 2,
%  tags = 0,
%  content = 1]
% \end{lstlisting}


% ACM's consolidated article template, introduced in 2017, provides a
% consistent \LaTeX\ style for use across ACM publications, and
% incorporates accessibility and metadata-extraction functionality
% necessary for future Digital Library endeavors. Numerous ACM and
% SIG-specific \LaTeX\ templates have been examined, and their unique
% features incorporated into this single new template.

% If you are new to publishing with ACM, this document is a valuable
% guide to the process of preparing your work for publication. If you
% have published with ACM before, this document provides insight and
% instruction into more recent changes to the article template.

% The ``\verb|acmart|'' document class can be used to prepare articles
% for any ACM publication --- conference or journal, and for any stage
% of publication, from review to final ``camera-ready'' copy, to the
% author's own version, with {\itshape very} few changes to the source.

% \section{Template Overview}
% As noted in the introduction, the ``\verb|acmart|'' document class can
% be used to prepare many different kinds of documentation --- a
% double-blind initial submission of a full-length technical paper, a
% two-page SIGGRAPH Emerging Technologies abstract, a ``camera-ready''
% journal article, a SIGCHI Extended Abstract, and more --- all by
% selecting the appropriate {\itshape template style} and {\itshape
%   template parameters}.

% This document will explain the major features of the document
% class. For further information, the {\itshape \LaTeX\ User's Guide} is
% available from
% \url{https://www.acm.org/publications/proceedings-template}.

% \subsection{Template Styles}

% The primary parameter given to the ``\verb|acmart|'' document class is
% the {\itshape template style} which corresponds to the kind of publication
% or SIG publishing the work. This parameter is enclosed in square
% brackets and is a part of the {\verb|documentclass|} command:
% \begin{verbatim}
%   \documentclass[STYLE]{acmart}
% \end{verbatim}

% Journals use one of three template styles. All but three ACM journals
% use the {\verb|acmsmall|} template style:
% \begin{itemize}
% \item {\texttt{acmsmall}}: The default journal template style.
% \item {\texttt{acmlarge}}: Used by JOCCH and TAP.
% \item {\texttt{acmtog}}: Used by TOG.
% \end{itemize}

% The majority of conference proceedings documentation will use the {\verb|acmconf|} template style.
% \begin{itemize}
% \item {\texttt{acmconf}}: The default proceedings template style.
% \item{\texttt{sigchi}}: Used for SIGCHI conference articles.
% \item{\texttt{sigplan}}: Used for SIGPLAN conference articles.
% \end{itemize}

% \subsection{Template Parameters}

% In addition to specifying the {\itshape template style} to be used in
% formatting your work, there are a number of {\itshape template parameters}
% which modify some part of the applied template style. A complete list
% of these parameters can be found in the {\itshape \LaTeX\ User's Guide.}

% Frequently-used parameters, or combinations of parameters, include:
% \begin{itemize}
% \item {\texttt{anonymous,review}}: Suitable for a ``double-blind''
%   conference submission. Anonymizes the work and includes line
%   numbers. Use with the \texttt{\acmSubmissionID} command to print the
%   submission's unique ID on each page of the work.
% \item{\texttt{authorversion}}: Produces a version of the work suitable
%   for posting by the author.
% \item{\texttt{screen}}: Produces colored hyperlinks.
% \end{itemize}

% This document uses the following string as the first command in the
% source file:
% \begin{verbatim}
% \documentclass[acmsmall]{acmart}
% \end{verbatim}

% \section{Modifications}

% Modifying the template --- including but not limited to: adjusting
% margins, typeface sizes, line spacing, paragraph and list definitions,
% and the use of the \verb|\vspace| command to manually adjust the
% vertical spacing between elements of your work --- is not allowed.

% {\bfseries Your document will be returned to you for revision if
%   modifications are discovered.}

% \section{Typefaces}

% The ``\verb|acmart|'' document class requires the use of the
% ``Libertine'' typeface family. Your \TeX\ installation should include
% this set of packages. Please do not substitute other typefaces. The
% ``\verb|lmodern|'' and ``\verb|ltimes|'' packages should not be used,
% as they will override the built-in typeface families.

% \section{Title Information}

% The title of your work should use capital letters appropriately -
% \url{https://capitalizemytitle.com/} has useful rules for
% capitalization. Use the {\verb|title|} command to define the title of
% your work. If your work has a subtitle, define it with the
% {\verb|subtitle|} command.  Do not insert line breaks in your title.

% If your title is lengthy, you must define a short version to be used
% in the page headers, to prevent overlapping text. The \verb|title|
% command has a ``short title'' parameter:
% \begin{verbatim}
%   \title[short title]{full title}
% \end{verbatim}

% \section{Authors and Affiliations}

% Each author must be defined separately for accurate metadata
% identification.  As an exception, multiple authors may share one
% affiliation. Authors' names should not be abbreviated; use full first
% names wherever possible. Include authors' e-mail addresses whenever
% possible.

% Grouping authors' names or e-mail addresses, or providing an ``e-mail
% alias,'' as shown below, is not acceptable:
% \begin{verbatim}
%   \author{Brooke Aster, David Mehldau}
%   \email{dave,judy,steve@university.edu}
%   \email{firstname.lastname@phillips.org}
% \end{verbatim}

% The \verb|authornote| and \verb|authornotemark| commands allow a note
% to apply to multiple authors --- for example, if the first two authors
% of an article contributed equally to the work.

% If your author list is lengthy, you must define a shortened version of
% the list of authors to be used in the page headers, to prevent
% overlapping text. The following command should be placed just after
% the last \verb|\author{}| definition:
% \begin{verbatim}
%   \renewcommand{\shortauthors}{McCartney, et al.}
% \end{verbatim}
% Omitting this command will force the use of a concatenated list of all
% of the authors' names, which may result in overlapping text in the
% page headers.

% The article template's documentation, available at
% \url{https://www.acm.org/publications/proceedings-template}, has a
% complete explanation of these commands and tips for their effective
% use.

% Note that authors' addresses are mandatory for journal articles.

% \section{Rights Information}

% Authors of any work published by ACM will need to complete a rights
% form. Depending on the kind of work, and the rights management choice
% made by the author, this may be copyright transfer, permission,
% license, or an OA (open access) agreement.

% Regardless of the rights management choice, the author will receive a
% copy of the completed rights form once it has been submitted. This
% form contains \LaTeX\ commands that must be copied into the source
% document. When the document source is compiled, these commands and
% their parameters add formatted text to several areas of the final
% document:
% \begin{itemize}
% \item the ``ACM Reference Format'' text on the first page.
% \item the ``rights management'' text on the first page.
% \item the conference information in the page header(s).
% \end{itemize}

% Rights information is unique to the work; if you are preparing several
% works for an event, make sure to use the correct set of commands with
% each of the works.

% The ACM Reference Format text is required for all articles over one
% page in length, and is optional for one-page articles (abstracts).

% \section{CCS Concepts and User-Defined Keywords}

% Two elements of the ``acmart'' document class provide powerful
% taxonomic tools for you to help readers find your work in an online
% search.

% The ACM Computing Classification System ---
% \url{https://www.acm.org/publications/class-2012} --- is a set of
% classifiers and concepts that describe the computing
% discipline. Authors can select entries from this classification
% system, via \url{https://dl.acm.org/ccs/ccs.cfm}, and generate the
% commands to be included in the \LaTeX\ source.

% User-defined keywords are a comma-separated list of words and phrases
% of the authors' choosing, providing a more flexible way of describing
% the research being presented.

% CCS concepts and user-defined keywords are required for for all
% articles over two pages in length, and are optional for one- and
% two-page articles (or abstracts).

% \section{Sectioning Commands}

% Your work should use standard \LaTeX\ sectioning commands:
% \verb|section|, \verb|subsection|, \verb|subsubsection|, and
% \verb|paragraph|. They should be numbered; do not remove the numbering
% from the commands.

% Simulating a sectioning command by setting the first word or words of
% a paragraph in boldface or italicized text is {\bfseries not allowed.}

% \section{Tables}

% The ``\verb|acmart|'' document class includes the ``\verb|booktabs|''
% package --- \url{https://ctan.org/pkg/booktabs} --- for preparing
% high-quality tables.

% Table captions are placed {\itshape above} the table.

% Because tables cannot be split across pages, the best placement for
% them is typically the top of the page nearest their initial cite.  To
% ensure this proper ``floating'' placement of tables, use the
% environment \textbf{table} to enclose the table's contents and the
% table caption.  The contents of the table itself must go in the
% \textbf{tabular} environment, to be aligned properly in rows and
% columns, with the desired horizontal and vertical rules.  Again,
% detailed instructions on \textbf{tabular} material are found in the
% \textit{\LaTeX\ User's Guide}.

% Immediately following this sentence is the point at which
% Table~\ref{tab:freq} is included in the input file; compare the
% placement of the table here with the table in the printed output of
% this document.

% \begin{table}
%   \caption{Frequency of Special Characters}
%   \label{tab:freq}
%   \begin{tabular}{ccl}
%     \toprule
%     Non-English or Math&Frequency&Comments\\
%     \midrule
%     \O & 1 in 1,000& For Swedish names\\
%     $\pi$ & 1 in 5& Common in math\\
%     \$ & 4 in 5 & Used in business\\
%     $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
%   \bottomrule
% \end{tabular}
% \end{table}

% To set a wider table, which takes up the whole width of the page's
% live area, use the environment \textbf{table*} to enclose the table's
% contents and the table caption.  As with a single-column table, this
% wide table will ``float'' to a location deemed more
% desirable. Immediately following this sentence is the point at which
% Table~\ref{tab:commands} is included in the input file; again, it is
% instructive to compare the placement of the table here with the table
% in the printed output of this document.

% \begin{table*}
%   \caption{Some Typical Commands}
%   \label{tab:commands}
%   \begin{tabular}{ccl}
%     \toprule
%     Command &A Number & Comments\\
%     \midrule
%     \texttt{{\char'134}author} & 100& Author \\
%     \texttt{{\char'134}table}& 300 & For tables\\
%     \texttt{{\char'134}table*}& 400& For wider tables\\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% Always use midrule to separate table header rows from data rows, and
% use it only for this purpose. This enables assistive technologies to
% recognise table headers and support their users in navigating tables
% more easily.

% \section{Math Equations}
% You may want to display math equations in three distinct styles:
% inline, numbered or non-numbered display.  Each of the three are
% discussed in the next sections.

% \subsection{Inline (In-text) Equations}
% A formula that appears in the running text is called an inline or
% in-text formula.  It is produced by the \textbf{math} environment,
% which can be invoked with the usual
% \texttt{{\char'134}begin\,\ldots{\char'134}end} construction or with
% the short form \texttt{\$\,\ldots\$}. You can use any of the symbols
% and structures, from $\alpha$ to $\omega$, available in
% \LaTeX~\cite{Lamport:LaTeX}; this section will simply show a few
% examples of in-text equations in context. Notice how this equation:
% \begin{math}
%   \lim_{n\rightarrow \infty}x=0
% \end{math},
% set here in in-line math style, looks slightly different when
% set in display style.  (See next section).

% \subsection{Display Equations}
% A numbered display equation---one set off by vertical space from the
% text and centered horizontally---is produced by the \textbf{equation}
% environment. An unnumbered display equation is produced by the
% \textbf{displaymath} environment.

% Again, in either environment, you can use any of the symbols and
% structures available in \LaTeX\@; this section will just give a couple
% of examples of display equations in context.  First, consider the
% equation, shown as an inline equation above:
% \begin{equation}
%   \lim_{n\rightarrow \infty}x=0
% \end{equation}
% Notice how it is formatted somewhat differently in
% the \textbf{displaymath}
% environment.  Now, we'll enter an unnumbered equation:
% \begin{displaymath}
%   \sum_{i=0}^{\infty} x + 1
% \end{displaymath}
% and follow it with another numbered equation:
% \begin{equation}
%   \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
% \end{equation}
% just to demonstrate \LaTeX's able handling of numbering.

% \section{Figures}

% The ``\verb|figure|'' environment should be used for figures. One or
% more images can be placed within a figure. If your figure contains
% third-party material, you must clearly identify it as such, as shown
% in the example below.
% \begin{figure}[h]
%   \centering
%   % \includegraphics[width=\linewidth]{sample-franklin}
%   \caption{1907 Franklin Model D roadster. Photograph by Harris \&
%     Ewing, Inc. [Public domain], via Wikimedia
%     Commons. (\url{https://goo.gl/VLCRBB}).}
%   \Description{A woman and a girl in white dresses sit in an open car.}
% \end{figure}

% Your figures should contain a caption which describes the figure to
% the reader.

% Figure captions are placed {\itshape below} the figure.

% Every figure should also have a figure description unless it is purely
% decorative. These descriptions convey what’s in the image to someone
% who cannot see it. They are also used by search engine crawlers for
% indexing images, and when images cannot be loaded.

% A figure description must be unformatted plain text less than 2000
% characters long (including spaces).  {\bfseries Figure descriptions
%   should not repeat the figure caption – their purpose is to capture
%   important information that is not already provided in the caption or
%   the main text of the paper.} For figures that convey important and
% complex new information, a short text description may not be
% adequate. More complex alternative descriptions can be placed in an
% appendix and referenced in a short figure description. For example,
% provide a data table capturing the information in a bar chart, or a
% structured list representing a graph.  For additional information
% regarding how best to write figure descriptions and why doing this is
% so important, please see
% \url{https://www.acm.org/publications/taps/describing-figures/}.

% \subsection{The ``Teaser Figure''}

% A ``teaser figure'' is an image, or set of images in one figure, that
% are placed after all author and affiliation information, and before
% the body of the article, spanning the page. If you wish to have such a
% figure in your article, place the command immediately before the
% \verb|\maketitle| command:
% \begin{verbatim}
%   \begin{teaserfigure}
%     \includegraphics[width=\textwidth]{sampleteaser}
%     \caption{figure caption}
%     \Description{figure description}
%   \end{teaserfigure}
% \end{verbatim}

% \section{Citations and Bibliographies}

% The use of \BibTeX\ for the preparation and formatting of one's
% references is strongly recommended. Authors' names should be complete
% --- use full first names (``Donald E. Knuth'') not initials
% (``D. E. Knuth'') --- and the salient identifying features of a
% reference should be included: title, year, volume, number, pages,
% article DOI, etc.

% The bibliography is included in your source document with these two
% commands, placed just before the \verb|\end{document}| command:
% \begin{verbatim}
%   \bibliographystyle{ACM-Reference-Format}
%   \bibliography{bibfile}
% \end{verbatim}
% where ``\verb|bibfile|'' is the name, without the ``\verb|.bib|''
% suffix, of the \BibTeX\ file.

% Citations and references are numbered by default. A small number of
% ACM publications have citations and references formatted in the
% ``author year'' style; for these exceptions, please include this
% command in the {\bfseries preamble} (before the command
% ``\verb|\begin{document}|'') of your \LaTeX\ source:
% \begin{verbatim}
%   \citestyle{acmauthoryear}
% \end{verbatim}

% \section{Acknowledgments}

% Identification of funding sources and other support, and thanks to
% individuals and groups that assisted in the research and the
% preparation of the work should be included in an acknowledgment
% section, which is placed just before the reference section in your
% document.

% This section has a special environment:
% \begin{verbatim}
%   \begin{acks}
%   ...
%   \end{acks}
% \end{verbatim}
% so that the information contained therein can be more easily collected
% during the article metadata extraction phase, and to ensure
% consistency in the spelling of the section heading.

% Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

% \section{Appendices}

% If your work needs an appendix, add it before the
% ``\verb|\end{document}|'' command at the conclusion of your source
% document.

% Start the appendix with the ``\verb|appendix|'' command:
% \begin{verbatim}
%   \appendix
% \end{verbatim}
% and note that in the appendix, sections are lettered, not
% numbered. This document has two appendices, demonstrating the section
% and subsection identification method.

% \section{Multi-language papers}

% Papers may be written in languages other than English or include
% titles, subtitles, keywords and abstracts in different languages (as a
% rule, a paper in a language other than English should include an
% English title and an English abstract).  Use \verb|language=...| for
% every language used in the paper.  The last language indicated is the
% main language of the paper.  For example, a French paper with
% additional titles and abstracts in English and German may start with
% the following command
% \begin{verbatim}
% \documentclass[sigconf, language=english, language=german,
%                language=french]{acmart}
% \end{verbatim}

% The title, subtitle, keywords and abstract will be typeset in the main
% language of the paper.  The commands \verb|\translatedXXX|, \verb|XXX|
% begin title, subtitle and keywords, can be used to set these elements
% in the other languages.  The environment \verb|translatedabstract| is
% used to set the translation of the abstract.  These commands and
% environment have a mandatory first argument: the language of the
% second argument.  See \verb|sample-sigconf-i13n.tex| file for examples
% of their usage.

% \section{SIGCHI Extended Abstracts}

% The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
% not in Word) produces a landscape-orientation formatted article, with
% a wide left margin. Three environments are available for use with the
% ``\verb|sigchi-a|'' template style, and produce formatted output in
% the margin:
% \begin{description}
% \item[\texttt{sidebar}:]  Place formatted text in the margin.
% \item[\texttt{marginfigure}:] Place a figure in the margin.
% \item[\texttt{margintable}:] Place a table in the margin.
% \end{description}

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.



% \begin{acks}
% Acknowledgments...
% \end{acks}

%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
%\bibliographystyle{ACM-Reference-Format}
% \bibliography{sample-base}


%%
%% If your work has an appendix, this is the place to put it.
%\appendix

% \section{Research Methods}

% \subsection{Part One}

% Lorem ipsum dolor sit amet, consectetur adipiscing elit. Morbi
% malesuada, quam in pulvinar varius, metus nunc fermentum urna, id
% sollicitudin purus odio sit amet enim. Aliquam ullamcorper eu ipsum
% vel mollis. Curabitur quis dictum nisl. Phasellus vel semper risus, et
% lacinia dolor. Integer ultricies commodo sem nec semper.

% \subsection{Part Two}

% Etiam commodo feugiat nisl pulvinar pellentesque. Etiam auctor sodales
% ligula, non varius nibh pulvinar semper. Suspendisse nec lectus non
% ipsum convallis congue hendrerit vitae sapien. Donec at laoreet
% eros. Vivamus non purus placerat, scelerisque diam eu, cursus
% ante. Etiam aliquam tortor auctor efficitur mattis.

% \section{Online Resources}

% Nam id fermentum dui. Suspendisse sagittis tortor a nulla mollis, in
% pulvinar ex pretium. Sed interdum orci quis metus euismod, et sagittis
% enim maximus. Vestibulum gravida massa ut felis suscipit
% congue. Quisque mattis elit a risus ultrices commodo venenatis eget
% dui. Etiam sagittis eleifend elementum.

% Nam interdum magna at lectus dignissim, ac dignissim lorem
% rhoncus. Maecenas eu arcu ac neque placerat aliquam. Nunc pulvinar
% massa et mattis lacinia.

%\bibliography{refs}

%\end{document}
%\endinput
%%
%% End of file `sample-acmsmall-conf.tex'.


==> overview.tex <==
\section[Dense Representation]{Dense Representation: The Good, The Bad, and The Pointers}%
\label{sec:overview}
\label{ssec:overview:dense}
%\rn{Lovely section title!}

This section gives a refresher on dense representations of algebraic datatypes (\Secref{sec:overview:overview})
and, using an example, illustrates the performance challenges of picking a
layout for a datatype's dense representation (\Secref{sec:overview:example}).

\subsection{Overview}%
\label{sec:overview:overview}

\emph{Algebraic datatypes} (ADTs) are a powerful language-based technology. ADTs can
express many complex data structures while, nevertheless, providing a
pleasantly high level of abstraction for application programmers.
% ADTs are directly supported in many functional languages, such as Haskell and
% dialects of ML, and can be modeled in object-oriented languages via restricted
% forms of classes (sealed classes in Java, case classes in Scala, etc.).
The high-level specification of ADTs leaves
space to experiment with low-level implementation strategies. Hence, we use ADTs
and a purely functional setting for our exploration of performance implications of
data layout.

%\paragraph{Mostly dense data representation in \gibbon{}.}
%
In a conventional implementation of algebraic datatypes, accessing a value of a
given ADT requires dereferencing a pointer to a heap object, then reading the
header word, to get to the payload.
% Getting to the
% payload may require one more pointer dereference.
Accessing the desired data may require multiple further pointer dereferences, as objects
may contain pointers to other objects, requiring the unraveling of multiple layers of nesting.
% \Red{It may require more than one pointer dereference because of the nested degree of \textit{indirections},
% that is, a pointer could store the location of another pointer which then carries the actual data?}
% \vs{TODO: Audit this part}
%
The whole process is often described as \emph{pointer chasing}, a fitting name, 
especially when the work per payload element is low.

In a dense representation of ADTs, as implemented in \gibbon{},
the data constructor stores
one byte for the constructor's {\em tag}, followed immediately by its fields,
in the hope of avoiding pointer chasing.
%
Wherever possible, the tag value occurs inline in a bytestream that
hosts multiple values.
%
As a result, values tend to reside compactly in the heap using contiguous blocks of
memory. This representation avoids or reduces pointer chasing and admits
efficient linear traversals favored by modern hardware via
prefetching and caching.
%% %
%% In contrast, such efficiency is either impossible or extremely
%% challenging for the approaches taken by most other functional
%% languages, where there is a more conventional treatment of algebraic
%% datatypes.
%% %
%% Such approaches resort to fully or mostly boxed representations of
%% values, and often the tradeoffs are made in the compiler in ways that
%% are hard for novice or even expert application programmers to
%% anticipate.

%\paragraph{Where dense representation falls short.}

\subsection{Running Example}%
\label{sec:overview:example}

The efficiency of traversals on dense representations of data structures
largely depends on how well access patterns and layout match each other.
%
Consider a datatype (already monomorphized) describing
a sequence of posts in a blog\footnote{Throughout the paper we use a subset of Haskell syntax, which
corresponds to the input language of the \gibbon compiler.}:
\begin{lstlisting}
    data BlogList = Nil | Blog Content HashTags BlogList
\end{lstlisting}
%
A non-empty blog value stores a content field (a
string representing the body of the blog post), a list of hash tags
summarizing keywords of the blog post, and a pointer to the rest of
the list.%
%
\footnote{%
  In practice, you may want to reuse a standard list type, e.g.:
  \input{figures/blog-polymorphic.tex} but a typical compiler (including
  \gibbon) would specialize the parametric list type with the \lstinline|Blog|
  type to arrive at an equivalent of the definition shown in the main text
  above.%
}. The datatype has one point of recursion and several variable-length fields in
the definition. To extend on this, \Secref{subsec:eval:trees:rightmost} contains
an example of tree-shaped data (two points of recursion, in particular) with a
fixed-length field. The most general case of multiple points of recursion and
variable-length fields is also handled by \system.

The most favorable traversal for the \lstinline|Blog| datatype
is the same as the order in
which the fields appear in the datatype definition. In this case, \gibbon{} can
assign the dense and pointer-free layout as shown in Figure~\ref{fig:traversal-ideal}.
Solid blue arrows connecting adjacent fields represent unconditional sequential
accesses---i.e., reading a range of bytes in a buffer, and then reading the next
consecutive range.
Such a traversal will reap the benefits of locality.

\begin{figure}[t]
  \begin{lstlisting}[]
  emphKeyword :: String -> BlogList -> BlogList
  emphKeyword keyword blogs = case blogs of
      Nil -> Nil
      Blog content hashTags blogs' ->
          case search keyword hashTags of
            True -> let content' = emphContent content keyword
                        blogs''  = emphKeyword keyword blogs'
                      in Blog content' hashTags blogs''
            False -> let blogs'' = emphKeyword keyword blogs'
                       in Blog content hashTags blogs''
   \end{lstlisting}
  \caption{Blog traversal motivating example}
  \label{fig:blog-traversal}
\end{figure}

%\begin{center} 

%\end{center}

%
% Artem: vv--this blows out the suspense!
%There is no work to compute the \emph{start} of a downstream field,
%because its starting address is at the end of the preceding field!

%\paragraph{Skipping over fields of a datatype.}
%
On the other hand, consider a traversal with less efficient access patterns (\figref{fig:blog-traversal}).
%
The algorithm scans blog entries for a given keyword in \lstinline|HashTags|.
%
If the hash tags of a particular blog entry contain the keyword, the
algorithm puts an emphasis on every occurrence of the keyword in the content
field.
%
In terms of access patterns, if we found a match in the hash tags field,
subsequent accesses to the fields happen in order, as depicted in Figure~\ref{fig:traversal-blog-time-complexity-left}.
%
Otherwise, the traversal skips over the content field, as depicted in Figure~\ref{fig:traversal-blog-time-complexity-right}.
%
% \begin{center}
%   \includegraphics[width=0.4\linewidth]{figures/traveral_blog_then_gibbon_time_complexity.pdf} \, \,
%     \includegraphics[width=0.4\linewidth]{figures/traveral_blog_else_gibbon_time_complexity.pdf}
% \ap{I think they should be a proper Figure}
% \end{center}

%\begin{center}

%\end{center}


%
Here we use red lines to represent accesses that must \emph{skip over} some data
between the current position in the buffer and the target data. \new{Data may be constructed recursively
and will not necessarily have a statically-known size, so finding the end of a piece of unneeded data requires
scanning through that data in order to reach the target data.}
%
This \new{extra traversal (parsing data just to find the end of it)} requires an arbitrarily large amount of work because
the \lstinline|content| field has a variable, dynamically-allocated size. 
%There is
%no way of knowing where it ends without storing a pointer to the start of \lstinline|HashTags|.

% \begin{figure}[t]
%     \begin{minipage}[c]{\linewidth}
%     \centering
%     \subfloat[][True case]{
%       \centering
%     \includegraphics[width=0.4\textwidth]{figures/traveral_blog_then_gibbon_time_complexity.pdf}\label{fig:traversal-blog-time-complexity-left}}
%     \subfloat[][False case]{
%       \centering
%     \includegraphics[width=0.4\textwidth]{figures/traveral_blog_else_gibbon_time_complexity.pdf}\label{fig:traversal-blog-time-complexity-right}}
%     \label{fig:traversal-blog-time-complexity}
%     \caption{\ap{alignment of pictures and captions looks off}\new{Out of order accesses (red), incurring costly extra traversals over fields in the middle.}}
%   \end{minipage}\hfill
% \end{figure}

%\paragraph{Shortcut pointers.}
%
\new{Extra traversals that perform useful no work}, like skipping over the \lstinline|content| field above,
can degrade the asymptotic efficiency of programs.
%
One way to avoid such traversals is to use pointers.
%
For instance, when \gibbon detects that it has to skip over intervening data, it
changes the definition of the constructor by inserting \emph{shortcut pointers},
which provide an exact memory address to skip to in constant time.
% (similar in spirit to pointer swizzling). % Artem: <- what's that??
%
For our example program, \gibbon{} introduces one shortcut
pointer for the \lstinline|HashTags| field, and another one for the tail of the list.
%

  % \begin{figure}[t]
  %   \begin{minipage}[c]{\linewidth}
  %   \centering
  %   \subfloat[][True case]{
  %   \includegraphics[width=0.4\textwidth]{figures/traveral_blog_then_gibbon_pointers.pdf}\label{fig:traversal-blog-pointers-left}}
  %   \subfloat[][False case]{
  %   \includegraphics[width=0.4\textwidth]{figures/traveral_blog_else_gibbon_pointers.pdf}\label{fig:traversal-blog-pointers-right}}
  %   \caption{Representation with pointers to allow random access.}
  %   \label{fig:traversal-blog-pointers}
  % \end{minipage}\hfill
  % \end{figure}

The pointers provide direct accesses to the respective fields when needed and
restore the constant-time asymptotic complexity for certain operations.
\new{This results in the access patterns shown in Figure~\ref{fig:traversal-blog-pointers-left} and~\ref{fig:traversal-blog-pointers-right}.}
Red dashed lines represent pointer-based constant-time field accesses.
%
Otherwise, the access patterns are similar to what we had before.

The pointer-based approach in our example has two weaknesses. First, this
approach is susceptible to the usual problems with pointer chasing. Second, just
like with the initial solution, we access fields in an order that does not match
the layout: the hash tags field is always accessed first but lives next to the
content field. 
%In the next subsection we give an overview of our analysis, which
%helps to improve this example and results in the access patterns shown in Figure~\ref{fig:traversal-blog-optimized}.

\system, described in the following section, automates finding
the weaknesses of the pointer-based approach and improving data layout and code accordingly.
For instance, performance in our example can be improved by swapping the
ordering between the \lstinline|Content| and \lstinline|HashTags| fields.
%
Given this reordering, the hash tags are available directly at the start of the
value, which lines up with the algorithm better, as the algorithm always
accesses this field first.
%
Additionally, our program's \lstinline|True| case (the keyword gets a hit within the
hash tags) is more efficient because after traversing the content to highlight
the keyword it stops at the next blog entry ready for the algorithm to make
the recursive call.
%
This improved data layout results in the more-streamlined access patterns shown in Figures~\ref{fig:traversal-blog-optimized-left} and~\ref{fig:traversal-blog-optimized-right}.
%
%\begin{center}
%  \includegraphics[width=0.4\linewidth]{figures/traveral_blog_then_gibbon_optimized.pdf} \, \,
%  \includegraphics[width=0.4\linewidth]{figures/traveral_blog_else_gibbon_optimized.pdf}
%\end{center}
%\vspace{-2.8em}
%\begin{center}

%\caption{Optimized layout with favorable access patterns.}
%  \label{fig:traversal-blog-pointers}

\begin{figure}[t]
  \centering
  \captionsetup[subfigure]{justification=centering}
\begin{subfigure}{0.43\textwidth}
\includegraphics[width=\textwidth]{figures/Ideal_serial_layout_linear_access.pdf}
\caption{{Ideal access patterns}}
\label{fig:traversal-ideal}
\end{subfigure}
\\
\begin{subfigure}{0.43\textwidth}
\includegraphics[width=\textwidth]{figures/traveral_blog_then_gibbon_time_complexity.pdf}
\caption{{True case extra traversals}}
\label{fig:traversal-blog-time-complexity-left}
\end{subfigure}
\begin{subfigure}{0.43\textwidth}
\includegraphics[width=\textwidth]{figures/traveral_blog_else_gibbon_time_complexity.pdf}
\caption{{False case extra traversals}}
\label{fig:traversal-blog-time-complexity-right}
\end{subfigure}
\caption{Showing a dense pointer-free layout with ideal accesses on top. Numbers represent the access order. 
          Out of order accesses (red), incur costly extra traversals over fields in the middle.}
\end{figure}


\begin{figure}[t]
  \captionsetup[subfigure]{justification=centering}
  \begin{minipage}[]{\linewidth}
  \centering
  \subfloat[][{True case unoptimized}]{
  \includegraphics[width=0.50\textwidth]{figures/traveral_blog_then_gibbon_pointers.pdf}\label{fig:traversal-blog-pointers-left}}
  \subfloat[][{True case optimized}]{
  \includegraphics[width=0.50\textwidth]{figures/traveral_blog_then_gibbon_optimized.pdf}\label{fig:traversal-blog-optimized-left}}
  \\
  \subfloat[][{False case unoptimized}]{
  \includegraphics[width=0.50\textwidth]{figures/traveral_blog_else_gibbon_pointers.pdf}\label{fig:traversal-blog-pointers-right}}
  \subfloat[][{False case optimized}]{
  \includegraphics[width=0.50\textwidth]{figures/traveral_blog_else_gibbon_optimized.pdf}\label{fig:traversal-blog-optimized-right}}
  \caption{Showing the unoptimized representation with pointers to allow random access and the optimized layout with favorable access patterns.}
\end{minipage}\hfill
\end{figure}
%\end{center}



% %
% This improved layout is produced automatically by \system{}.

% Yet, there remains plenty of room for improvement: if we optimize the
% data layout for this specific program, we can (1) further compact our
% blog items by doing with just one shortcut pointer and (2) achieve
% a better, more linear traversal in the ``then'' branch.
% %
% To get these improvements, we design an approach that combines
% type-level and control-flow information and restructures the program
% accordingly.

% Artem: the next subsection largely repeats contributions from Intro and doesn't
% provide new insights in how the system works. In the interest of space as well
% as presentation I mute it for the time being. I think what it was supposed to
% do (show how the system works using the BlogList example) is achieved in
% section 3.
% \subsection{Picking A Better Layout With \system}
% \label{ssec:overview:marmoset}

% % Artem: vv--this all has been said and will be repeated again many times.
% %                Let's just focus on an example...
% % Our approach is to increase compactness and linear access by taking
% % into account temporal access patterns in the program.
% % %
% % Given the results of a program analysis, we reorder the fields in type
% % constructors (and adjust the code accordingly).
% %
% % Artem: [future work]
% %        let's not reiterate the point that we did not implement (below).
% % We note that, although our depictions above show two shortcut
% % pointers, our \system{} actually enables a significant compaction,
% % thanks its reordering of the fields.
% %
% % With reordering, we can remove the first shortcut pointer, that is,
% % the one pointing to the content field, because each of the two
% % conditional branches in our program already fully traverse the
% % hash-tags field, and thus already pay for finding the starting address
% % of the content field.
% %
% % However, to realize this single-pointer version, there some
% % improvements to the rest of the \gibbon{} compiler that are needed,
% % and we leave such efforts to future work.

% \paragraph{Customizable layouts.}
% %
% In \system{}, we treat data ordering as a free variable, adapting
% it to the code that uses the data.
% %
% % Artem: [future work]
% % We also provide annotations, which the user can add in comments to
% % partially or fully constrain the search space of orderings
% % (narrowing).
% %
% There are also examples where widening the search space to include
% transformations of the \emph{program order} as well would yield even
% better solutions, which could complement our approach, Infact, we use
% \textit{code-motion} of let bindings as another free variable in our
% optimization and talk about when we use it to further optimize the
% running example in~\ref{sec:attributes}. If data-flow dependencies allow
% code-motion of let bindings, we place fields in such a way that mimics
% a \textit{structure of arrays} type transformation.
% Consider for example a list datatype:
% \begin{lstlisting}
% data List =  Nil | Cons Int List
% \end{lstlisting}
% Here, \lstinline|List| on the right-hand side of the equals sign is a recursive
% field representing the tail of a linked list. We show that having the element field
% (\lstinline|Int| in the example) after the tail of the list may offer similar benefits to a
% \textit{structure-of-arrays} representation if datatypes are packed by the
% compiler. This is a cherry on top of optimizing for the access patterns as discussed before.
% % Artem: the next sentence goes into too much details.
% % Since, the Integer fields are all next to each other in memory, albeit, in the reverse order.

% \paragraph{From access patterns in the program to the field-access graph, a cost model of field orderings.}
% %
% The key to our approach is a cost model that assigns costs to
% different field orderings and a compiler pass that infers costs for
% given programs and assigns fields accordingly.
% %
% Our cost model involves the inference for each data-type constructor
% in the program of a \emph{field-access graph}.
% %
% This graph represents the temporal ordering of accesses among fields
% and the associated costs, based on the control-flow and data -flow graph
% of the program.
% %
% Regarding the \lstinline|Blog| constructor, for example, our analysis produces a
% field-access graph with three vertices representing the three fields, where each
% edge means that one field is accessed immediately before the other.
% %
% The edges are induced by the two branches in our example function: in
% the ``then'' branch, we have an edge going from the hash-tags to the
% content field, and one from the content to the tail-pointer field; in
% the ``else'' branch there is an edge from the hash-tags to the
% list-tail field. Edges are differented by whether they arise from a data flow
% dependency or purely an outcome of the control flow of the program.
% Section~\ref{design:fieldgraph} talks about this distinction further.

% \paragraph{From field-access graph to optimized ordering, via ILP solver.}
% %
% From this graph, we obtain a cost model for different orderings by
% weighting each edge.
% %
% Such weights are determined in our approach by approximate properties
% of the program's control flow, e.g., the likelihood of a given access
% based on the branching structure leading to the access.
% %
% Our approach takes a simple but effective approximation based on
% static control flow and data flow, but more sophisticated approximations are
% possible.
% %
% Given a cost graph, \system{} then encodes it as an optimization problem that
% can be solved by an off-the-shelf ILP (integer linear programming) solver.
% %
% This optimization problem is tractable because its size is in
% proportion to the size of the data-type definition, not that of the
% whole program.
% %
% From the resulting ILP solution, we can decode the result and obtain
% an efficient reordering of the fields.
% %
% In general, our \system{}
% analyses one pair of function definition and data-type constructor at a time,
% and rewrites the program to reflect the reordering of its fields.


==> relatedwork.tex <==
\section{Related Work}

\subsection{Cache-conscious data}

%\paragraph{Using generational garbage collection to implement cache-conscious data placement in object-oriented languages~\cite{ccgarbage}}
%
Chilimbi and Larus~\cite{ccgarbage} base on an object-oriented language with a
generational garbage collector, which they extend with a heuristic for
copying objects to the TO space.
%
Their heuristic uses a special-purpose graph data structure, the \emph{object affinity
graph}, to identify when groups of objects are accessed by the program
close together in time.
%
When a given group of objects have high affinity in the object
affinity graph, the collector is more likely to place them close
together in the TO space.
%
As such, a goal of their work and ours is to achieve higher data-access locality
by carefully grouping together objects in the heap.
%
However, a key difference from our work is that their approach bases its placement decisions
on an object-affinity graph that is generated from profiling data, which is
typically collected online by some compiler-inserted instrumentation.
%
The placement decisions made by our approach are based on data collected by static analysis of the program.
%
Such an approach has the advantage of not depending on the output of dynamic profiling, and therefore
avoids the implementation challenges of dynamic profiling.
%
A disadvantage of not using dynamic profiling is that the approach
cannot adapt to changing access patterns that are highly input
specific.
%
We leave open for future work the possibility of getting the best of both approaches.

%% There are two properties of object oriented programming that are utilized. Objects are less than 32 KB and that they are not lightweight use objects. Since the cache block sizes these days are 64 KB this means that the fields of the objects need not be optimized for and the only layout optimization should be object level optimization.
%% The paper introduces a concepts of a object affinity graph which is a graph consisting of vertices as live objects
%% % in the garbage collector
%% and edges encode the temporal affinity between the objects. This graph is generated by hooking the application with a real time profiler that tracks these temporal affinities. During a scavenge phase the copying garbage collector then copies these objects over to the ``TO'' space in an order that increases the cache performance. They use a greedy algorithm that traverses the max weighted edge and copyies the objects over in this greedy fashion. Miss rates are improved by 20\% to 41\% and performace by 18\% to 31\% compared to prior work.


%\paragraph{Cache-Conscious Structure Definition~\cite{CSD}}
%
%The work extends the work Cache-Conscious structure layout by focusing on data structures that are larger than the size of a cache block. Previous work worked best for data structures that are around half the size of a cache block. This work builds upon the prior work by extending it with two more techniques. These are \textbf{structure splitting} and \textbf{field reordering}.
%
%Mapping concurrently accessed elements of a struct in the same cache block provides an implicit prefetch. If these elements do not fit in the same cache block then placing them in non-conflicting cache blocks will reduce cache misses.
%
Chilimbi et al.~\cite{CSD} introduce the idea of hot/cold splitting of a data structure, where elements are categorized as being ``hot'' if accessed frequently and ``cold'' if accessed inferquently.
This information is obtained by profiling the program. Cold fields are placed into a new object via an indirection and hot fields remain unchanged. In their approach, at runtime, there is a cache-concious garbage collector~\cite{ccgarbage} that co-locates the modified object instances.
This paper also suggests placing fields with high temporal affinity within the same cache block. For this they recommend  \texttt{bbcache}, a field recommender for a data structure. \texttt{bbcache} forms a field affinity graph which combines static information about the source location of structure field accesses with dynamic information about the temporal ordering of accesses and their access frequency.
% \textbf{Shortcomings: } Applicable to only the pointer world, does not apply to the packed world like in gibbon where the trees are serialized in memory. Not applicable to functional progams. Does not apply to recursive data structures.

% \paragraph{Cache-Conscious Structure Layout~\cite{CSL}}

%Poor reference locality is one major bottleneck in today's programs. Since programmers often do not program keeping in mind the hierarchical  structure of caches in today's architectures, the memory performance of these programs is sometimes far from ideal.
% This paper targets the problem at the source, i.e, solve the problem of poor reference locality within these programs (pointer based programs in C).
%Their proposed technique is improves on prior work in that it requires less programmer effort, less architectural dependence and less source code modifications.
Chilimbi et al.~\cite{CSL} propose two techniques to solve the problem of poor reference locality.
\begin{description}
\item[ccmorph] This works on tree-like data structures, and it relies on the programmer making a calculated guess about the safety of the operation on the tree-like data structure. It performs two major optimizations: clustering and coloring. Clustering take a the tree like data structure and attempts to pack likely to be accessed elements in the structure within the same cache block. There are various ways to pack a subtree, including clustering $k$ nodes in a subtree together, depth first clustering, etc.
% This depends on the program. This technique does not attempt to suggest the optimal clustering based on the program.
Coloring attempts to map simultaneously accessed data elements to non-conflicting regions of the cache.
\item[ccmalloc] This is a memory allocator similar to \texttt{malloc} which takes an additional parameter that points to an existing data structure element which is likely accessed simultaneously. This requires programmer knowledge and effort in recognizing and then modifying the code with such a data element. \texttt{ccmalloc} tries to allocate the new data element as close to the existing data as possible, with the initial attempt being to allocate in the same cache block. It tries to put likely accessed elements on the same page in an attempt to improve TLB performance.
\end{description}
%Using these techniques they are able to get significant improvements in the run-time of the program. Future work is to get rid of programmer effort and be able to analyze the program statically or profiling techniques.

%\paragraph{SHAPES~\cite{Shapes, Shapes2}}
Franco et al.~\cite{Shapes, Shapes2} suggest
that the layout of a data structure should be defined once at the point of initialization, and all further code that interacts with the structure should be ``layout agnostic''. Ideally, this means that performance improvements involving layout changes can be made without requiring changes to program logic. To achieve this, classes are extended to support different layouts, and types carry layout information---code that operates on objects may be polymorphic over the layout details.

\subsection{Data layout description and binary formats}

Chen et al.~\cite{Dargent} propose a data layout description framework \emph{Dargent}, which allows programmers to specify the data layout of an ADT. It is built on top of the Cogent language~\cite{o2016cogent}, which is a first order polymorphic functional programming language. Dargent targets C code and provides proofs of formal correctness of the compiled C code with respect to the layout descriptions. Rather than having a compiler attempting to determine an efficient layout, their focus is on allowing the programmer to specify a particular layout they want and have confidence in the resulting C code.
% Their work however, is set in a different environment and does not evaluate the data layout transformations in view of performance. In addition, they do not automatically optimize for the best layout when it comes to performance. Their work does not support the ordering of recursive fields in the algebraic data type either.

% \paragraph{PADS ~\cite{PADS, Pads2, Pads3}} Something about PADS/ML here.

% \subsection{Protocols, parsing, and binary formats}

Significant prior work went into generation of verified efficient code for interacting with binary data formats (parsing and validating). For example, EverParse~\cite{EverParse} is a framework for generating verified parsers and formatters for binary data formats, and it has been used to formally verify zero-copy parsers for authenticated message formats. With Narcissus~\cite{Narcissus}, encoders and decoders for binary formats could be verified and extracted, allowing researchers to certify the packet processing for a full internet protocol stack. Other work~\cite{GenericPacketDescriptions} has also explored the automatic generation of verified parsers and pretty printers given a specification of a binary data format, as well as the formal verification of a compiler for a subset of the Procotol Buffer serialization format~\cite{VPBdeleware}.

Back~\cite{DataScript} demonstrates how a domain-specific language for describing binary data formats could be useful for generating validators and for easier scripting and manipulation of the data from a high-level language like Java. \cite{PacketTypes} introduce \emph{Packet Types} for programming with network protocol messages and provide language-level support for features commonly found in protocol formats like variable-sized and optional fields.

%Data Representation Synthesis~
Hawkins et al.~\cite{Hawkins} introduce \relc, a framework for synthesizing low-level C\texttt{++} code from a high-level
relational representation of the code. The user describes and writes code that represents data at a high level as relations. Using a decomposition
of the data that outlines memory representation, \relc synthesizes correct and efficient low-level code.

Baudon et al.~\cite{BitStealingMadeLegal} introduce the \ribbit DSL, which allows programmers to describe the layout of ADTs that are monomorphic and immutable.
\ribbit provides a dual view on ADTs that allows both a high-level description of the ADT that the client code follows and a user-defined memory representation of the ADT
for a fine-grained encoding of the layout. Precise control over memory layout allows \ribbit authors to develop optimization algorithms over the ADTs, such as struct packing, bit stealing, pointer tagging, unboxing, etc.
Although this approach enables improvements to layout of ADTs, it is different from \system's: \ribbit focuses on \emph{manually} defining low-level memory representation of the ADT whereas \system \emph{automatically} optimizes the high-level layout (ordering of fields in the definition ADT) relying on \gibbon for efficient packing of the fields.
While \ribbit invites the programmer to encode their best guess about the optimal layout, \system comes up with such layout by analysing access patterns in the source code.
% This has performance enhancing effects due to locality. % Artem: looks disconnected from the previous sentence

\subsection{Memory layouts}


Early work on specifications of memory layouts was explored in various studies of PADS, a language for describing ad hoc data-file formats~\cite{PADS, Pads2, Pads3}.

Lattner and Adve~\cite{poolallocation} introduce a technique for improving the memory layout of the heap of a given C program.
%
Their approach is to use the results of a custom static analysis to enable \emph{pool allocation} of heap objects.
%
Such automatic pool allocation bears some resemblance to our approach, where we use region-based allocation in tandem with region inference, and thanks to static analysis can group fields of a given struct into the same pool, thereby
improving locality in certain circumstances.
%

Floorplan~\cite{Floorplan} is a declarative language for specifying high-level memory layouts, implemented as a compiler which generates Rust code. The language has forms for specifying sizes, alignments, and other features of chunks of memory in the heap, with the idea that any correct state of the heap can be derived from the Floorplan specification. It was successfully used to eliminate 55 out of 63 unsafe lines of code (all of the unsafe code relating to memory safety) of the immix garbage collector.


% While this paper has been concerned with the format and layout of serialized objects and fields in memory, there has been significant research on the serialized layout of data persisted to disk or sent over the network: on the specification of network message protocols~\cite{PacketTypes}, on the efficient parsing of authenticated message formats and binary data~\cite{EverParse}, and so on. Similarly, prior work has explored the verified  with binary data~\cite{DataScript, Narcissus}.

% \subsection{Uncategorized}

% \paragraph{Shapes~\cite{Shapes, Shapes2}}

% \paragraph{hobbit~\cite{Hobbit, Hobbit2}}

% \paragraph{Contiguity types ~\cite{contiguityTypes}}

% \paragraph{The hardness of cache conscious data placement ~\cite{hardnessLayout}}

% \paragraph{Data layout optimization based on the spatio-temporal model of field access ~\cite{9948361}}

% \paragraph{Recursion Twisting ~\cite{recursionTwisting}}

%\paragraph{Automatic Pool Allocation for Disjoint Data Structures ~\cite{poolallocation}}


%The idea is that it is easier to perform intraprocedural optimization at link time when multiple files are being compiled together. The compiler generates data structure graphs of disjoint data structures for each functions, for data structures that are accessed in a type safe manner, it automatically allocates pools for data structures.

% \paragraph{Detecting Conflicts Between Structure Accesses ~\cite{larusAndHilfinger}}

% \paragraph{An analytical cache model ~\cite{analyticalCacheModel}}

% \paragraph{Principles of optimal page replacement ~\cite{popr}}

% \paragraph{Organizing and maintenance of large ordered indexes ~\cite{Bayer1972OrganizationAM}}

% \paragraph{Enhancing performance in a persistent object store ~\cite{eronique1995enhancing}}

